Equivariant Hypergraph Diffusion Neural Operators

Hypergraph neural networks (HNNs) using neural networks to encode hypergraphs provide a promising way to model higher-order relations in data and further solve relevant prediction tasks built upon such higher-order relations. However, higher-order relations in practice contain complex patterns and are often highly irregular. So, it is often challenging to design an HNN that suffices to express those relations while keeping computational efficiency. Inspired by hypergraph diffusion algorithms, this work proposes a new HNN architecture named ED-HNN, which provably represents any continuous equivariant hypergraph diffusion operators that can model a wide range of higher-order relations. ED-HNN can be implemented efficiently by combining star expansions of hypergraphs with standard message passing neural networks. ED-HNN further shows great superiority in processing heterophilic hypergraphs and constructing deep models. We evaluate ED-HNN for node classification on nine real-world hypergraph datasets. ED-HNN uniformly outperforms the best baselines over these nine datasets and achieves more than 2\%$\uparrow$ in prediction accuracy over four datasets therein.

==> arxiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> arxiv/section_files/000-abstract.tex <==
   \vspace{-3mm}
\begin{abstract}
\setcounter{footnote}{0}
    Hypergraph neural networks (HNNs) using neural networks to encode hypergraphs provide a promising way to model higher-order relations in data and further solve relevant prediction tasks built upon such higher-order relations. However, higher-order relations in practice contain complex patterns and are often highly irregular. So, it is often challenging to design an HNN that suffices to express those relations while keeping computational efficiency. Inspired by hypergraph diffusion algorithms, this work proposes a new HNN architecture named \proj, which provably approximates any continuous equivariant hypergraph diffusion operators that can model a wide range of higher-order relations. \proj can be implemented efficiently by combining star expansions of hypergraphs with standard message passing neural networks. \proj further shows great superiority in processing heterophilic hypergraphs and constructing deep models. We evaluate \proj for node classification on nine real-world hypergraph datasets. \proj\footnote{Our code is available at: \url{https://github.com/Graph-COM/ED-HNN}.} uniformly outperforms the best baselines over these nine datasets and achieves more than 2\%$\uparrow$ in prediction accuracy over four datasets therein.       
    %The irregularity of those relations also cause computation challenges.   
    %are inpired by the recently designed hypergraph diffusion algorithms and
   % it is often unclear whether they are rc enough to represent certain higher-order relations.  %they could model. Building complicated HNNs 
    
  %Hypergraphs provide the abstraction to study higher-order relations in data. Hypergraph neural networks (HNNs) that use neural networks to encode hypergraph data have recently been investigated for the prediction tasks on hypergraphs. However, the design of HNNs is challenging as it is often unclear what types of higher-order relations in data they could model. On the other hand, too    
\end{abstract}

==> arxiv/section_files/001-introduction.tex <==
  \vspace{-2mm}
\section{Introduction} \label{sec:intro}
  \vspace{-1mm}
Machine learning on graphs has recently attracted great attention in the community due to the ubiquitous graph-structured data and the associated inference and prediction problems~\cite{zhu2005semi,zhu2003semi,zhou2004learning,hamilton2020graph,nickel2015review,chami2020machine}.
Current works primarily focus on graphs which can model only pairwise relations in data. Emerging research has shown that higher-order relations that involve more than two entities often reveal more significant information in many applications~\cite{benson2021higher,schaub2021signal,battiston2020networks,lambiotte2019networks,liu2022neural}. For example, higher-order network motifs build the  fundamental  blocks of many real-world networks~\cite{mangan2003structure,benson2016higher,tsourakakis2017scalable,li2017motif,li2017inhomogeneous}. Session-based (multi-step) behaviors often indicate the preferences of web users in more precise ways~\cite{xia2021self,wang2021session,wang2020next,wang2022exploiting}. To capture these higher-order relations, hypergraphs provide a dedicated mathematical abstraction~\cite{berge1984hypergraphs}. However, learning algorithms on hypergraphs are still far  underdeveloped as opposed to those on graphs.

Recently, inspired by the success of graph neural networks (GNNs), researchers have started investigating hypergraph neural network models (HNNs)~\cite{feng2019hypergraph,yadati2019hypergcn,dong2020hnhn,huang2021unignn,chien2021you,bai2021hypergraph,arya2020hypersage,yadati2020neural,yang2020hypergraph}. %Similarly to GNNs, HNNs associate the nodes in the hypergraph with vector representations and then keep updating those representations by combining the representations from the neighbors. 
Compared with GNNs, designing HNNs is more challenging. First, as aforementioned, higher-order relations modeled by hyperedges could contain very complex information. Second, hyperedges in real-world hypergraphs are often of large and irregular sizes. Therefore, how to effectively represent higher-order relations while efficiently processing those irregular hyperedges is the key question to answer when one is to design HNNs. Unfortunately, just as other types of neural networks (NNs), HNNs look like a black box. Given an HNN, one can hardly tell the type of relations that it can represent and thus often fails to make a suitable tradeoff between the expressiveness and the computational efficiency of the model.        


%effectiveness and efficiency often form a tradeoff.
%However, previous works often designed HNNs based on heuristics, which results in either less expressive models or over-complicated models. We provide a detailed explanation in Sec.~\ref{sec:previous} 

%However, previous works often       
%First, hyperedges are often of large and irregular sizes. How to efficiently   
%as for higher-order relations modeled by the hyperedges, different    design a novel HNN architecture,  
%benchmark the design of HNNs  


In this work, inspired by the recently developed  hypergraph diffusion algorithms~\cite{zhou2007learning,hein2013total,li2020quadratic,liu2021strongly,fountoulakis2021local,takai2020hypergraph,zhang2017re,tudisco2021nonlinear}, we design a novel HNN architecture that holds provable expressiveness to approximate a large class of hypergraph diffusion while keeping computational efficiency. Hypergraph diffusion is significant due to its transparency and has been widely applied to clustering~\cite{zhou2007learning,li2017inhomogeneous,li2018submodular}, semi-supervised learning~\cite{hein2013total,zhang2017re,tudisco2021nonlinear,li2018quadratic}, ranking aggregation~\cite{li2017inhomogeneous,chitra2019random}, network analysis~\cite{li2020quadratic,liu2021strongly,fountoulakis2021local,takai2020hypergraph} and signal processing~\cite{zhang2019introducing,schaub2021signal,komodakis2009beyond,werner2008high}. However, traditional hypergraph diffusion needs to first handcraft potential functions to  model higher-order relations and then use their gradients or some variants of their gradients as the diffusion operators to characterize the exchange of diffused quantities on the nodes within one hyperedge. The design of those potential functions often requires significant insights into the applications, which may not be available in practice.

%This covers the applications where none of the nodes in a higher-order relation are treated as inherently special.

We observe that the most commonly-used hyperedge potential functions are permutation invariant, which covers the applications where none of the nodes in a higher-order relation are treated as inherently special. For such potential functions, we further show that their induced diffusion operators must be permutation equivariant. Inspired by this observation, we propose a NN-parameterized permutation-equivariant architecture that is expressive to provably represent any continuous hyperedge diffusion operators, whose NN parameters can be learned in a data-driven way. We also introduce an efficient implementation of the architecture that can be easily implemented over current GNN platforms~\cite{FeyPyG,wang2019dgl}: We just need to combine a bipartite representation (or star expansion~\cite{agarwal2006higher,zien1999multilevel}, equivalently) of hypergraphs and the standard message passing neural network (MPNN)~\cite{gilmer2017neural}. By repeating this architecture by layers with shared parameters, we finally obtain our model named Equivariant Diffusion-based HNN (\proj). Fig.~\ref{fig:diag} shows an illustration of hypergraph diffusion and the key architecture in \proj. 

To the best of our knowledge, we are the first one to establish the connection between the general class of hypergraph diffusion algorithms and the design of HNNs. Previous HNNs were either less expressive to represent equivariant diffusion operators~\cite{feng2019hypergraph,yadati2019hypergcn,dong2020hnhn,huang2021unignn,chien2021you,bai2021hypergraph} or needed to learn the representations by adding significantly many auxiliary nodes~\cite{arya2020hypersage,yadati2020neural,yang2020hypergraph}. We provide detailed discussion of them in Sec.~\ref{sec:previous}. We also show that due to the equivariant architecture, \proj is by design good at predicting node labels over heterophilic hypergraphs where hyperedges mix nodes from different classes. Moreover, \proj can go very deep without much performance decay. %due to the parameter sharing across layers. 

As a by-product, our proof of expressiveness does not use equivariant polynomials as a bridge, which were used previously in set-function approximation~\cite{zaheer2017deepset,maron2018invariant,segol2020universal}. Our statement allows precise representations of continuous equivariant set functions (when each set element has 1-dim feature channel) by compositing a continuous function and the sum of another continuous function on each set entry, while previous works have only achieved an approximation result. This result may be of independent interest for the community.         

We evaluate \proj by performing node classsification over 9 real-world hypergraph datasets. \proj uniformly outperforms all baseline methods in averaged performance and achieves significant improvement (more than 2$\%\uparrow$) over 4 datasets therein. \proj also shows super robustness when going deep. We further carefully design synthetic experiments to demonstrate the expressiveness of \proj and the superiority of \proj in processing heterphilic hypergraphs. 

\begin{figure}[t]
    \centering
    \includegraphics[trim={0.3cm 11.7cm 0.1cm 4cm},clip,width=1.\linewidth]{images/Main-Diag.pdf}
    \vspace{-6mm}
    \caption{Hypergraph diffusion often uses permutation-invariant hyperedge potentials to model higher-order relations. The gradients or their variants  of those potentials determine the diffusion process and are termed diffusion operators. Our \proj can universally represent such operators by feeding node representations into the message from hyperedges to nodes.}
       \vspace{-3mm}
    \label{fig:diag}
\end{figure}
%over... (\pan{Todo: emphasize real-data exp, heterophily and expressiveness}).


% have been proposed~\cite{}, while the  ~\cite{}.
% are proposed to hyperedges have been associated with set functions and Lov\'{a}sz extension-based potentials have found greatly useful~\cite{}.

% so the total-variation potential was proposed and behaved well in the case with large hyperedges~\cite{hein2013total,zhang2017re}. Recently, to model complex higher-order patterns, hyperedges have been associated with set functions and Lov\'{a}sz extension-based potentials have found greatly useful~\cite{}.  


% Hypergraph diffusion has been widely used  


% Finding the minimal potential point, which essentially  

% which may guide the flow  the  
% potential functions  

% make accurate recommendation~\cite{}.        


% 1. Explain the importance of higher-order graph/hypergraph learning. Introduce one or two real-world examples (network motif applications, higher-order MRF).

% 2. Recent works on hypergraph neural networks mainly generalized standard GNNs to hypergraphs and proposed hypergraph neural networks as a black box. Seldom works really investigated into the mechanism and built its connection to white-box hypergraph learning problems. 

% 3. Our work is motivated by the traditional learning algorithm to compute Hypergraph PageRanks and Higher-order MRF MAP. 

% \pan{Move a part to introduction} Hypergraph diffusion has been widely used in data clustering~\cite{zhou2007learning,li2017inhomogeneous,li2018submodular}, semi-supervised learning~\cite{hein2013total,zhang2017re,tudisco2021nonlinear}, ranking aggregation~\cite{li2017inhomogeneous,chitra2019random}, network analysis~\cite{li2018quadratic,liu2021strongly,fountoulakis2021local,takai2020hypergraph}, signal denoising~\cite{zhang2019introducing,schaub2021signal}, inference over higher-order markov random field~\cite{komodakis2009beyond,werner2008high}. 

% \\ We observe that both (sub)gradient descent algorithm and Douglas-Rachford splitting algorithm essentially correspond to iteratively using (permutation) equivariant diffusion operators designed on hyperedges. 
% \\ However, all previous hypergraph neural network models fail to model equivariant diffusion operators on hyperedges and restrict themselves to over-simplified invariant diffusion operators. 
% \\ Not surprisingly, previous models suffer from either limited expressive power or generalization issues induced by over-complex neural network layers to complement the loss of expressive power.   

% 4. In this work, we propose hypergraph neural networks (HNN) based on equivariant diffusion (ED) operators and call the model \proj 
% \\ Each \proj layer contains the following three steps: (1) Learn hyperedge representations via a sum pooling of node representations of each hyperedge; (2) Operate a concatenation of the representations of \emph{each node-hyperedge pair} to compute the messages from hyperedges to nodes; (3) Update node representations via a sum-pooling of the messages.
% \\ The second step is the key to implement ED, which makes our model substantially different from previous HNN models. 
% \\ We may show \proj universally approximates any continuous hypergraph diffusion operators.
% %\\ We systematically study the advantages of using ED. 
% \\ In theory, we further prove that using ED a much smaller latent dimension of node/hyperedge representations is needed to represent hypergraph diffusion than using invariant diffusion (ID). 
% \\ As a by-product, our proof techniques also strengthen the previous argument on the expressive power of equivariant set functions. We avoid using equivariant polynomials and reduce the needed dimensions of the element representations in the set from an exponential order to a linear order.    

% 5. Empirically, we evaluate \proj in two synthetic settings and xxx many real-world hypergraph node classification tasks. \\
% The first synthetic setting shows that ED much better approximate hypergraph diffusion than ID to justify our theory.  \\
% The second synthetic setting shows that ED is extremely good at learning node labels across different heterophilic levels of hypergraphs generated by stochastic block models. \\ 
% ED-GNN also significantly outperforms baselines on real-world hypergraphs by about xxx. 

% \pan{Mention that hypergraph diffusion -> node level tasks, leave graph level tasks for future study}


  

==> arxiv/section_files/002-preliminaries.tex <==
   \vspace{-2mm}
\section{Preliminaries: Hypergraphs and Hypergraph Diffusion} \label{sec:prelim}
   \vspace{-1mm}
% We are interested in supervised learning problems on hypergraphs by a diffusion model, in which we are given nodes with features and labels, as well as hyperedges connecting them.

In this section, we formulate the hypergraph diffusion problem, along the way, introduce the notations.
\begin{definition}[Hypergraph] \label{def:hypergraph}
 Let $\Set{G} = (\Set{V}, \Set{E}, \Mat{X})$ be an attributed hypergraph where $\Set{V}$ is the node set of size $N$ and $\Set{E}$ is the hyperedge set of size $M$. Each hyperedge $e = \{v_1^{(e)},...,v_{\lvert e \rvert}^{(e)}\}$ is a subset of $\Set{V}$. Unlike graphs, a hyperedge may contain more than two nodes. $\Mat{X}=[...,\Mat{x}_v,...]^T\in\mathbb{R}^{N}$ denotes the node attributes and $\Mat{x}_v$ denotes the attribute of node $v$. Define $d_v=|\{e\in\mathcal{E}:v\in e\}|$ as the degree of node $v$. Let $\Mat{D},\,\Mat{D}_e$ denote the diagonal degree matrix for $v\in\Set{V}$ and the sub-matrix for $v\in e$.
%Let $\Mat{K} \in \{0, 1\}^{n \times m}$ denote the incident matrix where $\Mat{K}_{ij} = 1$ if and only if $v_i \in e_j$. 
\end{definition}
%A hyperedge $e$ may contain more than two nodes so hypergraphs are used to model higher-order relational data.

Here, we use 1-dim attributes for convenient discussion while our experiments often have multi-dim attributes. Learning algorithms will combine attributes and hypergraph structures into (latent) features defined as follows. These features can be further used to make prediction for downstream tasks.
\begin{definition}[Latent features] \label{def:node_feat}
Let $\Mat{h}_v \in \real$ denote the (latent) features of node $v\in \Set{V}$. The feature vector $\Mat{H} = \begin{bmatrix}..., \Mat{h}_{v}, ... \end{bmatrix}_{v\in\Set{V}}^\top \in \real^{N}$ includes node features as entries. Further, collect the features into a edge feature vector $\Mat{H}_e = \begin{bmatrix} \Mat{h}_{e, 1} & \cdots & \Mat{h}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert}$, where $\Mat{h}_{e,i}$ corresponds to the feature $\Mat{h}_{v_i^{(e)}}$ for some node $v_i^{(e)}\in e$.  Note that for any $v\in e$, there is one corresponding index $i\in \{1,...,\lvert e\rvert\}$. Later, we may use subscripts $(e,i)$ and $(e,v)$ interchangeably if they cause no confusion. %For, $i\in [F]$, we use $\Mat{H}_e[i]$ and $\Mat{h}_v[i]$ to denote the corresponding $i$th feature channels.
%collect all the feature vectors of nodes within edge $e$, where $\Mat{h}_{e,i}$ corresponds to the node features of node $v_i^{(e)}$ inside hyperedge $e$. 
%Suppose each node has initial features $\Mat{x}_i \in \real^d$ which are organized by initial feature matrix $\Mat{X} \in \real^{n \times d}$.
\end{definition}

A widely-used heuristic to generate features $\Mat{H}$ is via hypergraph diffusion algorithms. 

\begin{definition}[Hypergraph Diffusion] \label{def:node_feat}
Define node potential functions $f(\cdot;\Mat{x}_v):\mathbb{R} \rightarrow \mathbb{R}$ for $v\in\Set{V}$ and hyperedge potential functions $g_e(\cdot):\mathbb{R}^{|e|} \rightarrow \mathbb{R}$ for each $e\in\Set{E}$.  The hypergrah diffusion combines the node attributes and the hypergraph structure and asks to solve
\begin{align} \label{eqn:diffusion}
    \min_{\Mat{H}} \sum_{v \in \Set{V}} f(\Mat{h}_v; \Mat{x}_v) + \sum_{e \in \Set{E}} g_e(\Mat{H}_e).
\end{align}
In practice, $g_e$ is often shared across hyperedges of the same size. Later, we ignore the subscript $e$.
\end{definition}


The two potential functions are often designed via heuristics in traditional hypergraph diffusion literatures. Node potentials often correspond to some negative-log kernels of the latent features and the initial attributes. For example, $f(\Mat{h}_v; \Mat{x}_v)$ could be $(\Mat{h}_v - \Mat{x}_v)_2^2$ when to compute hypergraph PageRank diffusion~\cite{li2020quadratic,takai2020hypergraph} or $-\Mat{x}_v\Mat{h}_v$ when to compute hypergraph min-cut~\cite{stobbe2010efficient,jegelka2013reflection,li2018revisiting}. Hyperedge potentials are more significant and complex, as they need to model those higher-order relations between more than two objects. Here list a few examples. 

\begin{example}[Hyperedge potentials] \label{exp:potential}
Some practical $g(\Mat{H}_e)$ may be chosen as follows. %Note that most previous works only contain one feature channel $F=1$. Here, we list their general variants.
\begin{itemize}[leftmargin=3mm]
    \item Clique Expansion (CE, hyperedges reduced to cliques) plus pairwise potentials~\cite{zhou2007learning}: $\sum_{u,v\in e} (\Mat{h}_v-\Mat{h}_{u})_2^2 $ or with properly degree normalization $\sum_{u,v\in e}(\frac{\Mat{h}_v}{\sqrt{d_v}}-\frac{\Mat{h}_u}{\sqrt{d_u}})_2^2\,(\triangleq g(\Mat{D}_e^{-1/2}\Mat{H}_e))$.\vspace{-0.5mm}
    \item Divergence to the  mean~\cite{tudisco2021nonlinear,tudisco2021nonlinear2}: $\sum_{v\in e} (\Mat{h}_v-\||e|^{-1}\Mat{H}_e\|_p)_2^2$, where $\|\cdot\|_p$ computes the $\ell_p$-norm. \vspace{-0.5mm} %each feature channel of $\Mat{H}_e$ separately.% where the number of features channels is $F=1$.
    \item Total Variation (TV)~\cite{hein2013total,zhang2017re,takai2020hypergraph}: $\max_{u,v\in e} |\Mat{h}_v-\Mat{h}_u|^p$, $p\in\{1,2\}$. \vspace{-0.5mm}% where the number of features channels is $F=1$.
    \item Lov\'{a}sz Extension~\cite{lovasz1983submodular} for cardinality-based set functions (LEC)~\cite{jegelka2013reflection,li2018submodular,li2020quadratic,liu2021strongly}: $\langle \Mat{y}, \varsigma(\Mat{H}_e) \rangle^p$, $p\in\{1,2\}$ where $\Mat{y}=\begin{bmatrix} ...,\Mat{y}_j,... \end{bmatrix}^\top\in\mathbb{R}^{|e|}$ is a constant vector and $\varsigma(\Mat{H}_e)$ sorts the values of $\Mat{H}_e$ in a decreasing order.% is also in a decreasing order, i.e., $y_j\geq \Mat{y}_{j+1}$, $\forall j\in[e-1]$. %Here, suppose  $\Mat{y}_{|e|+1}=0$\, for convenience.
    %\item Lov\'{a}sz Extension for cardinality-based set functions  (LE)~\cite{lovasz1983submodular,jegelka2013reflection,li2018revisiting,li2018quadratic}: $\sum_{i=1}^F\max_{\Mat{y}_i\in \Set{B}_e}\langle \Mat{y}_i, \Mat{H}_e[i] \rangle^p$, $p\in\{1,2\}$, where  $\Set{B}_e\subset\mathbb{R}^{|e|}$ is the base polytope induced by a submodular function defined on $e$. This generalizes total variation. 
\end{itemize}\vspace{-2mm}
\end{example}
One may reproduce TV by using LEC and setting $\Mat{y}_1=-\Mat{y}_{|e|}=1$. To reveal more properties of these hyperedge potentials $g(\cdot)$ later, we give the following definitions.

%Heuristic $g(\cdot)$'s are complicated while they all satisfies permutation invariance defined as follows.  %To reveal more properties of $g(\cdot)$, we list the following formal definitions:

% \begin{definition} \label{def:permutation}
% Let $\pi: [K] \rightarrow [K]$ be an automorphism, then permutation matrix  is defined as $\Mat{P}_{\pi}$ who has value one at entries $(\pi(i),i), \forall i \in [K]$ while taking zero at any other positions.
% A permutation group $\Pi[K]$ is defined as a set which collects all of such $\Mat{P}_\pi$.
% \end{definition}

% \begin{definition}[Permutation Invariance \& Equivariance] \label{def:permutation_ivariant} 
% Function $\psi: \mathbb{R}^{K\times F} \rightarrow \real^{F'}$ is permutation-invariant if for any $K$-dim permutation matrix $\Mat{P}\in\Pi[K]$, %$\,\forall \Mat{P} \in \Pi[K]$ denote permutation matrix, 
% $\psi(\Mat{P} \Mat{Z}) = \psi(\Mat{Z})$ for all $\Mat{Z} \in \mathbb{R}^{K\times F}$. Function $\psi: \mathbb{R}^{K\times F} \rightarrow \mathbb{R}^{K\times F'}$ is permutation-equivariant if for any $K$-dim permutation matrix $\Mat{P}\in\Pi[K]$, $\psi(\Mat{P} \Mat{Z}) = \Mat{P}\psi(\Mat{Z})$ for all $\Mat{Z} \in \mathbb{R}^{K\times F}$.
% \end{definition}
\begin{definition}[Permutation Invariance \& Equivariance] \label{def:permutation_ivariant} 
Function $\psi: \mathbb{R}^{K} \rightarrow \real$ is permutation-invariant if for any $K$-dim permutation matrix $\Mat{P}\in\Pi[K]$, %$\,\forall \Mat{P} \in \Pi[K]$ denote permutation matrix, 
$\psi(\Mat{P} \Mat{Z}) = \psi(\Mat{Z})$ for all $\Mat{Z} \in \mathbb{R}^{K}$. Function $\psi: \mathbb{R}^{K} \rightarrow \mathbb{R}^{K}$ is permutation-equivariant if for any $K$-dim permutation matrix $\Mat{P}\in\Pi[K]$, $\psi(\Mat{P} \Mat{Z}) = \Mat{P}\psi(\Mat{Z})$ for all $\Mat{Z} \in \mathbb{R}^{K}$.
\end{definition}

%\begin{definition} \label{def:permutation_equivariant} (Permutation Equivariance)
%Let $f: \real^k \rightarrow \real^k$ be a permutation-equivariant function, then $\forall \Mat{P} \in \Grp{P}_k$, $f(\Mat{P} \Mat{x}) = \Mat{P} f(\Mat{x})$ for all $\Mat{x} \in \real^k$.
%\end{definition}

%Here, $F,F'$ could be any positive integers, which become clear based on the context. 
We may easily verify permutation invariance of the hyperedge potentials in Example~\ref{exp:potential}. The physical meaning behind this observation is that the prediction goal of an application is often independent of node identities in a hyperedge so practical $g$'s often keep invariant w.r.t. the node ordering~\cite{veldt2020hypergraph}.
%affect the diffusion results.   

%We note that potential function $g(\cdot)$ should be permutation-invariant since row permutation of the edge feature matrix results in an equivalent class. \pan{This may be more natural put with g definition together.}
%No matter in which order we arrange data inside $\Mat{H}_e$, $g(\cdot)$ should give the identical potential value. 




% Here are a few examples. 
% \begin{example}[Node potentials]
% The node potential $f(\Mat{h}_v; \Mat{x}_v)$ often corresponds to a negative-log kernel of the latent features and the initial attributes: (a) Hypergraph PageRank diffusion~\cite{li2018quadratic,takai2020hypergraph}, $\|\Mat{h}_v - \Mat{x}_v\|_2^2$; (b) Hypergraph min-cut diffusion~\cite{stobbe2010efficient}, $-\Mat{h}_v^T\Mat{x}_v$.
% \end{example}

% For example, node potential $f(\Mat{h}_v; \Mat{x}_v)$ could be $\|\Mat{h}_v - \Mat{x}_v\|_2^2$ when to compute hypergraph PageRank diffusion~\cite{li2018quadratic,takai2020hypergraph} or $-\Mat{h}_v^T\Mat{x}_v$ to compute hypergraph cut~\cite{stobbe2010efficient}. Examples of edge potentials $g(\Mat{H}_e)$ include a combination of clique expansion and pairwise potentials $\sum_{u,v\in e} \|\Mat{x}_v-\Mat{x}_u\|_2^2$, Lov\'{a}sz extension and \cite{tudisco2021nonlinear}.   

% (Heuristics, cannot apply to heterophilic)

% hypergraph diffusion include hypergraph  

% Node potential: $f_v(\cdot ;x_v)$: $\mathbb{R}^{m} \rightarrow \mathbb{R}.$ %We assume that $f_v = f_{u}$ if the node degree $d_v = d_{u'}$.
%     \item hyperedge potential: $g_e(\cdot): \mathbb{R}^{|e|\times m}\times \mathbb{R}$. %We
%     %Denote $\bar{z} =(z_1,z_2^{(e)},...,z_|e|^{(e)})$ where $z_{i}^{(e)}$ is the block of the input vector $\bar{z}_e$ associated with node $v_{i}^{(e)}$.
    
%     \item In hypergraphs, we often do not have node identities so $f_v=f_u$ if $d_v= d_{u}$. We also assume that $g_e = g_{e'}$ if $|e| = |e'|$ and $g_{e}$ is permutation invariant: $g_e(\bar{h}_e) = g_e(\bar{h}'_e)$ if $\{\Mat{h}_v|v\in e\}=\{\Mat{h}_v'|v\in e\}$. As the information of node degrees and hyperedge sizes are clear, we simply use $f$ and $g$ to uniformly denote node potentials and hyperedge potentials respectively.

% Unlike ordinary graphs, a hyperedge can connect with more than two nodes, i.e., $\lvert e \rvert \ge 2$.
% To attain node adjacent matrix (i.e., an $n$ by $n$ matrix whose non-zero entries indicate which two nodes are connected), one can use $\Mat{K}\Mat{K}^\top$ that transforms hyperedges into cliques.
% \begin{definition}[Node features] \label{def:node_feat}
% Let $\Mat{h}_i \in \real^d$  \pan{revise to $F$} be the node embedding of the node $v_i \in \Set{V}$. We organize all the node features into the rows of a feature matrix $\Mat{H} = \begin{bmatrix} \Mat{h}_{1} & \cdots & \Mat{h}_{n} \end{bmatrix}^\top \in \real^{n \times d}$. Suppose each node has initial features $\Mat{x}_i \in \real^d$ which are organized by initial feature matrix $\Mat{X} \in \real^{n \times d}$.
% \end{definition}

% % Similarly, we let matrix $\Mat{H} = \begin{bmatrix} \Mat{h}_{1} & \cdots & \Mat{h}_{n} \end{bmatrix}^\top \in \real^{n \times d}$ concatenates all the node features after diffusion.
% \begin{definition}[Edge features] \label{def:edge_feat}
% % Given an hyperedge $e \in \Set{E}$, the 
% Let edge feature matrix $\Mat{H}_e = \begin{bmatrix} \Mat{h}_{e, 1} & \cdots & \Mat{h}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert \times d}$ collect all the feature vectors of nodes within edge $e$, where $\Mat{h}_{e,i}$ corresponds to the node features of node $v_i^{(e)}$ inside hyperedge $e$. \pan{Define the relation between $\Mat{h}_{e}$ and $\Mat{h}$. Denote an implicit mapping between $(e,i)$ and $(e,v)$.}
% \end{definition}

% Hypergraph diffusion algorithms solve node embeddings \pan{unify the terminology} $\Mat{H}$ to minimize some potential functions \pan{add some background} defined over hypergraphs.
% We proposed a general hypergraph diffusion model \pan{Review hypergraph diffusion instead of proposing a model; Also motivates the applications of this is crucial.} that accumulates potential of individual node embeddings and the joint potential among nodes connected by each hyperedge in a hypergraph $\Set{G}$:
% \begin{align} \label{eqn:diffusion}
%     \min_{\Mat{H}} \sum_{v \in \Set{V}} f(\Mat{h}_v; \Mat{x}_v) + \sum_{e \in \Set{E}} g(\Mat{H}_e),
% \end{align}
% where $f: \real^{d} \rightarrow \real$ denotes the node potential function, which defines an independent likelihood of each node representation, $g
% : \real^{\lvert e \rvert \times d} \rightarrow \real$ is the hyperedge potential function \pan{different hyperedges may have different sizes}, which specifies a joint constraints on the embeddings of nodes connected by one hyperedge.
% \textcolor{red}{High-Order Page Rank}.
% \textcolor{red}{High-Order Markov Random Field}.

% To optimize Eq.~\eqref{eqn:diffusion}, it is often to use gradient-based methods which we will elaborate in Sec. \ref{sec:model} \pan{Need better motivations, add references and discuss previous approaches; Okay, we should put this into the next section.}. 
% Suppose $f(\cdot)$ and $g(\cdot)$ are differentiable, then we denote the gradient of $f(\cdot)$ taking value at $\Mat{h}_v$ as: $\nabla f(\Mat{h}_v; \Mat{x}) = \frac{\partial f(\Mat{z}; \Mat{x})}{\partial \Mat{z}} \lvert_{\Mat{z} = \Mat{h}_v}$,
% and since $g(\cdot)$ is a function of a set of nodes, its partial derivative with respect to node $v$ taking value at $\Mat{H}_e$ is defined as: $\nabla_v g(\Mat{H}_e) = \nabla_v g\left(\Mat{h}_{e, 1}, \cdots, \Mat{h}_{e,\lvert e \rvert}\right) = \frac{\partial_v g\left(\Mat{z}_{e, 1}, \cdots, \Mat{z}_{e, \lvert e \rvert}\right)}{\partial \Mat{z}_{e, v}} \Big\lvert_{\Mat{z}_{e,i} = \Mat{h}_{e,i}}$ \pan{I think this notation may have some issues.}.
% To reveal more properties of $g(\cdot)$, we list the following formal definitions:

% \begin{definition} \label{def:permutation}
% Let $\pi: [k] \rightarrow [k]$ be an automorphism, then permutation matrix  is defined as $\Mat{P}_{\pi}$ who has value one at entries $(i, \pi(i)), \forall i \in [k]$ while taking zero at any other positions.
% A permutation group $\Grp{P}_k$ \pan{revise to $\Pi[k]$} is defined as a set which collects all of such $\Mat{P}_\pi$.
% \end{definition}

% \begin{definition} \label{def:permutation_ivariant} (Permutation Invariance)
% Let $f: \real^k \rightarrow \real$ be a permutation-invariant function, then $\forall \Mat{P} \in \Grp{P}_k$, $f(\Mat{P} \Mat{x}) = f(\Mat{x})$ for all $\Mat{x} \in \real^k$.
% \end{definition}

% \begin{definition} \label{def:permutation_equivariant} (Permutation Equivariance)
% Let $f: \real^k \rightarrow \real^k$ be a permutation-equivariant function, then $\forall \Mat{P} \in \Grp{P}_k$, $f(\Mat{P} \Mat{x}) = \Mat{P} f(\Mat{x})$ for all $\Mat{x} \in \real^k$.
% \end{definition}

% We note that potential function $g(\cdot)$ should be permutation-invariant since row permutation of the edge feature matrix results in an equivalent class. \pan{This may be more natural put with g definition together.}
% No matter in which order we arrange data inside $\Mat{H}_e$, $g(\cdot)$ should give the identical potential value. 



% \begin{itemize}
%     \item Attributed hypergraphs: $\gG=(V,E,X)$.  $X\in\mathbb{R}^{|V|\times m}$. $x_v$ denotes the attributes for node $v$. A hyperedge $e\in E$ is a subset of nodes $e=\{v_1^{(e)},...,v_{|e|}^{(e)}\}\subseteq V$ where $|e|$ is the hyperedge size. %(Start from 1-dim case for simplicity).
    
%     \item Define node-diffused matrix $H\in\mathbb{R}^{|V|\times m}$ where $\Mat{h}_v$ denotes the row for node $v$. Given $e\in E$, we use notation bar-subscript $\bar{h}_e\in \mathbb{R}^{|e|\times m}$ to denote  concatenation $\oplus_{v\in e} \Mat{h}_v$ whose $i$th block is $\Mat{h}_{v_i^{(e)}}$. We also use the subscript without bar $q_e\in \mathbb{R}^{|e|\times m}$ to denote concatenation of $\oplus_{v\in e} q_{e,v}$ where $q_{e,v}\in \mathbb{R}^{m}$ which is a representation for a hyperedge-node pair.
    
    
%     %= (\Mat{h}_{v_1^{(e)}},...,\Mat{h}_{v_|e|^{(e)}})$. %where $z_i = \Mat{h}_{v_i^{(e)}}$ for $i\in[e]$.
    
%     \item Node potential: $f_v(\cdot ;x_v)$: $\mathbb{R}^{m} \rightarrow \mathbb{R}.$ %We assume that $f_v = f_{u}$ if the node degree $d_v = d_{u'}$.
%     \item hyperedge potential: $g_e(\cdot): \mathbb{R}^{|e|\times m}\times \mathbb{R}$. %We
%     %Denote $\bar{z} =(z_1,z_2^{(e)},...,z_|e|^{(e)})$ where $z_{i}^{(e)}$ is the block of the input vector $\bar{z}_e$ associated with node $v_{i}^{(e)}$.
    
%     \item In hypergraphs, we often do not have node identities so $f_v=f_u$ if $d_v= d_{u}$. We also assume that $g_e = g_{e'}$ if $|e| = |e'|$ and $g_{e}$ is permutation invariant: $g_e(\bar{h}_e) = g_e(\bar{h}'_e)$ if $\{\Mat{h}_v|v\in e\}=\{\Mat{h}_v'|v\in e\}$. As the information of node degrees and hyperedge sizes are clear, we simply use $f$ and $g$ to uniformly denote node potentials and hyperedge potentials respectively.% by removing the subscripts for simplicity.
    
    
%     %where $Z_e\in \mathbb{R}^{|e|\times m}$ and $P$ is a $|e|$-by-$|e|$ permutation matrix. As the information of node degrees and hyperedge sizes are clear, we simply use $f$ and $g$ by removing the subscripts for simplicity.
%     %if $\{z_1^{(e)},z_2^{(e)},...,z_{|e|}^{(e)}\}=\{z_1'^{(e)},z_2'^{(e)},...,z_{|e|}'^{(e)}\}$. %In the following, for simplicity, our discussion focus on uniform hypergraphs, though experiments may have non-uniform hypergraphs. So we denote $g_e = g$ for simplicity.
% \end{itemize}

% \paragraph{Hypergraph Convolutional Networks}
% Graph neural networks (GNN) are broadly adopted for learning problems on graphs.
% Recent works \cite{feng2019hypergraph, bai2021hypergraph, yadati2019hypergcn, dong2020hnhn, huang2021unignn} have generalized various GNNs for ordinary graphs onto hypergraphs.
% Nevertheless, most of existing hypergraph convolution are based on clique expansion propagation with degree normalization and nonlinear transformation.
% Taking HGNN \cite{feng2019hypergraph} for an example, it has the following node-wise update formula for each layer:
% \begin{align} \label{eqn:hgnn}
%     \Mat{h}_v^{(t+1)} = \sigma\left( \frac{1}{\sqrt{d_v}} \sum_{e: v \in e} \frac{1}{\lvert e \rvert} \sum_{u: u \in e} \frac{\Mat{h}_u^{(t)}}{\sqrt{d_u}} \Mat{\Theta}^{(t)} + \Mat{b}^{(t)} \right),
% \end{align}
% where $\Mat{h}_v^{(t)}$ denotes the features of node $v$ at the $t$-th layer, $d_v$ denotes the degree of node $v$, $\sigma$ is a non-linear activation, and $\Mat{\Theta}^{(t)}, \Mat{b}^{(t)}$ are parameters of linear transformation and bias, respectively.
% We argue that each layer's update (Eq. \ref{eqn:hgnn}) can be regarded as an optimization step of a special case of objective Eq. \ref{eqn:diffusion}.
% We show this by letting $g(\Mat{Z}_e) = \sum_{(v, u) \in e} \lVert \Mat{h}_v^{(e)}/\sqrt{d_v} - \Mat{h}_u^{(e)}/\sqrt{d_u} \rVert_2^2$ and $f(\Mat{h}_v; \Mat{x}_v) = 0$.
% Since $g$ is strongly convex, we can reach optimum by gradient descent. And the gradient step will coincide with Eq. \ref{eqn:hgnn} in form.
% \textcolor{red}{need a derivation and correction later.}
% \textcolor{red}{add AllSet?}

% \paragraph{Nonlinear Hypergraph Diffusion (HyperND)}




==> arxiv/section_files/003-model.tex <==
 % \vspace{-2mm}
\section{Neural Equivariant Diffusion Operators and \proj} \label{sec:model}
 % \vspace{-1mm}
Previous design of hyperedge potential functions is tricky. Early works adopted clique or star expansion by reducing hyperedges into (weighted) edges~\cite{zhou2007learning,agarwal2006higher,li2017inhomogeneous} and further used traditional graph methods. Later, researchers proved that those hyperedge reduction techniques cannot well represent higher-order relations~\cite{li2017inhomogeneous,chien2019hs}. Therefore, Lov\'{a}sz extensions of set-based cut-cost functions on hyperedges have been proposed recently and used as the potential functions~\cite{hein2013total,li2018submodular,li2020quadratic,takai2020hypergraph,liu2021strongly,fountoulakis2021local,yoshida2019cheeger}. However, designing those set-based cut cost is practically hard and needs a lot of trials and errors. Other types of handcrafted hyperedge potentials to model information propagation can also be found in~\cite{neuhauser2022consensus,neuhauser2021opinion}. %which again are handcrafted and heavily based on heuristics and evaluation performance. 

%~\cite{li2018submodular}, and  Lov\'{a}sz extensions of those set functions are further
%Hypergraph diffusion has been widely used in applications. However, heuristic design of the potential functions requires significant insights into the applications. For example, early works often adopted clique or star expansion by reducing hypergraphs into graphs~\cite{zhou2007learning,star}. Later, researchers found that such graph reduction techniques often generate huge distortion of hypergraph cut functions ~\cite{li2017inhomogeneous}, so total variation was proposed and behaved well in the case with large hyperedges~\cite{hein2013total,zhang2017re}. Recently, to model complex higher-order patterns, e.g., the hierarchy of foodweb networks~\cite{}, hyperedges have been associated with set functions and Lov\'{a}sz extension-based potentials have found greatly useful~\cite{}. Particularly for node classification tasks, as opposed to the edge case that connects two nodes from either the same or different categories, hyperedges may consist of nodes from multiple categories with various ratios, which makes handcrafting potentials far more complicated.    

Our idea uses data-driven approaches to model such potentials, which naturally brings us to HNNs. On one hand, we expect to leverage the extreme expressive power of NNs to learn the desired hypergraph diffusion automatically from the data. On the other hand, we are interested in having novel hypergraph NN (HNN) architectures inspired by traditional hypergraph diffusion solvers. 

To achieve the goals, next, we show by the gradient descent algorithm (GD) or alternating direction method of multipliers (ADMM)~\cite{boyd2011distributed}, solving objective Eq.~\ref{eqn:diffusion} amounts to iteratively applying some hyperedge diffusion operators. Parameterizing such operators using NNs by each step can unfold hypergraph diffusion into an HNN. We make the key observation that the diffusion operators are inherently \textit{permutation-equivariant}. To universally represent them, we propose a standard form to design  equivariant NN-based operators and use it to build \proj via an efficient implementation. %By repeating this computational unit, we construct our Equivariant Diffusion-based HNN, dubbed \proj.

%To the best of our knowledge, \proj is the first one to adopt equivariant hyperedge-processing architecture. All previous HGNN models adopt permutation-invariant hyperedge operation, which limits their power to represent general hypergraph diffusion. Although a very recent work proposed to view each hyperedge as a multi-set so building multi-set equivariant operator is a natural thought~\cite{chien2021you}, no specific equivariant achitecture was proposed albeit universally representable as \proj guarantees. As a by product, our representation theory complements the previous studies on set-function representation~\cite{segol2020universal} and~\cite{zaheer2017deepset}. Our proof technique avoids using equivariant polynomial approximation and thus allows a precise representation of continuous equivariant set functions by composing a continuous function and the sum of another continuous function on each set entry.         



%Theoretically, 

%hypergraph diffusion process.   

%Specifically, given a hypergraph with initial values defined on the nodes, design potential functions that characterize higher-order relations reflected by the hyperedges. Then, diffuse the node values across hyperedges to decrease the total potential of the hypergraph. The convergent values that achieve minimal total potential encode all the higher-order relations and can be further used to make prediction. Hypergraph diffusion is significant due to the transparency of the algorithms and has found applications in  clustering~\cite{zhou2007learning,li2017inhomogeneous,li2018submodular}, semi-supervised learning~\cite{hein2013total,zhang2017re,tudisco2021nonlinear}, ranking aggregation~\cite{li2017inhomogeneous,chitra2019random}, network analysis~\cite{li2018quadratic,liu2021strongly,fountoulakis2021local,takai2020hypergraph}, signal denoising~\cite{zhang2019introducing,schaub2021signal} and image processing~\cite{komodakis2009beyond,werner2008high}.

%However, designing good potential functions often requires significant insights into the applications. Early works often adopted clique or star expansion by reducing hypergraphs into graphs~\cite{zhou2007learning,star,li2017inhomogeneous} and adopt  graph potentials. Later, researchers proved that those graph reduction techniques can hardly well represent higher-order relations~\cite{li2017inhomogeneous,chien2019}. Therefore, recently, set-based costs on hyperedges have been proposed~\cite{}, and  Lov\'{a}sz extension of those set functions can be used as the potential functions~\cite{}. However, how to design those set-based costs are practically hard and need a lot of trials and errors. Other types of hyperedge potentials to model the divergence of node values and information propagation can be found in~\cite{}, which are all handcrafted and heavily based on heuristics. 

% We show that hypergraph diffusion operators are inherently \textit{permutation-equivariant}.


% the traditional solvers of Eq.~\eqref{eqn:diffusion} based on the gradient descent algorithm (GD) and alternating direction method of multipliers (ADMM). We observe that 

% show by using gradient descent algorithm or Douglas-Rachford splitting algorithm, solving objective Eq. \ref{eqn:diffusion} amounts to iteratively applying hypergraph diffusion operators.
% Parameterizing such diffusion operators using neural networks by each step can unfold the optimization algorithm to be a Hypergraph Neural Network (HGNN).  \pan{Inspire our work}
% We show that hypergraph diffusion operators are inherently \textit{permutation-equivariant}.
% To universally represent them, we propose a standard form of equivariant mapping and follow this form to design our permutation-equivariant neural networks.
% By repeating this computational unit, we construct our Equivariant Diffusion-based Hypergraph Neural Network, dubbed ED-HGNN.

% Therefore, the key motivation of our approaches is whether we may use data-driven approaches, neural networks specifically, to automatically learn the desired hypergraph diffusion. On the other hand, we are also interested in having novel hypergraph neural network architectures inspired by traditional hypergraph diffusion solvers. 

% %inspire the design of hypergraph neural network models?


% %\pan{Claim how to implement equi hyperedge operator is non-trivial. Previous works are regular. Moreover, standard model, do not need to worry this.}


% We are interested in supervised representation learning on hypergraphs.
% In this section, we show by using gradient descent algorithm or Douglas-Rachford splitting algorithm, solving objective Eq. \ref{eqn:diffusion} amounts to iteratively applying hypergraph diffusion operators.
% Parameterizing such diffusion operators using neural networks by each step can unfold the optimization algorithm to be a Hypergraph Neural Network (HGNN).  \pan{Inspire our work}
% We show that hypergraph diffusion operators are inherently \textit{permutation-equivariant}.
% To universally represent them, we propose a standard form of equivariant mapping and follow this form to design our permutation-equivariant neural networks.
% By repeating this computational unit, we construct our Equivariant Diffusion-based Hypergraph Neural Network, dubbed ED-HGNN.
\vspace{-2mm}
\subsection{Emerging Equivariance in Hypergraph Diffusion}
\label{sec:emerge_equivariance}
\vspace{-1mm}
We start with discussing the traditional solvers for Eq.~\ref{eqn:diffusion}. If $f$ and $g$ are both differentiable, one straightforward optimization approach is to adopt gradient descent. The node-wise update of each iteration can be formulated as below:
\begin{align} \label{eqn:gd}
    \Mat{h}_v^{(t+1)} \leftarrow \Mat{h}_v^{(t)} - \eta (\nabla f(\Mat{h}_v^{(t)}; \Mat{x}_v) + \sum_{e: v\in e} [\nabla g(\Mat{H}_e^{(t)})]_v), \quad \text{for}\; v\in \Set{V},
\end{align}
where $[\nabla g(\Mat{H}_e)]_v$ denotes the gradient w.r.t. $\Mat{h}_v$ for $v\in e$. We use the supscript $t$ to denote the number of the current iteration, $\Mat{h}_v^{(0)} = \Mat{x}_v$ is the initial features, and $\eta$ is known as the step size.

For general $f$ and $g$, we may adopt ADMM~\cite{boyd2011distributed}: For each $e\in\Set{E}$, we introduce an auxiliary variable $\Mat{Q}_e = \begin{bmatrix} \Mat{q}_{e,1} & \cdots & \Mat{q}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert}$. We initialize $\Mat{h}_v^{(0)}=\Mat{x}_v$ and $\Mat{Q}_e^{(0)}=\Mat{H}_e^{(0)}$. And then, iterate 
%We introduce $\Mat{Q}_e = \Mat{S}_e^{(t)} + \Mat{R}_e^{(t+1)}$ as an intermediate auxiliary variable. 
%This problem can be solved via ADMM: Introducing $\Mat{Q}_e = \Mat{S}_e^{(t)} + \Mat{R}_e^{(t+1)}$ an intermediate variable,
\begin{align} \label{eqn:admm-q}
    \Mat{Q}_e^{(t+1)} &\leftarrow  \prox_{\eta g}(2\Mat{H}_e^{(t)} - \Mat{Q}_e^{(t)}) - \Mat{H}_e^{(t)} + \Mat{Q}_e^{(t)}, \quad \text{for}\; e\in \Set{E}, \\ \label{eqn:admm-h}
    \Mat{h}_v^{(t+1)} &\leftarrow  
    \prox_{\eta f(\cdot;\Mat{x}_v)/d_v}(\sum_{e:v\in e}\Mat{q}_{e,v}^{(t+1)}/d_v), \quad \text{for}\; v\in \Set{V},
\end{align}
where $\prox_{\psi}(\Mat{h}) \triangleq \arg\min_{\Mat{z}} \psi(\Mat{z}) + \frac{1}{2}\|\Mat{z}-\Mat{h}\|_2^2$ is the proximal operator. The detailed derivation can be found in Appendix~\ref{sec:ADMM-derive}. Note that previous hypergraph diffusion algorithms based on primal-dual hybrid gradient descent~\cite{hein2013total} or alternative projection~\cite{li2018revisiting,li2020quadratic} for some specific $f$ and $g$ are close related to the above general form given by ADMM. 
The operator $\prox_{\psi}(\cdot)$ has nice  properties as reviewed in Proposition~\ref{prop:prox}, which enables the possibility of NN-based approximation even when $f$ and $g$ are not differentiable. One noted non-differentiable example is the LEC case when $g(\Mat{H}_e)=\langle \Mat{y}, \varsigma(\Mat{H}_e) \rangle^p$. %However, previous heuristics of $g$ expect divergence to the mean are convex.
\begin{proposition}[\cite{parikh2014proximal,polson2015proximal}]\label{prop:prox}
If $\psi(\cdot):\mathbb{R}^K\rightarrow \mathbb{R}$ is a lower semi-continuous convex function, then $\prox_{\psi}(\cdot)$ is 1-Lipschitz continuous. 
\end{proposition}



The node-side operations, gradient $\nabla f(\cdot;\Mat{x}_v)$ and proximal gradient $\prox_{\eta f(\cdot;\Mat{x}_v)}(\cdot)$ are relatively easy to model, while the operations on hyperedges are more complicated. We name gradient $\nabla g(\cdot):\mathbb{R}^{|e|}\rightarrow \mathbb{R}^{|e|}$ and proximal gradient $\prox_{\eta g}(\cdot):\mathbb{R}^{|e|}\rightarrow \mathbb{R}^{|e|}$ as  \textit{hyperedge diffusion operators}, since they summarize the collection of node features inside a hyperedge and dispatch the aggregated information to interior nodes individually. %These hyperedge diffusion operators can be intuitively interpreted as a (one-hop) information fusion among nodes connected by some hyperedge.
Next, we reveal one crucial property of those hyperedge diffusion operators by the following propostion (see the proof in Appendix~\ref{sec:proof-equi-op}):
\begin{proposition} \label{prop:equivariant_op}
 Given any permutation-invariant hyperedge potential function $g(\cdot)$, hyperedge diffusion operators $\prox_{\eta g}(\cdot)$ and $\nabla g(\cdot)$  are permutation equivariant.
\end{proposition}
%We provide the proof of Proposition \ref{prop:equivariant_op} in Appendix~\ref{sec:proof-equi-op}. 
It states that an permutation invariant hyperedge potential leads to an operator that should process different nodes in a permutation-equivariant way. 






% We initialize $\Mat{h}_v^{(0)}=\Mat{x}_v$ and $\Mat{Q}_e^{(0)}=\Mat{H}_e^{(0)}$. 

% . Then, 


% A common strategy to solve Eq. \ref{eqn:alm} is to minimize $\Mat{H}_e$ and $\Mat{R}_e$ alternatively, which induces a form of Alternating Direction Method of Multipliers (ADMM) as below \pan{reference, node degree was not defined.}:
% \begin{align} \label{eqn:admm}
%     \Mat{Q}_e^{(t+1)} &\leftarrow  \prox_{g,\frac{1}{\lambda}}(2\Mat{H}_e^{(t)} - \Mat{Q}_e^{(t)}) - \Mat{H}_e^{(t)} + \Mat{Q}_e^{(t)} \\
%     \Mat{h}_v^{(t+1)} &\leftarrow  
%     \prox_{\frac{1}{f,\lambda d_v}}\left(\frac{1}{d_v}\sum_{e:e\in v}\Mat{q}_{e,v}^{(t)};\pan{x_v}\right),
% \end{align}
% where we introduce $\Mat{Q}_e = \Mat{S}_e^{(t)} + \Mat{R}_e^{(t+1)} = \begin{bmatrix} \Mat{q}_{e,1} & \cdots & \Mat{q}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert \times d} $ as an intermediate auxiliary variable. The detailed derivation can be found in the \textcolor{red}{Appendix}.





% %$\Mat{R}_e = \Mat{H}_e$ for every $e \in \Set{E}$.

% not necessarily differentiable (e.g., $g$ penalizes the maximal element), which hinders us to reach the minimum via simple gradient descent.
% When $g(\Mat{H}_e)$ is non-differentiable, we solve this problem using Augmented Lagrangian Method (ALM) \pan{reference}.
% We first introduce dual variables $\Mat{S}_e \in \real^{\lvert e \rvert \times d}$ and duplicate the hyperedge features $\Mat{H}_e$ into $\Mat{R}_e = \begin{bmatrix} \Mat{r}_{e,1} & \cdots & \Mat{r}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert \times d}$ such that $\Mat{R}_e = \Mat{H}_e$ for every $e \in \Set{E}$.
% Then by ALM, our primal problem can be derived as:
% \begin{align} \label{eqn:alm}
% \pan{\max_{S_e}\min_{R_e,H}}\sum_{v\in \Set{V}} f(\Mat{h}_v; \Mat{x}_v) + \sum_{e\in \Set{E}} g(\Mat{R}_e) +  \frac{\lambda}{2}\sum_{e\in \Set{E}}\lVert \Mat{R}_e - \Mat{H}_e + \Mat{S}_e\ \Vert_2^2 - \frac{\lambda}{2}\sum_{e\in \Set{E}} \lVert \Mat{S}_e \rVert^2.
% \end{align}
% A common strategy to solve Eq. \ref{eqn:alm} is to minimize $\Mat{H}_e$ and $\Mat{R}_e$ alternatively, which induces a form of Alternating Direction Method of Multipliers (ADMM) as below \pan{reference, node degree was not defined.}:
% \begin{align} \label{eqn:admm}
%     \Mat{Q}_e^{(t+1)} &\leftarrow  \prox_{g,\frac{1}{\lambda}}(2\Mat{H}_e^{(t)} - \Mat{Q}_e^{(t)}) - \Mat{H}_e^{(t)} + \Mat{Q}_e^{(t)} \\
%     \Mat{h}_v^{(t+1)} &\leftarrow  
%     \prox_{\frac{1}{f,\lambda d_v}}\left(\frac{1}{d_v}\sum_{e:e\in v}\Mat{q}_{e,v}^{(t)};\pan{x_v}\right),
% \end{align}
% where we introduce $\Mat{Q}_e = \Mat{S}_e^{(t)} + \Mat{R}_e^{(t+1)} = \begin{bmatrix} \Mat{q}_{e,1} & \cdots & \Mat{q}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert \times d} $ as an intermediate auxiliary variable. The detailed derivation can be found in the \textcolor{red}{Appendix}.

% We name gradient $\nabla_{v} g(\cdot)$ and proximal gradient $\prox_{\frac{1}{\lambda} g}(\cdot)$ as \textit{hypergraph diffusion operator} \pan{hyperedge diffusion operator}, since they summarize the collection of node features inside a hyperedge and dispatch the aggregated information to interior nodes individually.
% These hypergraph diffusion operators can be intuitively interpreted as a (one-hop) information fusion among nodes connected by some hyperedge.
% We reveal one crucial property of hypergraph diffusion operators by the following propostion:
% \begin{proposition} \label{prop:equivariant_op}
% Hypergraph diffusion operators $\prox_{\frac{1}{\lambda},g}(\Mat{H}_e)$ (\pan{Use the full}) and $\nabla_v g(\Mat{H}_e)$ \pan{I do not think this is an okay notation. We need to consider defining $\nabla g() = [\nabla_v g]_{v\in e}$} are permutation-equivariant operators with respect to node features $\Mat{h}_v$ for any potential function $g(\cdot)$.
% \end{proposition}
% We provide the proof of Proposition \ref{prop:equivariant_op} in \textcolor{red}{Appendix}. It states that hypergraph diffusion operator $\nabla_v g(\Mat{H}_e)$ and $\prox_{\frac{1}{\lambda},g}(\Mat{H}_e)$ should not only aggregate features regardless of the node order, but should also pass distinctive messages to different nodes.
% This means the operator $\prox_{\frac{1}{\lambda},g}(\Mat{H}_e)$ and $\nabla_v g(\Mat{H}_e)$ are both equivariant set functions.

% After reviewing different forms of hypergraph diffusion, now we assume both node-wise and hyperedge potential functions are unknown.

\subsection{Building Equivariant Hyperedge Diffusion Operators}
\vspace{-1mm}
\label{sec:build_equivariance}
%Hyperedge diffusion operators are essentially permutation-equivariant operators as shown above. 
To model permutation-equivariant diffusion operators, we may resort to previous studies on NN architectures to represent equivariant multi-set functions~\cite{zaheer2017deepset,maron2018invariant,segol2020universal}. However, there are still some gaps when we apply their approaches in the hypergraph setting. In practice, these works focus on the case with separate multi-sets, such as prediction over  separate sets of images or 3-D points, while hypergraphs contain a large number of hyperedges that are overlapped. Moveover, as  hyperedges could be large and irregular in practice, how to build scalable equivariant NN architectures on hyperedges is challenging. Note that although graphs also have coupled  edges, edges in graphs are of regular size two. Building equivariant edge operation in graphs is often much less crucial or challenging than that in hypergraphs. %much more  challenging than that in traditional GNN design. %In theory, although previous works proved the universal approximation of their proposed architecture~\cite{segol2020universal}, the construction uses the universality of equivariant polynomials as a bridge, which induces two issues of the obtained conclusion. First, the theory does not provide a precise representation of a permutation-equivariant function. Second, the needed latent dimension is exponential w.r.t. the input feature dimension, which conflicts with the scalability requirement in hypergraph models.

%Specifically, for an equivariant function $\psi(\cdot):\mathbb{R}^{K\times F} \rightarrow \mathbb{R}^{K\times F}$, they suggest 
% \begin{align}\label{eqn:equivariant}
%     \psi(\cdot) = L_m\circ \sigma \circ L_{m-1}\circ  \cdots \circ \sigma \circ L_{1},\, \text{where}\, L_i(\Mat{Z})= \Mat{Z}\Mat{W}_i^{(1)} +  \mathbf{1}\mathbf{1}^T\Mat{Z}\Mat{W}_i^{(2)} + \mathbf{1}\Mat{W}_i^{(3)T},
% \end{align}
% $\sigma$ is entry-wise nonlinear activation. 
% $\Mat{W}_i^{(j)}\in\mathbb{R}^{F\times F}$ for $j\in\{1,2\}$ and $\Mat{W}_i^{(3)}\in\mathbb{R}^{F}$ are parameters

% %$\Mat{W}_i^{(j)}\in\mathbb{R}^{F_{\text{in}}^{(i)}\times F_{\text{out}}^{(i)}}$ for $j\in\{1,2\}$ and $\Mat{W}_i^{(3)}\in\mathbb{R}^{F_{\text{out}}^{(i)}}$ are parameters where $F_{\text{in}}^{(1)}=F_{\text{out}}^{(m)}=F$ and $F_{\text{in}}^{(i+1)}=F_{\text{out}}^{(i)}$ for $i\in 1,2,...,m-1$.

% However, there are still some gaps when applying Eq.~\ref{eqn:equivariant} to the hypergraph setting. Practically, $\psi$ is used to make prediction for decoupled multi-sets, such as prediction over each separate collection of images or 3-D points, while hypergraphs contain a large number of coupled multi-sets. As a hypergraph may contain thousands of hyperedges and a node may appear in hundreds of hyperedges, how to build scalable equivariant operators for all hyperedges is crucial. Note that graphs also couple thousands of edges while edges are of regular size two so building equivariant edge operation is not that crucial and challenging in traditional GNN design. In theory, although previous work proved the universal approximation of the architecture Eq.~\ref{eqn:equivariant}~\cite{segol2020universal}, the construction uses the universality of equivariant polynomials as a bridge, which induces two issues. First, the conclusion may not allow a precise representation of $\psi(\cdot)$. Second, the needed latent dimension is exponential w.r.t. the dimensions $K$ and $F$, which conflicts with the scalability requirement in hypergraph models. 

Our design is built upon the following Theorem~\ref{thm:equivarnt_form_1dim}. We leave the proof in Appendix~\ref{sec:proof-equi-1dim}. %and \ref{sec:proof-equi-Fdim}.

%As shown below, we formally specifies a general form that equivariant function must have:
\begin{theorem} \label{thm:equivarnt_form_1dim}
 $\psi(\cdot): [0,1]^K \rightarrow \mathbb{R}^K$ is a continuous permutation-equivariant function, if and only if it can be represented as  $[\psi(\Mat{Z})]_i = \rho(\Mat{z}_i, \sum_{j=1}^K \phi(\Mat{z}_j))$, $i\in [K]$ for any $\Mat{Z} = \begin{bmatrix} ...,\Mat{z}_i,...\end{bmatrix}^\top\in [0,1]^{K}$, 
% \begin{align}
%     \psi(x_1, x_2,\cdots,x_k) =
%      \begin{bmatrix} 
%     \rho(x_1, \sum_{i=1}^K \phi(x_i)) \\
%     \rho(x_2, \sum_{i=1}^K \phi(x_i)) \\
%     \vdots\\
%     \rho(x_3, \sum_{i=1}^K \phi(x_i)) \\
%     \end{bmatrix}
% \end{align}
where $\rho: \real^{K'} \rightarrow \real$, $\phi: \real \rightarrow \real^{K'-1}$ are two continuous functions, and $K'$ could be as small as $K$. 
\end{theorem}  \vspace{-1mm}

Theorem~\ref{thm:equivarnt_form_1dim} indicates that any continuous permutation-equivariant function where each entry of the input $\Mat{Z}$ has 1-dim feature channel can be precisely represented as a composition of a continuous function $\rho$ and the sum of another continuous function $\phi$ on each input entry. This result generalizes the representation of permutation-invariant functions by $\rho(\sum_{i=1}^K\phi(\Mat{z}_i))$ in~\cite{zaheer2017deepset} to the equivariant case. An architecture with a similar spirit was proposed in~\cite{segol2020universal} for equivariant set function representations. However, %in practice, the work targeted at a single set representation instead of hypergraph with coupled sets~\cite{segol2020universal}. 
in theory, their proof used the universality of equivariant polynomials as a bridge so their construction $\hat{\psi}(\Mat{Z})$ only allows approximation, i.e., small $\|\psi(\Mat{Z})-\hat{\psi}(\Mat{Z})\|$ instead of precise representation in Theorem~\ref{thm:equivarnt_form_1dim}. Note that, in practice, $\rho$ and $\phi$ often need to be further approximated by NNs. So, the precise representaiton in Theorem~\ref{thm:equivarnt_form_1dim} has more values of its theoretical implication than its practical usage given the results in~\cite{segol2020universal}. %Also, $K'\geq K$ is tight by generalizing the proof for invariant set function representation~\cite{wagstaff2019limitations}. 



% More practical significance can be achieved when we consider multiple feature dimensions:
% \begin{theorem} \label{thm:equivarnt_form_Fdim}
%  $\psi(\cdot): [0,1]^{K\times F} \rightarrow \mathbb{R}^{K}$ is a  permutation-equivariant function, if and only if it can be represented as  $[\psi(\Mat{Z})]_i = \rho(\Mat{z}_i, \sum_{j=1}^K \phi(\Mat{z}_j))$, $i\in [K]$, for any $\Mat{Z} = \begin{bmatrix} ...,\Mat{z}_i,...\end{bmatrix}^\top\in [0,1]^{K\times F}$.
% % \begin{align}
% %     \psi(x_1, x_2,\cdots,x_k) =
% %      \begin{bmatrix} 
% %     \rho(x_1, \sum_{i=1}^K \phi(x_i)) \\
% %     \rho(x_2, \sum_{i=1}^K \phi(x_i)) \\
% %     \vdots\\
% %     \rho(x_3, \sum_{i=1}^K \phi(x_i)) \\
% %     \end{bmatrix}
% % \end{align}
% where $\rho: \real^{K'+1} \rightarrow \real$, $\phi: \real^F \rightarrow \real^{K'}$ are two  functions, and $K'$ could be as small as $K^4F^2$. 
% \end{theorem}
% The construction in~\cite{segol2020universal} that adopts equivariant polynomials needs the latent dimension to representation each entry $\phi(\Mat{z}_i)$ to be in the order of $K'\geq {K+F \choose F}$ to achieve even just approximate representations, which is practically infeasible. Note that $K^4F^2$ in Theorem~\ref{thm:equivarnt_form_Fdim} is not still tight.

The above theoretical observation inspires the design of equivariant hyperedge diffusion operators. Specifically, for an operator $\hat{\psi}(\cdot):\mathbb{R}^{|e|}\rightarrow \mathbb{R}^{|e|}$ that may denote either gradient $\nabla g(\cdot)$ or proximal gradient $\prox_{\eta g}(\cdot)$ for each hyperedge $e$, we may parameterize it as: \vspace{-1mm}
\begin{align}\label{eq:equi-form}
    [\hat{\psi}(\Mat{H}_e)]_v=\hat{\rho}(\Mat{h}_v, \sum_{u\in e} \hat{\phi}(\Mat{h}_u)),\,\text{for $v\in e$,}\, \text{where $\hat{\rho},\,\hat{\phi}$ are multi-layer perceptions (MLPs). }
\end{align}
Intuitively, the inner sum collects the $\hat{\phi}$-encoding node features within a hyperedge and then $\hat{\rho}$ combines the collection with the features from each node further to perform separate operation. 

The implementation of the above $\hat{\psi}$ is not trivial. A naive implementation is to generate an auxillary node to representation each $(v,e)$-pair for  $v\in\Set{V}$ and $e\in\Set{E}$ and learn its representation as adopted in  \cite{yadati2020neural,arya2020hypersage,yang2020hypergraph}. However, this may substantially increase the model complexity. 

Our implementation is built upon the widely-used bipartite representations~\cite{dong2020hnhn,huang2021unignn,chien2021you} (or  star expansion~\cite{zien1999multilevel,agarwal2006higher}, equivalently) of hypergraphs paired with the standard message passing NN (MPNN)~\cite{gilmer2017neural} that can be efficiently implemented via  commonly-used GNN platforms~\cite{FeyPyG,wang2019dgl}. Specifically, we build a bipartite graph $\Set{\bar{G}} = (\Set{\bar{V}}, \Set{\bar{E}})$. The node set $\Set{\bar{V}}$ contains two parts $\Set{V}\cup\Set{V_{\Set{E}}}$ where $\Set{V}$ is the original node set while $\Set{V_{\Set{E}}}$ contains nodes that correspond to original hyperedges $e\in\Set{E}$. Then, add an edge between $v\in\Set{V}$ and $e\in\Set{E}$ if $v\in e$. The model \textbf{\proj} is implemented by following \textbf{Algorithm 1}.
% For different 
% \begin{enumerate}[leftmargin=4mm]
%     \item Designing the messages from $\Set{V}$ to $\Set{E}$:\quad  $\Mat{m}_{u\rightarrow e}^{(t)} = \hat{\phi}(\Mat{h}_u^{(t)})$, for all $u\in\Set{V}$. 
%     \item Sum $\Set{V}\rightarrow \Set{E}$ messages over hyperedges $\Mat{m}_{e}^{(t)} = \sum_{u\in e} \Mat{m}_{u\rightarrow e}^{(t)}$, for all $e\in\Set{E}$.
%     \item Broadcast $\Mat{m}_{e}^{(t)}$ and design the messages from $\Set{E}$ to $\Set{V}$: $\Mat{m}_{e\rightarrow v}^{(t)} = \hat{\rho}(\Mat{h}_v^{(t)},\Mat{m}_{e}^{(t)})$, for all $v\in e$.% and $e\in\Set{E}$. 
%     \item Update $\Mat{h}_v^{(t+1)}= \hat{\varphi}(\Mat{h}_v^{(t)}, \sum_{e:u\in e}\Mat{m}_{e\rightarrow u}^{(t)}, \Mat{x}_v, d_v)$, for all $v\in\Set{V}$,  where $\hat{\varphi}$ is another MLP. 
% \end{enumerate}


\begin{table}[t]
\begin{tabular}{l}
\hline 
\textbf{Algorithm 1: \proj} \\
\hline
\textbf{Initialization:} $\Mat{H}^{(0)}=\Mat{X}$ \textbf{and three MLPs $\hat{\phi},\,\hat{\rho},\, \hat{\varphi}$ (shared across $L$ layers).} \\
%\textbf{Output:} $\Mat{H}^{(L)}$.\\
\textbf{For} $t=0,1,2,...,L-1$, \textbf{do:}\\
1. Designing the messages from $\Set{V}$ to $\Set{E}$:\quad  $\Mat{m}_{u\rightarrow e}^{(t)} = \hat{\phi}(\Mat{h}_u^{(t)})$, for all $u\in\Set{V}$. \\ 
2. Sum $\Set{V}\rightarrow \Set{E}$ messages over hyperedges $\Mat{m}_{e}^{(t)} = \sum_{u\in e} \Mat{m}_{u\rightarrow e}^{(t)}$, for all $e\in\Set{E}$.\\
3. Broadcast $\Mat{m}_{e}^{(t)}$ and design the messages from $\Set{E}$ to $\Set{V}$: $\Mat{m}_{e\rightarrow v}^{(t)} = \hat{\rho}(\Mat{h}_v^{(t)},\Mat{m}_{e}^{(t)})$, for all $v\in e$. \\% and $e\in\Set{E}$.\\
4. Update $\Mat{h}_v^{(t+1)}= \hat{\varphi}(\Mat{h}_v^{(t)}, \sum_{e:u\in e}\Mat{m}_{e\rightarrow u}^{(t)}, \Mat{x}_v, d_v)$, for all $v\in\Set{V}$. \\
\hline 
\end{tabular}
\vspace{-0.4cm}
\end{table}

The equivariant diffusion operator $\hat{\psi}$ can be constructed via steps 1-3. The last step is to update the node features to accomplish the first two terms in Eq.~\ref{eqn:gd} or the ADMM update Eq.~\ref{eqn:admm-h}. The initial attributes $\Mat{x}_v$ and node degrees are included to match the diffusion algorithm by design. As the diffusion operators are shared across iterations, \proj shares parameters across layers. Now, we summarize the joint contribution of our theory and  efficient implementation as follows.

\begin{proposition}\label{prop:universal}
MPNNs on bipartite representations (or star expansions) of hypergraphs are  expressive enough to learn any continuous diffusion operators induced by invariant hyperedge potentials.   
\end{proposition}

%According to Proposition~\ref{prop:prox}, any lower semi-continuous convex function $g$ corresponds to a continuous Lipschitz diffusion operator \prox_g(\cdot). So, \proj is able to represent the diffusion 

\proj can well approximate the GD algorithm (Eq.~\ref{eqn:gd}), while \proj does not perfectly match ADMM unless we assume $\Mat{Q}_e^{(t)}=\Mat{H}_e^{(t)}$ in Eq.~\ref{eqn:admm-q} for a practical consideration. This assumption may reduce the performance of the hypergraph diffusion algorithm while our model \proj has already achieved good enough empirical performance. Tracking $\Mat{Q}_e^{(t)}$ means recording the messages from $\Set{E}$ to $\Set{V}$ for every iteration, which is not supported by the current GNN platforms~\cite{FeyPyG,wang2019dgl} and may consume more memory. We leave the study of the algorithms that can track the update of $\Mat{Q}_e^{(t)}$ as a future study. A co-design of the algorithm and the system may be needed to guarantee the scalability of the algorithm.  

\textbf{Extension.} Our \proj can be naturally extended to build equivariant node operators because of the duality between hyperedges and nodes, though this is not necessary in the traditional hypergraph diffusion problem Eq.~\ref{eqn:diffusion}. Specifically, we call this model \projtwo, which simple revises the step 1 in \proj as $\Mat{m}_{u\rightarrow e}^{(t)} = \hat{\phi}(\Mat{h}_u^{(t)}, \Mat{m}_e^{(t-1)})$ for any $e$ such that $u\in e$. Due to the page limit, we put some experiment results on \projtwo in Appendix~\ref{sec:expr_edgnn2}.


\subsection{Discussion: Advantages of \proj in Heterophilic Settings and Deep Models}
\label{sec:dis_heterophily}
Here, we discuss several advantages of \proj due to the design of equivariant diffusion operators. 

Heterophily describes the network phenomenon where nodes with the same labels and attributes are less likely to connect to each other directly~\cite{rogers2010diffusion}. %A direct example of network heterophily is intimate relationships where people with different genders are more likely to build a family in a social network. 
Predicting node labels in heterophilic networks is known to be more challenging than that in homophilic networks, and thus has recently become an important research direction in the community~\cite{pei2020geom,zhu2020beyond,chien2021adaptive,lim2021large}. Heterophily has been proved  as a more common phenomenon in hypergraphs than in graphs since it is hard to expect all nodes in a giant hyperedge to share a common label~\cite{li2017inhomogeneous,veldt2021higher}. Moreover, predicting node labels in heterophilic hypergraphs is more challenging than that in graphs as a hyperedge may consist of the nodes from multiple categories.% in different ratios. %(see Fig.~\ref{fig:heterophily}).

Learnable equivariant diffusion operators are expected to be superior in predicting heterophilic node labels. For example, if a hyperedge $e$ of size 3 is known to cover two nodes $v,u$ from class $\Set{C}_1$ while one node $w$ from class $\Set{C}_0$. We may use the LEC potential $\langle\Mat{y},\varsigma(\Mat{H}_e)\rangle^2$ by setting $\Mat{y} = [1,-1,0]^\top$. Suppose the three nodes' attibutes are $\Mat{H}_e=[\Mat{h}_v, \Mat{h}_u, \Mat{h}_w]^\top=[0.7, 0.5, 0.3]^\top$, where $\Mat{h}_v$, $\Mat{h}_u$ are close as they are from the same class. One may check the hyperedge diffusion operator gives $\nabla g(\Mat{H}_e) = [0.4, -0.4, 0]^\top$. One-step gradient descent $\Mat{h}_v - \eta [\nabla g(\Mat{H}_e)]_v$ with a proper step size ($\eta < 0.5$) drags $\Mat{h}_v$ and $\Mat{h}_u$ closer while keeping $\Mat{h}_w$ unchanged. However, invariant diffusion that allocates every node with the same change does not help with the classification. Moreover, consider another case when the ground truth is different, say $w,u$ from the same class and $v$ from the other, using the above $\Mat{y}$ may increase the error. However, learnable operators can solve the problem, e.g., by learning another $\Mat{y}=[0,1,-1]^\top$. 

Moreover, equivariant hyperedge diffusion operators are also good at building deep models. GNNs tend to degenerate the performance when going deep, which is often attributed to their oversmoothing~\cite{li2018deeper,oono2019graph} and overfitting problems~\cite{cong2021provable}. Equivariant operators allocating different messages to different nodes helps with overcoming the oversmoothing issue. On the other hand, diffusion operators by sharing parameters across different layers  may reduce the risk of overfitting.     


\subsection{Previous Hypergraph Neural Networks for Representing Hypergraph Diffusion}\label{sec:previous}

\proj is the first HNN inspired by the general class of hypergraph diffusion and can provably achieve  universal approximation of hyperedge diffusion operators. So, how about previous HNNs representing hypergraph diffusion? We temporarily ignore the big difference in whether parameters are shared across layers and give some analysis as follows. HGNN~\cite{feng2019hypergraph} runs graph convolution~\cite{kipf2016semi} on clique expansions of hypergraphs, which directly assumes the hyperedge potentials follow CE plus pairwise potentials and cannot learn other operations on hyperedges. HyperGCN~\cite{yadati2019hypergcn} essentially leverages the total variation potential by adding mediator nodes to each hyperedge, which adopts a transformation technique of the total variantion potential in~\cite{chan2018spectral,chan2020generalizing}. A few works view each hyperedge as a multi-set of nodes and each node as a multi-set of hyperedges~\cite{dong2020hnhn,huang2021unignn,chien2021you,bai2021hypergraph,arya2020hypersage,yadati2020neural,yang2020hypergraph,jo2021edge}. 
Among them, HNHN~\cite{dong2020hnhn}, UniGNNs~\cite{huang2021unignn}, EHGNN~\cite{jo2021edge} and AllSet~\cite{chien2021you} build two invariant set-pooling functions on both the hyperedge and node sides, which cannot represent equivariant functions. One subtle point is that Uni\{GIN,GraphSAGE,GCNII\}~\cite{huang2021unignn} adopt a jump link in each layer to pass node features from the former layer directly to the next and may expect to use a complicated node-side invariant function $\hat{\psi}'(\Mat{h}_v^{(t)},\sum_{e:v\in e} \Mat{m}_e^{(t)})$ to approximate our $\hat{\psi}(\Mat{h}_v^{(t)},\sum_{e:v\in e} \Mat{m}_{e\rightarrow v}^{(t)})=\hat{\psi}(\Mat{h}_v^{(t)},\sum_{e:v\in e} \hat{\rho}(\Mat{h}_v^{(t)},\Mat{m}_e^{(t)}))$ in Step 4 of \textbf{Algorithm 1} directly. This may be doable in theory. However, the jump-link solution may expect to have a higher dimension of $\Mat{m}_e^{(t)}$ (dim=$|\cup_{e:v\in e} e|$) so that the sum pooling $\sum_{e:v\in e} \Mat{m}_e^{(t)}$ does not lose anything from the neighboring nodes of $v$ before interacting with $\Mat{h}_v^{(t)}$, while in \proj,  $\Mat{m}_e^{(t)}$ needs dim=$|e|$ according to Theorem~\ref{thm:equivarnt_form_1dim}. Our empirical experiments also verify more expressiveness of \proj. HCHA~\cite{bai2021hypergraph} and UniGAT~\cite{yang2020hypergraph} compute attention weights as a result of combining node features and hyperedge messages, which looks like our $\rho$ operation. However, a scalar attention weight is too limited to represent the potentially complicated $\rho$. HyperSAGE~\cite{arya2020hypersage},   MPNN-R~\cite{yadati2020neural} and LEGCN~\cite{yang2020hypergraph} may learn hyperedge equivariant operators, while they need many auxillary nodes that represent node-hyperedge pairs. Of course, none of these works have mentioned any theoretical arguments on universal representation of hypergraph diffusion as ours.  

% $\mathcal{N}_{v}$    

% %, by inheriting from GIN~\cite{xu2018how} and GraphSAGE~\cite{hamilton2017inductive}


% designing message from $V$ to $E$ as $\Set{M}_{\Set{V}\rightarrow \Set{E}} = \hat{\phi}(\Mat{h}_u)$. 

% %=\Set{V}\cup\Set{V_{\Set{E}}}$. 



% To prove Theorem \ref{thm:equivarnt_form}, we sequentially adopt Lemma \ref{lem:equivariant_form} and results of invariant set functions in \cite{zaheer2017deepset}.
% We defer the detailed proof into \textcolor{red}{Appendix}.
% Theorem \ref{thm:equivarnt_form} demonstrates that an equivariant set function can be modeled by a pair-wise relationship between each element and a summarized vector of the whole set.
% Note that our proof avoids equivariant polynomials used in \cite{segol2019universal}, thus we can restrict the dimension of the summarized vector to be $d$.





% But their construction requires an exponential hidden dimension with respect to set cardinality to represent hyperedge features, which is infeasible to implement.
% In this section, we propose a more plausible solution to uniformly approximate equivariant operators capable of representing any type of hypergraph diffusions.


% However, there are still some gaps when applying their techniques to the hypergraph setting. Practically, most previous works focus on building models for multi-sets that are not coupled, such as a set of images or 3-D points, while hypergraphs contain coupled multi-sets as a node may appear in multiple hyperedges. Graphs couple edges that can be viewed as sets of nodes while edges in graphs are of regular size two so building equivariant edge operation is not that crucial and challenging in GNN design. In theory, previous works proposed the form of linear layer composed with the entry-wise nonlinear activation to build equivariant multi-set representation~\cite{zaheer2017deepset,maron2018invariant}, which has later been proved to achieve universal approximation~\cite{segol2020universal}. However, the proof in~\cite{segol2020universal} uses equivariant polynomials as a bridge, which induces two issues of the obtained conclusion. The statement is always an approximation statement and the  


% Hence, how to build computationally efficient equivariant hyperedge operations in HGNN?

% Hence, how to efficiently build equivariant hyperedge operations in HGNN 

% No previous works have proposed the coupled ones as we observed in hypergraphs.

% Hyperedge operaters are set eqvariant, then how to build them? Building equivariant set neural network architecture has been studied in xxx. Practically, they mostly focus on building separate sets. No previous works have proposed the coupled ones as we observed in hypergraphs. Theoretically, deepset and Maron proposes the form of linear layer composed with the entry-wise nonlinear activation to build equivariant set representation. Segol proves the unverival approximation of it, while Segol's proof is built upon equivariant polynomial so there is only approximation result. However, we may have precise argument as following theorem, though learning $\rho$ and $\phi$ via NN still needs approximation.  

% The crucial thing is how to efficiently implement it. Bipartite framework: One cannot record everything and do invariance. The key is to invariant pooling on hyperedge side. When message passes from hyperedge to nodes, do equivariant before pooling. Overall the processing is equivariant. Different from Allsets, Allset first invariant pool and second jump link. However, such invariant pool may need to enlarge the dimension to record the entire receptive field. 

% \subsection{} 
% further build double equivariant.

% build attention equivariant (All set uses a single vector) 

% \cite{yadati2020neural} build new nodes for node hyperedge pair (too complicated)

% \cite{arya2020hypersage} use complement $e/v$ to build rep

% \cite{dong2020hnhn} double invariant sets no jump link

% \cite{huang2021unignn} double invariant sets with jump link

% \cite{chien2021you} double invariant no jump link

% \cite{yadati2019hypergcn} use a mediator.

% It seems that~\cite{bai2021hypergraph} considers the attention equi. (also double invariant)

% \subsection{}



% %maron discuss the general linear layers to build equivariant set representation while there is no universal guarantee. Segol   


% The choice of $g(\cdot)$ varies from different tasks. For real-world data, it is intractable to handcraft a potential function that precisely express prior distribution over hyperedges.
% Recent works \cite{gregor2010learning, liu2019alista, chen2018theoretical, yang2021graph, liu2021elastic} have shown that unrolling and parameterizing each iteration of an optimization problem with neural networks can express more universal objectives and achieve faster convergence.
% Motivated by this line of works, we intend to construct a parametric hypergraph diffusion operator that can be learned from data. \pan{Claim how to implement equi hyperedge operator is non-trivial. Previous works are regular. Moreover, standard model, do not need to worry this.}

% \pan{Build a bipartite graph by following HNHN and allset. However, we show that invariant sum pooling when message  The sum pooling over hyperedges. When message passes from hyperedges to nodes, we do an additional operation. This techniques have been used in xxx while no hypergraph NN has used this to build eq.  Moreover, our results are not approximation results. The needed dimension is polynomial w.r.t.... }
% A handy choice to parameterize hypergraph diffusion operator is neural networks. However, typical architectures, such as Multi-Layer Perceptrons (MLP), would not be the candidate as they do not satisfy the equivariance property.
% % Zaheer \etal \cite{zaheer2017deepset} proposed a sum-pooling based architecture that can represent any set functions, 
% To achieve order invariance, one may consider DeepSet \cite{zaheer2017deepset} which introduces a sum-pooling scheme to represent arbitrary set functions.
% However, it is subject to invariant operators, which are essentially less expressive than equivariant operators.
% Segol \etal \cite{segol2019universal} adopted symmetric polynomials as a tool to approximate equivariant set function.
% But their construction requires an exponential hidden dimension with respect to set cardinality to represent hyperedge features, which is infeasible to implement.
% In this section, we propose a more plausible solution to uniformly approximate equivariant operators capable of representing any type of hypergraph diffusions.


% % In previous section, we already know to approximate hypergraph diffusion operator, we need to build a permutation-equivariant set function.
% % Even though it is well-known that building a permutation-invariant set function is as simple as raising the input elements into a high-dimension space, summing over the set to obtain a summarized vector, and projecting it to the output space, how to constructing a permutation-equivariant function remains elusive in the literature.

% Our follow-up discussion falls on how to represent permutation-equivariant functions in general. To this end, we first provide the following lemma:
% \begin{lemma} \label{lem:equivariant_form}
% $f: \mathbb{R}^k \rightarrow \mathbb{R}^k$ is an equivariant function if and only if $f(\cdot)$ can be represented as the following form, 
% \begin{align}
%     f(x_1, x_2, \cdots , x_{k-1}, x_k) = 
%     \begin{bmatrix} 
%     p(x_1, x_2, \cdots, x_{k-1}, x_k) \\
%     p(x_2, x_3, \cdots, x_k, x_1) \\
%     \vdots \\
%     p(x_N, x_1, \cdots, x_{k-2}, x_{k-1}) \\
%     \end{bmatrix}
% \end{align}
% where $p(\cdot): \mathbb{R}^k \rightarrow \mathbb{R}$ is permutation-invariant with respect to the last $k-1$ elements of inputs. 
% \end{lemma}
% We give a proof in the \textcolor{red}{Appendix}.
% Lemma \ref{lem:equivariant_form} implies that an equivariant function can be element-wisely decomposed into partially invariant mappings, which bridges the construction of invariant and equivariant functions.
% Prior works \cite{zaheer2017deepset, wagstaff2019limitations} have guaranteed a finite-dimension and continuous construction of invariant functions.
% Using Lemma \ref{lem:equivariant_form}, we are about to compose width-limited and continuous equivariant functions using such invariant functions.
% As shown below, we formally specifies a general form that equivariant function must have:
% \begin{theorem} \label{thm:equivarnt_form}
% $g(\cdot): \mathbb{R}^k \rightarrow \mathbb{R}^k$ is a continuous equivariant function,if and only if $g(\cdot)$ can be represented as the following form, 
% \begin{align}
%     g(x_1, x_2,\cdots,x_k) =
%      \begin{bmatrix} 
%     \rho(x_1, \sum_{i=1}^k \phi(x_i)) \\
%     \rho(x_2, \sum_{i=1}^k \phi(x_i)) \\
%     \vdots\\
%     \rho(x_3, \sum_{i=1}^k \phi(x_i)) \\
%     \end{bmatrix}
% \end{align}
% where $\rho: \real^d \rightarrow \real$, $\phi: \real \rightarrow \real^d$ are all continuous functions. \pan{fill in the F dim case.}
% \end{theorem}
% To prove Theorem \ref{thm:equivarnt_form}, we sequentially adopt Lemma \ref{lem:equivariant_form} and results of invariant set functions in \cite{zaheer2017deepset}.
% We defer the detailed proof into \textcolor{red}{Appendix}.
% Theorem \ref{thm:equivarnt_form} demonstrates that an equivariant set function can be modeled by a pair-wise relationship between each element and a summarized vector of the whole set.
% Note that our proof avoids equivariant polynomials used in \cite{segol2019universal}, thus we can restrict the dimension of the summarized vector to be $d$.
% % \textcolor{red}{emphasize the difference between ICLR 2019 and ours. Ours does not need equivariant polynomial, and the dimension can be reduced to d}

% \subsection{Unfolding Hypergraph Diffusion as HGNN}
% \pan{Suggest to directly merge this section with the previous one.}
% We observe that each diffusion step for both differentiable (Eq. \ref{eqn:gd}) and non-differentiable (Eq. \ref{eqn:admm}) potential functions can be unified into the following form:
% \begin{align} \label{eqn:neural_diffusion}
%     \Mat{h}_v^{(t+1)} = \rho\left(\Mat{h}_v^{(t)}, \sum_{e:v \in e} \phi_v(\Mat{H}_e^{(t)}) \right)
% \end{align}
% where $\phi: \real^{|e| \times d} \rightarrow \real^{|e| \times d}$ corresponds to gradient operators over hyperedges $\nabla_{v} g(\cdot)$ and $\prox_{\frac{1}{\rho} g}(\cdot)$ that aggregates node features to be hyperedge-level features and dispatches them to each node, $\phi_v(\cdot)$ indexes the value at node $v$, while $\rho: \real^{d} \times \real^{d} \rightarrow \real^{d}$ combines hyperedge features with node features.
% The choice of $f(\cdot)$ and $g(\cdot)$ varies from different tasks. For real-world data, handcrafting potential functions that precisely express prior distribution over hyperedges can be intractable.
% Recent works \textcolor{red}{Cite LISTA and other unrolling graph papers} have shown that unrolling each iteration in an optimization problem can naturally derive similar structures to multi-layer neural networks, that introduces a group of learnable parameters to express more universal objectives and achieve faster convergence.
% Motivated by this line of works, we intend to construct a parametric hypergraph diffusion operator that can be learned from data.
% Thereby we parameterize $\rho(\cdot)$ and $\phi(\cdot)$ with some learnable parameters $\Mat{\Theta}$, then Eq. \ref{eqn:neural_diffusion} can be viewed as the $t$-th layer of hypergraph neural networks.
% Unfolding $L$ iterations results in an $L$-layer hypergraph neural networks.

% \subsection{Implementing Equivariant Diffusion HGNN}

% With Theorem \ref{thm:equivarnt_form}, we can borrow neural networks to parameterize $\rho(\cdot)$ and $\phi(\cdot)$ due to the universal approximation theorem.
% This implies we can build a neural hypergraph diffusion operator in the following form: 
% \begin{align} \label{eqn:neural_nd}
% \nabla_v g\left(\Mat{h}^{(e)}_1, \Mat{h}^{(e)}_2,....,\Mat{h}^{(e)}_{|e|}\right) =
%  \begin{bmatrix} 
% \MLP_2(\Mat{h}^{(e)}_1, \sum_{i=1}^{|e|} \MLP_1(\Mat{h}^{(e)}_i)) \\
% \MLP_2(\Mat{h}^{(e)}_2, \sum_{i=1}^{|e|} \MLP_1(\Mat{h}^{(e)}_i)) \\
% \vdots\\
% \MLP_2(\Mat{h}^{(e)}_{|e|}, \sum_{i=1}^{|e|} \MLP_1(\Mat{h}^{(e)}_i)) \\
% \end{bmatrix},
% \end{align}
% where $\MLP_1: \real^d \rightarrow \real^{|e|d}$ raises the dimension of each node feature, and $\MLP_2: \real^d \times \real^{|e|d} \rightarrow \real^{d'}$ concatenates the feature of the first input and the summarized vector and projects them into the output space.
% During the training stage, we iteratively invoke Eq. \ref{eqn:neural_nd} for $L$ times, and optimize MLP parameters by back propagating loss of some downstream tasks.

% \subsection{Comparison with Hypergraph Neural Networks}


% \begin{proposition} (Informal)
% AllSet, HGNN, HyperGNN are permutation-invariant but not permutation-equivariant.
% \end{proposition}

% \textcolor{red}{discuss difference between other models AllSet, HyperGCN, HGNN.}

% \textcolor{red}{another clue is first propose our model, and then discuss existing models, how our model degenerate to their model.}


% \textcolor{red}{discuss a variant of our model: two equivariant set functions (allset)}

% \textcolor{red}{our model can go deeper to achieve better performance due to diffusion model}

% \textbf{Introduce how we implement the equivariant diffusion via neural networks. Overall, we have \proj.}


% Suppose we are to approximate $H_v^{(1)}$ where $H^{(0)} = X$, initial $q_e^{(0)}=0$. (put into appendix)
% \begin{align*}
%         q_e^{(1)} &\leftarrow  \prox_{\frac{1}{\rho},g}(2\bar{h}_e^{(0)}) - \bar{h}_e^{(0)}\\
%         h_v^{(1)} &\leftarrow  
%         \prox_{\frac{1}{\rho d_v},f}(p_v),\quad \text{where}\; p_v=\frac{1}{d_v}\sum_{e:e\in v}q_{e,v}^{(1)}%\\
%         %s_e^{(t+1)} &\leftarrow s_e^{(t)} + r_e^{(t+1)} - \bar{h}_v^{(t+1)}
%     \end{align*} 

% Or you may choose Gradient-descent (main text):
%     \begin{align*}
%         h_v^{(t+1)} \leftarrow  h_v^{(t)} - \alpha \left(\nabla f(h_v^{(t)};x_v) + \sum_{e: v\in e} q_{e,v}^{(t)}\right), \quad \text{where}\; q_{e,v}^{(t)} = \nabla g(\bar{h}_e^{(t)}),\; \text{for}\; v\in V.
%     \end{align*}
    

% % If we consider the update as a hypergraph operator $\psi: h_v^{(t)} \rightarrow h_v^{(t+1)}$, both settings essentially correspond to a mapping function
% % %\begin{align*}
% % %    h_v^{(t+1)} = \psi_1(h_v^{(t)}, \oplus_{e:v\in e} q_{e,v}^{(t+1)}),\,\text{where}\;q_{e,v}^{(t+1)} = \psi_2(h_v^{(t)}, \oplus_{u\in e/v} h_u^{(t)})  
% % %\end{align*}
% % \begin{align*}
% %     z = \psi(x, \oplus_{e:v\in e}\oplus_{u\in e/v} s_{e,u}),\; \text{where}\; s_{e,u} = h_{u}^{(t)}. %q_{e,v}^{(t+1)}),\,\text{where}\;q_{e,v}^{(t+1)} = \psi_2(h_v^{(t)}, \oplus_{u\in e/v} h_u^{(t)})  
% % \end{align*}
% % which is invariance with respect to the permutation $\pi_v$ over $\{e|v\in e\}$ and the  permutations $\pi_{v,e}$ over $\{u\in e|u\neq v\}$, i.e., 





% \textbf{3. Prove dimension argument: vs ID, vs jump link + ID}

% %I use $[\nabla g(\bar{x}_e)]_v$ to denote the gradient w.r.t. $x_v$ of the invariant function $g(\cdot)$ with $|e|$-dim input $\bar{x}_e = (...,x_u,...)_{u\in e}$. 




% Our proposal: 
% \begin{itemize}
%     \item Equivariant operator:
% \begin{align*}
%     \text{MLP}_3(x_v,x_v^{(0)},\sum_{e:v\in e} \text{MLP}_2(x_v, \sum_{u\in e}\text{MLP}_1(x_u))).
% \end{align*}
% Theoretically, we just need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2) $\text{MLP}_2: \mathbb{R}^{|e|+1} \rightarrow \mathbb{R}$; (3) $\text{MLP}_3: \mathbb{R}^3 \rightarrow \mathbb{R}$



% \item Jump-link + Invariant operator: 
% \begin{align*}
%     \text{MLP}_3(x_v, \sum_{e:v\in e} \text{MLP}_2(\sum_{u\in e}\text{MLP}_1(x_u))).
% \end{align*}
% Theoretically, we need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2)
% $\text{MLP}_2: \mathbb{R}^{|e|} \rightarrow \mathbb{R}^{(|e|-1)*d_v+1}$; (3) $\text{MLP}_3: \mathbb{R}^{(|e|-1)*d+1} \rightarrow \mathbb{R}$.

% % \item Small invariant operator (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% % \begin{align*}
% %     \text{MLP}_2(\sum_{e:v\in e} \sum_{u\in e}\text{MLP}_1(x_u)).
% % \end{align*}
% % We know this cannot give universal approximation. But the parameter selection should be at least the same as equivariant operator.


% \item Big invariant operator: 
% \begin{align*}
%     \text{MLP}_3(\sum_{e:v\in e} \text{MLP}_2(\sum_{u\in e}\text{MLP}_1(x_u))).
% \end{align*}
% We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

% \item Attention-based (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% \begin{align*}
%     Attention_2(\text{MLP}_2(Attention_1(\{\text{MLP}_1(x_u)|u\in e\}))|e:v\in e).
% \end{align*}
% We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

% \end{itemize}

% Empirical comparison: We study the dependence on $k$ from 20-200. We should consider alternative projection and subgradient descent. We should consider the following models with degree and node feature fixed.

% %We also add the following three models.

% % \begin{itemize}
% % \item Small equivariant operator (In sec 3, we do not need to discuss this, which is just for fair comparison):
% % \begin{align*}
% %     \sum_{e:v\in e} \text{MLP}_2(x_v, \sum_{u\in e}\text{MLP}_1(x_u)).
% % \end{align*}

% % \item Small invariant operator (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% % \begin{align*}
% %     \text{MLP}_2(\sum_{e:v\in e} \sum_{u\in e}\text{MLP}_1(x_u)).
% % \end{align*}

% %\end{itemize}

% \begin{itemize}
%     \item Equivariant operator:
% \begin{align*}
%     \text{Linear}_3(x_v,\log d_v,\text{mean}_{e:v\in e} \text{MLP}_2(x_v, \log |e|, \text{mean}_{u\in e}\text{MLP}_1(x_u,\log d_v))).
% \end{align*}
% %Theoretically, we just need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2) $\text{MLP}_2: \mathbb{R}^{|e|+1} \rightarrow \mathbb{R}$; (3) $\text{MLP}_3: \mathbb{R} \rightarrow \mathbb{R}$



% \item Jump-link + Invariant operator: 
% \begin{align*}
%     \text{Linear}_3(x_v, \log d_v,  \text{mean}_{e:v\in e} \text{MLP}_2(\log |e|,\text{mean}_{u\in e}\text{MLP}_1(x_u,\log d_v))).
% \end{align*}
% %Theoretically, we need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2)
% %$\text{MLP}_2: \mathbb{R}^{|e|} \rightarrow \mathbb{R}^{(|e|-1)*d+1}$; (3) $\text{MLP}_3: \mathbb{R}^{(|e|-1)*d+1} \rightarrow \mathbb{R}$.

% % \item Small invariant operator (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% % \begin{align*}
% %     \text{MLP}_2(\sum_{e:v\in e} \sum_{u\in e}\text{MLP}_1(x_u)).
% % \end{align*}
% % We know this cannot give universal approximation. But the parameter selection should be at least the same as equivariant operator.


% \item Big invariant operator: 
% \begin{align*}
%     \text{Linear}_3(\log d_v,\text{mean}_{e:v\in e} \text{MLP}_2(\log |e|, \text{mean}_{u\in e}\text{MLP}_1(x_u,\log d_u))).
% \end{align*}
% We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

% \item Attention-based (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% \begin{align*}
%     Attention_2(\log d_v,\text{MLP}_2(Attention_1(\log |e|,\{\text{MLP}_1(x_u)|u\in e\}))|e:v\in e).
% \end{align*}
% We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

% \end{itemize}



% \begin{itemize}
%     \item Equivariant operator: $\text{MLP}_1: 2\times 200, 200\times k$, $\text{MLP}_2: k+2\times 200,  200\times k+2$, $\text{Linear}_3: k+2\times 1$.
    
%     \item Fair equivariant operator: $\text{MLP}_1: 1\times 200, 200\times k$, $\text{MLP}_2: k+2\times 200, 200\times 200$. $\text{Linear}_3: 200\times 1$.
    
%     \item Jump-link + Invariant operator: $\text{MLP}_1: 1\times 200, 200\times k$,
%     $\text{MLP}_2: k+1\times 200, 200\times 200$
%     $\text{Linear}_3: 200+2\times 1$.

%     %\item Small Invariant operator: $\text{MLP}_1: 1\times 200, 200\times k$,
%     %$\text{MLP}_2: k\times 200, 200\times 1$.

%     \item Big Invariant operator: $\text{MLP}_1: 1\times 200, 200\times k$,
%     $\text{MLP}_2: k+1\times 200, 200\times 200$,
%     $\text{Linear}_3: 201\times 1$.   

%     \item Attention: $\text{MLP}_1: 1\times 200, 200\times k$,
%     $\text{Attention}_1: {k+1}\times {k+1}$,
%     $\text{MLP}_2: {k+1}\times 200, 200\times 200$,
%     $\text{Attention}_2: 201\times 1$.

% \end{itemize}

==> arxiv/section_files/004-related.tex <==
\vspace{-2mm}
\section{Further Discussion on Related Works} \label{sec:related}
\vspace{-1mm}
We have discussed the most relevant works on HNN architectures and hypergraph diffusion algorithms in Sec.~\ref{sec:model}. Here, we review some relevant works on optimization-inspired NNs. Optimization-inspired NNs often get praised for their interpretability~\cite{monga2021algorithm,chen2021learning} and certified convergence under certain conditions of the learned operators~\cite{ryu2019plug,teodoro2017scene,chan2016plug}. Early works that adopt optimization-inspired NNs focus on the applications such as compressive sensing~\cite{gregor2010learning,xin2016maximal,liu2019alista, chen2018theoretical}, speech processing~\cite{hershey2014deep,wang2018end}, image denoising~\cite{zhang2017learning,meinhardt2017learning,rick2017one,chen2016trainable}, partitioning~\cite{zheng2015conditional,liu2017deep}, deblurring~\cite{schuler2015learning,li2020efficient} and so on. Recently, optimization-inspired NNs have also been applied to graphs~\cite{yang2021graph,liu2021elastic,chen2021graph,klicpera2019predict}. They unroll either learnable~\cite{yang2021graph,chen2021graph},  fixed $\ell_1$-norm~\cite{liu2021elastic} or fixed $\ell_2$-norm pair-wise potentials~\cite{klicpera2019predict} to formulate GNNs. Some works also view the graph diffusion as an ODE~\cite{chamberlain2021grand,thorpe2022grand++}, which essentially corresponds to our gradient descent Eq.~\ref{eqn:gd}. As there are only pairwise relations in graphs, the GNN design is often much simpler than the HNN counterpart. To construct an expressive operator with for pairwise relations is trivial. Implicit NNs~\cite{bai2019deep,el2021implicit} are to directly parameterize the optimum of an optimization problem. Implicit NNs have also been applied to graphs~\cite{dai2018learning,liu2021eignn,gu2020implicit,yang2021implicit} but not to hypergraphs. So, a future study of this work is to develop implicit models that can directly parameterize the solution to Eq.~\ref{eqn:diffusion}.    

%Recent works~\cite{gregor2010learning, liu2019alista, chen2018theoretical} that have shown that unrolling and parameterizing each iteration of an optimization problem with neural networks can express more universal objectives and achieve faster convergence, motivated by this line of works, we intend to construct a parametric hypergraph diffusion operator that can be learned from data. 

%Janossy pooling and others???

==> arxiv/section_files/005-experiments.tex <==
\vspace{-2mm}
\section{Experiments} \label{sec:exp}
\vspace{-3mm}
\begin{table}[t]
\small{\caption{Dataset statistics. CE homophily is the homophily score~\cite{pei2020geom} based on CE of hypergraphs.}
\label{tab:dataset_stats}}
\centering
\resizebox{0.90\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
& Cora & Citeseer & Pubmed & Cora-CA & DBLP-CA & Congress & Senate & Walmart & House \\
\midrule
\# nodes & 2708 & 3312 & 19717 & 2708 & 41302 & 1718 & 282 & 88860 & 1290 \\
\# edges & 1579 & 1079 & 7963 & 1072 & 22363 & 83105 & 315 & 69906 & 340 \\
%\# features & 1433 & 3703 & 500 & 1433 & 1425 & 100 & 100 & 100 & 100 \\
\# classes & 7 & 6 & 3 & 7 & 6 & 2 & 2 & 11 & 2 \\
%avg. $d_v$ & 2.767 & 2.043 & 2.756 & 2.693 & 3.411 & 427.251 & 20.177 & 6.184 & 10.180 \\
avg. $|e|$ & 1.748 & 1.541 & 1.963 & 1.929 & 2.213 & 8.654 & 9.531 & 3.461 & 8.056 \\
CE Homophily & 0.897 & 0.893 & 0.952 & 0.803 & 0.869 & 0.555 & 0.498 & 0.530 & 0.509 \\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\end{table}




\subsection{Results on Benchmarking Datasets} \label{sec:real-data-exp}
\vspace{-1mm}
\textbf{Experiment Setting.}
In this subsection, we evaluate \proj on nine real-world benchmarking hypergraphs. We focus on the semi-supervised node classification task. %in the transductive setting.
The nine datasets include co-citation networks (Cora, Citeseer, Pubmed), co-authorship networks (Cora-CA, DBLP-CA) \cite{yadati2019hypergcn}, Walmart \cite{amburg2020clustering}, House \cite{chodrow2021hypergraph}, Congress and Senate~\cite{fowler2006legislative,fowler2006connecting}. More details of these datasets can be found in Appendix~\ref{sec:dataset_detail}. Since the last four hypergraphs do not contain node attributes, we follow the method of \cite{chien2021you} to generate node features from label-dependent Gaussian distribution \cite{deshpande2018contextual}.

As we show in Table \ref{tab:dataset_stats}, these datasets already cover sufficiently diverse hypergraphs in terms of scale, structure, and homo-/heterophily.
We compare our method with top-performing models on these benchmarks, including HGNN \cite{feng2019hypergraph}, HCHA \cite{bai2021hypergraph}, HNHN \cite{dong2020hnhn}, HyperGCN \cite{yadati2019hypergcn}, %HyperSAGE \cite{arya2020hypersage}, 
UniGCNII \cite{huang2021unignn}, AllDeepSets \cite{chien2021you}, and AllSetTransformer \cite{chien2021you}.
All the hyperparameters for baselines follow from \cite{chien2021you} and we fix the learning rate, weight decay and other training recipes same with the baselines. Other model specific hyperparameters are obtained via grid search (see Appendix \ref{sec:hparam}). We randomly split the data into training/validation/test samples using 50\%/25\%/25\% splitting percentage by following \cite{chien2021you}. We choose prediction accuracy as the evaluation metric. We run each model for ten times with different training/validation splits to obtain the standard deviation. \vspace{-1mm}

\textbf{Performance Analysis.}
Table \ref{tab:real_data} shows the results. Our \proj uniformly outperforms all the compared models on all the datasets. We observe that the top-performing baseline models are AllSetTransformer, AllDeepSets and UniGCNII. %where the former two represent HNNs using two invariant multiset functions, while the later one improves traditional HNNs by initial and jumping links.
As having been analyzed in Sec.~\ref{sec:previous}, they model invariant set functions on both node and hyperedge sides. UniGCNII also adds initial and jump links, which accidentally resonates with our design principle (the step 4 in Algorithm 1). However, their performance has large variation across different datasets.
For example, UniGCNII attains promising performance on citation networks, however, has subpar results on Walmart dataset.
In contrast, our model achieves stably superior results, surpassing AllSet models by 12.9\% on Senate and UniGCNII by 12.5\% on Walmart.
We owe our empirical significance to the theoretical design of exact equivariant function representation. 
%While adopting set functions, AllSet models cannot capture equivariance.
%UniGCNII adopts jump links, but it is not as expressive as our \proj. 
Regarding the computational efficiency, we report the wall-clock times for training (for 100 epochs) and testing of all models over the largest hypergraph Walmart, where all models use the same hyperparameters that achieve the reported performance on the left. Our model achieves efficiency comparable to AllSet models~\cite{chien2021you} and is much faster than UniGCNII. So, the implementation of equivariant computation in \proj is still efficient. 
\begin{table}[t]
\small{\caption{Prediction Accuracy (\%). \textbf{Bold font$^\dagger$} highlights when \proj significantly (difference in means > 0.5 $\times$ std) outperforms all baselines. The \underline{best baselines} are underlined. The training and testing times are test on Walmart by using the same server with one GPU NVIDIA RTX A6000.}
\label{tab:real_data}}
\centering
\resizebox{1\textwidth}{!}{
\begin{tabular}{cccccc|c}
\toprule
& Cora & Citeseer & Pubmed & Cora-CA & DBLP-CA & Training Time ($10^{-1}$ s) \\
\midrule
HGNN \cite{huang2021unignn} & \underline{79.39 $\pm$ 1.36} & 72.45 $\pm$ 1.16 & 86.44 $\pm$ 0.44 & 82.64 $\pm$ 1.65 & 91.03 $\pm$ 0.20 & 0.24 $\pm$ 0.51 \\
HCHA \cite{bai2021hypergraph} & 79.14 $\pm$ 1.02 & 72.42 $\pm$ 1.42 & 86.41 $\pm$ 0.36 & 82.55 $\pm$ 0.97 & 90.92 $\pm$ 0.22 & 0.24 ± 0.01 \\
HNHN \cite{dong2020hnhn} & 76.36 $\pm$ 1.92 & 72.64 $\pm$ 1.57 & 86.90 $\pm$ 0.30 & 77.19 $\pm$ 1.49 & 86.78 $\pm$ 0.29 & 0.30 $\pm$ 0.56 \\
HyperGCN \cite{yadati2019hypergcn} & 78.45 $\pm$ 1.26 & 71.28 $\pm$ 0.82 & 82.84 $\pm$ 8.67 & 79.48 $\pm$ 2.08 & 89.38 $\pm$ 0.25 & 0.42 $\pm$ 1.51 \\
%HyperSAGE \cite{arya2020hypersage} & 78.23 $\pm$ 1.30 & 73.06 $\pm$ 1.48 & 88.72 $\pm$ 0.53 & 81.92 $\pm$ 1.04 & 91.49 $\pm$ 0.21 & 0.71 $\pm$ 0.81 \\
UniGCNII \cite{huang2021unignn} & 78.81 $\pm$ 1.05 & 73.05 $\pm$ 2.21 & 88.25 $\pm$ 0.40 & \underline{83.60 $\pm$ 1.14} & \underline{91.69 $\pm$ 0.19} & 4.36 $\pm$ 1.18 \\
AllDeepSets \cite{chien2021you} & 76.88 $\pm$ 1.80 & 70.83 $\pm$ 1.63 & \underline{88.75 $\pm$ 0.33} & 81.97 $\pm$ 1.50 & 91.27 $\pm$ 0.27 & 1.23 $\pm$ 1.09\\
AllSetTransformer \cite{chien2021you} & 78.58 $\pm$ 1.47 & \underline{73.08 $\pm$ 1.20} & 88.72 $\pm$ 0.37 & 83.63 $\pm$ 1.47 & 91.53 $\pm$ 0.23 & 1.64 $\pm$ 1.63 \\
\midrule
\proj (ours) & \textbf{80.31 $\pm$ 1.35}$^\dagger$ & \textbf{73.70 $\pm$ 1.38}$^\dagger$ & \textbf{89.03 $\pm$ 0.53}$^\dagger$ & 83.97 $\pm$ 1.55 & \textbf{91.90 $\pm$ 0.19}$^\dagger$ & 1.71 $\pm$ 1.13 \\
% \projtwo & 77.47 $\pm$ 1.62 & 72.65 $\pm$ 1.56 & 88.86 $\pm$ 0.40 & 82.17 $\pm$ 1.68 & 91.62 $\pm$ 0.29 \\
% ED-HNN Attn. & 78.63 $\pm$ 1.55 & 71.21 $\pm$ 1.37 & 88.74 $\pm$ 0.37 & 82.33 $\pm$ 1.74 & 91.84 $\pm$ 0.25 \\
\bottomrule
& Congress & Senate & Walmart & House & Avg. Rank & Inference Time ($10^{-2}$ s)\\
\midrule
HGNN \cite{huang2021unignn} & 91.26 $\pm$ 1.15 & 48.59 $\pm$ 4.52 & 62.00 $\pm$ 0.24 & 61.39 $\pm$ 2.96  & 4.89 & 1.01 $\pm$ 0.04 \\
HCHA \cite{bai2021hypergraph} & 90.43 $\pm$ 1.20 & 48.62 $\pm$ 4.41 & 62.35 $\pm$ 0.26 & 61.36 $\pm$ 2.53 & 5.44 & 1.54 $\pm$ 0.18 \\
HNHN \cite{dong2020hnhn} & 53.35 $\pm$ 1.45 & 50.93 $\pm$ 6.33 & 47.18 $\pm$ 0.35 & 67.80 $\pm$ 2.59 & 7.11 & 6.11 $\pm$ 0.05\\
HyperGCN \cite{yadati2019hypergcn} & 55.12 $\pm$ 1.96 & 42.45 $\pm$ 3.67 & 44.74 $\pm$ 2.81 & 48.32 $\pm$ 2.93 & 7.33 & 0.87 $\pm$ 0.06 \\
%HyperSAGE \cite{arya2020hypersage} & 92.12 $\pm$ 0.94 & \underline{55.56 $\pm$ 5.27} & 59.14 $\pm$ 0.45 & 68.40 $\pm$ 3.07 & 4.33 & 1.17 $\pm$ 0.02 \\
UniGCNII \cite{huang2021unignn} & \underline{94.81 $\pm$ 0.81} & 49.30 $\pm$ 4.25 & 54.45 $\pm$ 0.37 & 67.25 $\pm$ 2.57 & 3.67 & 21.22 $\pm$ 0.13\\
AllDeepSets \cite{chien2021you} & 91.80 $\pm$ 1.53 & 48.17 $\pm$ 5.67 & 64.55 $\pm$ 0.33 & 67.82 $\pm$ 2.40  & 4.89 & 5.35 $\pm$ 0.33 \\
AllSetTransformer \cite{chien2021you} & 92.16 $\pm$ 1.05 & \underline{51.83 $\pm$ 5.22} & \underline{65.46 $\pm$ 0.25} & \underline{69.33 $\pm$ 2.20} & 2.67 & 6.06 $\pm$ 0.67 \\
\midrule
\proj (ours) & 95.00 $\pm$ 0.99 & \textbf{64.79 $\pm$ 5.14}$^\dagger$ & \textbf{66.91 $\pm$ 0.41}$^\dagger$ & \textbf{72.45 $\pm$ 2.28}$^\dagger$ & 1.00 & 5.87 $\pm$ 0.36 \\
% \projtwo & 95.19 $\pm$ 1.34 & 65.01 $\pm$ 6.17 & 65.24 $\pm$ 0.45 & 70.95 $\pm$ 1.97 \\
% ED-HNN Attn. & 95.24 $\pm$ 1.48 & 65.32 $\pm$ 6.72 & 67.06 $\pm$ 0.53 & 71.10 $\pm$ 2.65 \\
\bottomrule
\end{tabular}}
\vspace{-4mm}
\end{table}

%\paragraph{Efficiency Analysis}


\vspace{-2mm}
\subsection{Results on Synthetic Heterophilic Hypergraph Dataset}
\vspace{-2mm}
\begin{table}[t]
\small{\caption{Prediction Accuracy (\%) over Synthetic Hypergraphs with Controlled Heterophily $\alpha$.}
\label{tab:syn_node_data}}
\centering
\resizebox{1\textwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{} & \multicolumn{2}{c}{Homophily} & \multicolumn{4}{c}{Heterophily} \\
& $\alpha = 1$ & $\alpha = 2$ & $\alpha = 3$ & $\alpha = 4$ & $\alpha = 6$ & $\alpha = 7$ \\
\midrule
HGNN \cite{huang2021unignn} & 99.86 $\pm$ 0.05 & 90.42 $\pm$ 1.14 & 66.60 $\pm$ 1.60 & 57.90 $\pm$ 1.43 & 50.77 $\pm$ 1.94 & 48.68 $\pm$ 1.21 \\
HGNN + JumpLink \cite{huang2021unignn} & 99.29 $\pm$ 0.19 & 92.61 $\pm$ 0.97 & 79.59 $\pm$ 2.32 & 64.39 $\pm$ 1.55 & 55.39 $\pm$ 2.01 & 51.14 $\pm$ 2.05 \\
AllDeepSets \cite{chien2021you} & 99.86 $\pm$ 0.07 & 99.13 $\pm$ 0.31 & 92.39 $\pm$ 1.68 & 80.12 $\pm$ 2.31 & 56.42 $\pm$ 0.85 & 52.14 $\pm$ 2.88 \\
AllDeepSets + JumpLink \cite{huang2021unignn} & 99.95 $\pm$ 0.07 & 99.08 $\pm$ 0.24 & 93.52 $\pm$ 1.31 & 83.45 $\pm$ 2.64 & 59.68 $\pm$ 1.27 & 52.21 $\pm$ 2.36 \\
AllSetTransformer \cite{chien2021you} & 98.60 $\pm$ 0.48 & 95.89 $\pm$ 0.90 & 88.38 $\pm$ 1.81 & 83.34 $\pm$ 1.33 & 54.13 $\pm$ 4.83 & 50.15 $\pm$ 1.73 \\
\midrule
\proj (ours)  & 99.95 $\pm$ 0.08 & \textbf{99.68 $\pm$ 0.13}$^{\dagger}$ & \textbf{95.37 $\pm$ 1.23}$^{\dagger}$ & \textbf{90.35 $\pm$ 0.83}$^{\dagger}$ & \textbf{65.58 $\pm$ 0.76}$^{\dagger}$ & \textbf{54.31 $\pm$ 2.40}$^{\dagger}$ \\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\end{table}

\paragraph{Experiment Setting.} As discussed, \proj is expected to perform well on heterophilic hypergraphs. We evaluate this point by using synthetic datasets with controlled heterophily.
%In this section, we verify our argument by synthetic datasets with controlled heterophily.
We generate data by using contextual hypergraph stochastic block model~\cite{deshpande2018contextual,ghoshdastidar2014consistency,chien2018community}. Specifically, we draw two classes of $2,500$ nodes each and then randomly sample 1,000 hyperedges. Each hyperedge consists of 15 nodes, among which $\alpha_i$ many are sampled from class $i$. We use $\alpha=\min\{\alpha_1,\alpha_2\}$ to denote the heterophily level. % from two classes with respect to a ratio $\alpha$.
%This ratio determines how many nodes with the same label will be connected by a hyperedge, which controls the homo-/heterophily of the hypergraphs. 
Afterwards, we generate label-dependent Gaussian node features.
We test both homophilic ($\alpha=1,2$ or CE homophily$\ge 0.7$) and heterophilic ($\alpha=4\sim 7$ or CE homophily $\le 0.7$) cases.
We compare \proj with HGNN \cite{feng2019hypergraph}, AllSet models \cite{chien2021you} and their variants with jump links. We follow previous 50\%/25\%/25\% data splitting methods and repeated 10 times the experiment.

\textbf{Results.} Table \ref{tab:syn_node_data} shows the results.
On homophilic datasets, all the models can achieve good results, while \proj keeps slightly better than others. Once $\alpha$ surpasses 3, i.e., entering the heterophilic regime, the superiority of \proj is more obvious. The jump-link trick indeed also helps, while building equivariance as \proj does directly provides more significant improvement.  
% Even for $\alpha = 0.3$ case, where half of neighboring nodes are labelled differently \pan{why this is half?}, our \proj can achieve 90.35\% prediction accuracy.
%Even for $\alpha = 4$ case, our \proj can still achieve 90.35\% prediction accuracy.
%Another interesting finding is that $\alpha = 7$ reaches the maximum tolerance to heterophily of all presented works.
\vspace{-2mm}
\subsection{Benefits in Deepening Hypergraph Neural Networks} \label{sec:depth_benefit}
\vspace{-1mm}
We also demonstrate that by using diffusion models and parameter tying, \proj can benefit from deeper architectures, while other HNNs cannot. % to achieve.
Fig.~\ref{fig:expr_depth} illustrates the performance of different models versus the number of network layers.
We compare with HGNN \cite{feng2019hypergraph}, AllSet models \cite{chien2021you}, and UniGCNII \cite{huang2021unignn}. UniGCNII inherits from~\cite{chen2020simple} which is known to be effective to counteract oversmoothness. The results reveal that AllSet models suffer from going deep. %Once the depth grows larger than 2, their performance declines rapidly.
HGNN working through more lightweight mechanism has better tolerance to depth. However, none of them can benefit from deepening.
On the contrary, \proj successfully leverages deeper architecture to achieve higher accuracy. For example, adding more layers boosts \proj by \textasciitilde1\% in accuracy on Pubmed and House, while elevating \proj from 58.01\% to 64.79\% on Senate dataset.

\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{images/depth.pdf}
\vspace{-3mm}
\small{\caption{Comparing Deep Achitectures across Different Models: Test Acc. v.s. \# Layers}\label{fig:expr_depth}}
\vspace{-3mm}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{images/dim_reduction.pdf}
\vspace{-2mm}
\small{\caption{Comparing the Powers to Represent known Diffusion: MAE v.s. Latent Dimensions}
\label{fig:expr_width}}
\vspace{-4mm}
\end{figure}
\vspace{-2mm}
\subsection{Expressiveness Justification on the Synthetic Diffusion Dataset}
\vspace{-1mm}
We are to evaluate the ability of \proj to express given hypergraph diffusion. We generate semi-synthetic diffusion data using the Senate hypergraph~\cite{chodrow2021hypergraph} and synthetic node features. The data consists of 1,000 pairs $(\Mat{H}^{(0)}, \Mat{H}^{(1)})$. The initial node features $\Mat{H}^{(0)}$ are sampled from 1-dim Gaussian distributions. To obtain $\Mat{H}^{(1)}$ we apply the gradient step in Eq.~\ref{eqn:gd}. For non-differential cases, we adopt subgradients for convenient computation. We fix node potentials as $f(\Mat{h}_v; \Mat{x}_v) = (\Mat{h}_v - \Mat{x}_v)^2$ and consider 3 different edge potentials in Example~\ref{exp:potential} with varying complexities: a) CE, b) TV ($p$=2) and c) LEC. The goal is to let one-layer models $\mathcal{V}\rightarrow\mathcal{E}\rightarrow\mathcal{V}$ to recover $\Mat{H}^{(1)}$.  We compare \proj with our implemented baseline (Invariant) with parameterized invariant set functions on both the node and hyperedge sides, and AllSet models \cite{chien2021you} that also adopt invariant set functions. We keep the scale of all models almost the same to give fair comparison, of which more details are given in Appendix~\ref{sec:diffusion_dataset}. The results are reported in Fig.~\ref{fig:expr_width}. The CE case gives invariant diffusion so all models can learn it well. The TV case mostly shows the benefit of the equivariant architecture, where the error almost does not increase even when the dimension decreases to 32. The LEC case is challenging for all models, though \proj is still the best. The reason, we think, is that learning the sorting operation in LEC via the sum pooling in Eq.~\ref{eq:equi-form} is empirically challenging albeit theoretically doable. A similar phenomenon has been observed in previous literatures~\cite{murphy2018janossy,wagstaff2019limitations}.  



% \begin{itemize}
% \item Equivariant operator:
% \begin{align*}
%     (x_v, x_v^{(0)}, \log d_v,\text{mean}(\text{MLP}_2(x_v, \log |e|, \text{mean}(\text{MLP}_1(x_u))))).
% \end{align*}

% \begin{align*}
% h_e^{(t)} = \text{mean}_u(\text{MLP}_1(h_u^{(t-1)}))\\
% m_{v\leftarrow e}^{(t)}=(h_v^{(t-1)}, \log |e|, h_e^{(t)}) \\
% h_v'^{(t)}= \text{mean}_{e:v\in e}\text{MLP}_2 (m_{v\leftarrow e}^{(t)})\\
% h_v^{(t)}= 
% (h_v^{(t-1)},x_v^{(0)}, \log d_v,h_v'^{(t)})
% \end{align*}

% \item double equi. 
% \begin{align*}
% h_e^{(t)} = \text{mean}_u(\text{MLP}_1(m_{u\rightarrow e}^{(t-1)}))\\
% m_{v\leftarrow e}^{(t)}=(h_v^{(t-1)}, \log |e|, h_e^{(t)}) \\
% h_v^{(t)}= \text{mean}_{e:v\in e}\text{MLP}_2 (m_{v\leftarrow e}^{(t)})\\
% m_{v\rightarrow e}^{(t)}= 
% (h_v^{(t-1)},h_e^{(t)}, x_v^{(0)}, \log d_v, h_v^{(t)})
% \end{align*}

% \end{itemize}

% 1. Synthetic data on one-step hypergraph diffusion to demonstrate the theory. Study the dependence on the model size. 

% 2. Synthetic data on node classification across different heterophilic levels of hypergraphs generated by stochastic block models. 

% 3. Real datasets experiments. 

==> arxiv/section_files/006-conclusion.tex <==
\vspace{-3mm}
\section{Conclusion} 
\vspace{-2mm}
This work introduces a new hypergraph neural network \proj that can model   hypergraph diffusion process. We show that any hypergraph diffusion with permutation-invariant potential functions can be represented by iterating equivariant diffusion operators. \proj provides an efficient way to model such operators based on the commonly-used GNN platforms. \proj shows superiority in processing heterophilic hypergraphs and constructing deep models. For future works, \proj can be applied to other tasks such as hypergraph regression tasks. Or implicit HNNs can be developed to directly optimize the optima of hypergraph diffusion problems.   

==> neurips 2022/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> neurips 2022/section_tex_files/000-abstract.tex <==
   \vspace{-3mm}
\begin{abstract}
    Hypergraph neural networks (HNNs) using neural networks to encode hypergraphs provide a promising way to model higher-order relations in data and further solve relevant prediction tasks built upon such higher-order relations. However, higher-order relations in practice contain complex patterns and are often highly irregular. So, it is particularly challenging to designing an HNN that suffices to express those relations while keeping computational efficiency. Inspired by hypergraph diffusion algorithms, this work proposes a new HNN architecture named \proj, which provably represents any continuous equivariant hypergraph diffusion operators that can model a wide range of higher-order relations. \proj can be implemented efficiently by combining star expansions of hypergraphs with standard message passing neural networks. \proj further shows great superiority in processing heterophilic hypergraphs and constructing deep models. We evaluate \proj for node classification on nine real-world hypergraph datasets. \proj  uniformly outperforms the best baselines over these nine datasets and achieves more than 2\%$\uparrow$ in prediction accuracy over four datasets therein.       
    %The irregularity of those relations also cause computation challenges.   
    %are inpired by the recently designed hypergraph diffusion algorithms and
   % it is often unclear whether they are rc enough to represent certain higher-order relations.  %they could model. Building complicated HNNs 
    
  %Hypergraphs provide the abstraction to study higher-order relations in data. Hypergraph neural networks (HNNs) that use neural networks to encode hypergraph data have recently been investigated for the prediction tasks on hypergraphs. However, the design of HNNs is challenging as it is often unclear what types of higher-order relations in data they could model. On the other hand, too    
\end{abstract}

==> neurips 2022/section_tex_files/001-introduction.tex <==
  \vspace{-2mm}
\section{Introduction} \label{sec:intro}
  \vspace{-1mm}
Machine learning on graphs has recently attracted great attention in the community due to the ubiquitous graph-structured data and the associated inference and prediction problems~\cite{zhu2005semi,zhu2003semi,zhou2004learning,hamilton2020graph,nickel2015review,chami2020machine}. Current works primarily focus on graphs which can model only pairwise relations in data. However, emerging research has shown that higher-order relations that involve more than two entities often reveal much more information in many significant applications~\cite{benson2021higher,schaub2021signal,battiston2020networks,lambiotte2019networks,liu2022neural}. For example, higher-order network motifs build the  fundamental  blocks of many real-world networks~\cite{mangan2003structure,benson2016higher,tsourakakis2017scalable,li2017motif,li2017inhomogeneous}. Session-based (multi-step) behaviors often indicate the preferences of web users more precisely~\cite{xia2021self,wang2021session,wang2020next,wang2022exploiting}. To capture these higher-order relations, hypergraphs provide a dedicated mathematical abstraction~\cite{berge1984hypergraphs}. However, learning algorithms on hypergraphs are still far  underdeveloped as opposed to those on graphs.

Recently, inspired by the success of graph neural networks (GNNs), researchers have started investigating hypergraph neural network models (HNNs)~\cite{feng2019hypergraph,yadati2019hypergcn,dong2020hnhn,huang2021unignn,chien2021you,bai2021hypergraph,arya2020hypersage,yadati2020neural,yang2020hypergraph}. %Similarly to GNNs, HNNs associate the nodes in the hypergraph with vector representations and then keep updating those representations by combining the representations from the neighbors. 
Compared with GNNs, designing HNNs is fundamentally more challenging. First, as aforementioned, higher-order relations modeled by hyperedges could contain very complex information. Second, hyperedges in real-world hypergraphs are often of large and irregular sizes. Therefore, how to effectively represent higher-order relations while efficiently processing those irregular hyperedges is the key question to answer when one is to design HNNs. Unfortunately, just as other types of neural networks (NNs), HNNs look like a black box. Given an HNN, one can hardly tell the type of relations that it can represent and thus often fails to make a suitable tradeoff between the expressiveness and the computational efficiency of the model.        


%effectiveness and efficiency often form a tradeoff.
%However, previous works often designed HNNs based on heuristics, which results in either less expressive models or over-complicated models. We provide a detailed explanation in Sec.~\ref{sec:previous} 

%However, previous works often       
%First, hyperedges are often of large and irregular sizes. How to efficiently   
%as for higher-order relations modeled by the hyperedges, different    design a novel HNN architecture,  
%benchmark the design of HNNs  


In this work, inspired by the recently developed  hypergraph diffusion algorithms~\cite{zhou2007learning,hein2013total,li2020quadratic,liu2021strongly,fountoulakis2021local,takai2020hypergraph,zhang2017re,tudisco2021nonlinear}, we design a novel HNN architecture that holds provable expressiveness to represent a large class of hypergraph diffusion while keeping computational efficiency. Hypergraph diffusion is significant due to its transparency and has been widely applied to clustering~\cite{zhou2007learning,li2017inhomogeneous,li2018submodular}, semi-supervised learning~\cite{hein2013total,zhang2017re,tudisco2021nonlinear,li2018quadratic}, ranking aggregation~\cite{li2017inhomogeneous,chitra2019random}, network analysis~\cite{li2020quadratic,liu2021strongly,fountoulakis2021local,takai2020hypergraph} and signal processing~\cite{zhang2019introducing,schaub2021signal,komodakis2009beyond,werner2008high}. However, traditional hypergraph diffusion needs to first handcraft potential functions to  model higher-order relations and then use their gradients or the variants as the diffusion operators to characterize the exchange of the features of the nodes within one hyperedge. The design of those potential functions often requires significant insights into the applications, which may not be available in practice.

\begin{figure}[t]
    \centering
    \includegraphics[trim={0.3cm 11.7cm 0.1cm 4cm},clip,width=1.\linewidth]{images/Main-Diag.pdf}
    \vspace{-6mm}
    \caption{Hypergraph diffusion often uses permutation-invariant hyperedge potentials to model higher-order relations. The gradients or their variants  of those potentials determine the diffusion process and are termed diffusion operators. Our \proj can universally represent such operators.}
       \vspace{-3mm}
    \label{fig:diag}
\end{figure}

We observe that the most commonly-used hyperedge potential functions are permutation invariant and show that their induced diffusion operators must be permutation equivariant. Therefore, we propose a NN-parameterized permutation-equivariant architecture that can provably represent any continuous hyperedge diffusion operators while the NN parameters can be learned in a data-driven way. We also introduce an efficient implementation of the architecture via current GNN platforms~\cite{FeyPyG,wang2019dgl}, which simply combines a bipartite representation (or star expansion~\cite{agarwal2006higher,zien1999multilevel}, equivalently) of hypergraphs and the standard message passing neural network (MPNN)~\cite{gilmer2017neural}. By repeating this architecture by layers with shared parameters, we build our model Equivariant Diffusion-based HNN (\proj). Fig.~\ref{fig:diag} shows an illustration of hypergraph diffusion and the key architecture in \proj. 

To the best of our knowledge, we are the first one to establish the connection between the general class of hypergraph diffusion algorithms and the design of HNNs. Previous HNNs are either less expressive to represent equivariant diffusion operators~\cite{feng2019hypergraph,yadati2019hypergcn,dong2020hnhn,huang2021unignn,chien2021you,bai2021hypergraph} or need to learn the representations by adding significantly many auxiliary nodes~\cite{arya2020hypersage,yadati2020neural,yang2020hypergraph}. We provide detailed discussion of them in Sec.~\ref{sec:previous}. We also show that due to the equivariant architecture, \proj is by design good at predicting node labels over heterophilic hypergraphs where hyperedges mix nodes from different classes. Moreover, \proj can go very deep without much performance decay. %due to the parameter sharing across layers. 

As a by-product, our proof of expressiveness does not use polynomials as a bridge, which were used previously in set-function approximation~\cite{zaheer2017deepset,maron2018invariant,segol2020universal}. Our statement allows precise representations of continuous equivariant set functions by compositing a continuous function and the sum of another continuous function on each set entry. This result may be of independent interest for the community.         

We evaluate \proj by performing node classsification over 9 real-world hypergraph datasets. \proj uniformly outperforms all baseline methods in averaged performance and achieves significant improvement (more than 2$\%\uparrow$) over 4 datasets therein. \proj also shows super robustness when going deep. We further carefully design synthetic experiments to demonstrate the expressiveness of \proj and the superiority of \proj in processing heterphilic hypergraphs. 

%over... (\pan{Todo: emphasize real-data exp, heterophily and expressiveness}).


% have been proposed~\cite{}, while the  ~\cite{}.
% are proposed to hyperedges have been associated with set functions and Lov\'{a}sz extension-based potentials have found greatly useful~\cite{}.

% so the total-variation potential was proposed and behaved well in the case with large hyperedges~\cite{hein2013total,zhang2017re}. Recently, to model complex higher-order patterns, hyperedges have been associated with set functions and Lov\'{a}sz extension-based potentials have found greatly useful~\cite{}.  


% Hypergraph diffusion has been widely used  


% Finding the minimal potential point, which essentially  

% which may guide the flow  the  
% potential functions  

% make accurate recommendation~\cite{}.        


% 1. Explain the importance of higher-order graph/hypergraph learning. Introduce one or two real-world examples (network motif applications, higher-order MRF).

% 2. Recent works on hypergraph neural networks mainly generalized standard GNNs to hypergraphs and proposed hypergraph neural networks as a black box. Seldom works really investigated into the mechanism and built its connection to white-box hypergraph learning problems. 

% 3. Our work is motivated by the traditional learning algorithm to compute Hypergraph PageRanks and Higher-order MRF MAP. 

% \pan{Move a part to introduction} Hypergraph diffusion has been widely used in data clustering~\cite{zhou2007learning,li2017inhomogeneous,li2018submodular}, semi-supervised learning~\cite{hein2013total,zhang2017re,tudisco2021nonlinear}, ranking aggregation~\cite{li2017inhomogeneous,chitra2019random}, network analysis~\cite{li2018quadratic,liu2021strongly,fountoulakis2021local,takai2020hypergraph}, signal denoising~\cite{zhang2019introducing,schaub2021signal}, inference over higher-order markov random field~\cite{komodakis2009beyond,werner2008high}. 

% \\ We observe that both (sub)gradient descent algorithm and Douglas-Rachford splitting algorithm essentially correspond to iteratively using (permutation) equivariant diffusion operators designed on hyperedges. 
% \\ However, all previous hypergraph neural network models fail to model equivariant diffusion operators on hyperedges and restrict themselves to over-simplified invariant diffusion operators. 
% \\ Not surprisingly, previous models suffer from either limited expressive power or generalization issues induced by over-complex neural network layers to complement the loss of expressive power.   

% 4. In this work, we propose hypergraph neural networks (HNN) based on equivariant diffusion (ED) operators and call the model \proj 
% \\ Each \proj layer contains the following three steps: (1) Learn hyperedge representations via a sum pooling of node representations of each hyperedge; (2) Operate a concatenation of the representations of \emph{each node-hyperedge pair} to compute the messages from hyperedges to nodes; (3) Update node representations via a sum-pooling of the messages.
% \\ The second step is the key to implement ED, which makes our model substantially different from previous HNN models. 
% \\ We may show \proj universally approximates any continuous hypergraph diffusion operators.
% %\\ We systematically study the advantages of using ED. 
% \\ In theory, we further prove that using ED a much smaller latent dimension of node/hyperedge representations is needed to represent hypergraph diffusion than using invariant diffusion (ID). 
% \\ As a by-product, our proof techniques also strengthen the previous argument on the expressive power of equivariant set functions. We avoid using equivariant polynomials and reduce the needed dimensions of the element representations in the set from an exponential order to a linear order.    

% 5. Empirically, we evaluate \proj in two synthetic settings and xxx many real-world hypergraph node classification tasks. \\
% The first synthetic setting shows that ED much better approximate hypergraph diffusion than ID to justify our theory.  \\
% The second synthetic setting shows that ED is extremely good at learning node labels across different heterophilic levels of hypergraphs generated by stochastic block models. \\ 
% ED-GNN also significantly outperforms baselines on real-world hypergraphs by about xxx. 

% \pan{Mention that hypergraph diffusion -> node level tasks, leave graph level tasks for future study}


  

==> neurips 2022/section_tex_files/002-preliminaries.tex <==
   \vspace{-2mm}
\section{Preliminaries: Hypergraphs and Hypergraph Diffusion} \label{sec:prelim}
   \vspace{-1mm}
% We are interested in supervised learning problems on hypergraphs by a diffusion model, in which we are given nodes with features and labels, as well as hyperedges connecting them.

In this section, we formulate the hypergraph diffusion problem, along the way, introduce the notations.
\begin{definition}[Hypergraph] \label{def:hypergraph}
 Let $\Set{G} = (\Set{V}, \Set{E}, \Mat{X})$ be an attributed hypergraph where $\Set{V}$ is the node set of size $N$ and $\Set{E}$ is the hyperedge set of size $M$. Each hyperedge $e = \{v_1^{(e)},...,v_{\lvert e \rvert}^{(e)}\}$ is a subset of $\Set{V}$. Unlike graphs, a hyperedge may contain more than two nodes. $\Mat{X}=[...,\Mat{x}_v,...]^T\in\mathbb{R}^{N}$ denotes the node attributes and $\Mat{x}_v$ denotes the attribute of node $v$. Define $d_v=|\{e\in\mathcal{E}:v\in e\}|$ as the degree of node $v$. Let $\Mat{D},\,\Mat{D}_e$ denote the diagonal degree matrix for $v\in\Set{V}$ and the sub-matrix for $v\in e$.
%Let $\Mat{K} \in \{0, 1\}^{n \times m}$ denote the incident matrix where $\Mat{K}_{ij} = 1$ if and only if $v_i \in e_j$. 
\end{definition}
%A hyperedge $e$ may contain more than two nodes so hypergraphs are used to model higher-order relational data.

Here, we use 1-dim attributes for convenient discussion while our experiments often have multi-dim attributes. Learning algorithms will combine attributes and hypergraph structures into (latent) features defined as follows. These features can be further used to make prediction for downstream tasks.
\begin{definition}[Latent features] \label{def:node_feat}
Let $\Mat{h}_v \in \real$ denote the (latent) features of node $v\in \Set{V}$. The feature vector $\Mat{H} = \begin{bmatrix}..., \Mat{h}_{v}, ... \end{bmatrix}_{v\in\Set{V}}^\top \in \real^{N}$ includes node features as entries. Further, collect the features into a edge feature vector $\Mat{H}_e = \begin{bmatrix} \Mat{h}_{e, 1} & \cdots & \Mat{h}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert}$, where $\Mat{h}_{e,i}$ corresponds to the feature $\Mat{h}_{v_i^{(e)}}$. Note that for any $v\in e$, there is one corresponding index $i\in \{1,...,\lvert e\rvert\}$. Later, we may use subscripts $(e,i)$ and $(e,v)$ interchangeably if there causes no confusion. %For, $i\in [F]$, we use $\Mat{H}_e[i]$ and $\Mat{h}_v[i]$ to denote the corresponding $i$th feature channels.
%collect all the feature vectors of nodes within edge $e$, where $\Mat{h}_{e,i}$ corresponds to the node features of node $v_i^{(e)}$ inside hyperedge $e$. 
%Suppose each node has initial features $\Mat{x}_i \in \real^d$ which are organized by initial feature matrix $\Mat{X} \in \real^{n \times d}$.
\end{definition}

A widely-used heuristic to generate features $\Mat{H}$ is via hypergraph diffusion algorithms. 

\begin{definition}[Hypergraph Diffusion] \label{def:node_feat}
Define node potential functions $f(\cdot;\Mat{x}_v):\mathbb{R} \rightarrow \mathbb{R}$ for $v\in\Set{V}$ and hyperedge potential functions $g_e(\cdot):\mathbb{R}^{|e|} \rightarrow \mathbb{R}$ for each $e\in\Set{E}$.  The hypergrah diffusion combines the node attributes and the hypergraph structure and asks to solve
\begin{align} \label{eqn:diffusion}
    \min_{\Mat{H}} \sum_{v \in \Set{V}} f(\Mat{h}_v; \Mat{x}_v) + \sum_{e \in \Set{E}} g_e(\Mat{H}_e).
\end{align}
In practice, $g_e$ is often shared across hyperedges up-to the size. Later, we ignore the subscript $e$.
\end{definition}

The two potential functions are often designed via heuristics in traditional hypergraph diffusion literatures. Node potentials often correspond to some negative-log kernels of the latent features and the initial attributes. For example, $f(\Mat{h}_v; \Mat{x}_v)$ could be $(\Mat{h}_v - \Mat{x}_v)_2^2$ when to compute hypergraph PageRank diffusion~\cite{li2020quadratic,takai2020hypergraph} or $-\Mat{x}_v\Mat{h}_v$ which essentially computes hypergraph min-cut~\cite{stobbe2010efficient,jegelka2013reflection}. Hyperedge potentials are more significant and complex, as they need to model those higher-order relations between more than two objects. Here list a few examples. 

\begin{example}[Edge potentials] \label{exp:potential}
In practice, hyperedge potential $g(\Mat{H}_e)$ may be chosen as follows. %Note that most previous works only contain one feature channel $F=1$. Here, we list their general variants.
\begin{itemize}[leftmargin=3mm]
    \item Clique Expansion (CE, hyperedges reduced to cliques) plus pairwise potentials~\cite{zhou2007learning}: $\sum_{u,v\in e} (\Mat{h}_v-\Mat{h}_{u})_2^2 $ or with properly degree normalization $\sum_{u,v\in e}(\frac{\Mat{h}_v}{\sqrt{d_v}}-\frac{\Mat{h}_u}{\sqrt{d_u}})_2^2\,(\triangleq g(\Mat{D}_e^{-1/2}\Mat{H}_e))$.\vspace{-0.5mm}
    \item Divergence to the  mean~\cite{tudisco2021nonlinear,tudisco2021nonlinear2}: $\sum_{v\in e} (\Mat{h}_v-\||e|^{-1}\Mat{H}_e\|_p)_2^2$, where $\|\cdot\|_p$ computes the $\ell_p$-norm. \vspace{-0.5mm} %each feature channel of $\Mat{H}_e$ separately.% where the number of features channels is $F=1$.
    \item Total Variation (TV)~\cite{hein2013total,zhang2017re,takai2020hypergraph}: $\max_{u,v\in e} |\Mat{h}_v-\Mat{h}_u|^p$, $p\in\{1,2\}$. \vspace{-0.5mm}% where the number of features channels is $F=1$.
    \item Lov\'{a}sz Extension~\cite{lovasz1983submodular} for cardinality-based set functions (LEC)~\cite{jegelka2013reflection,li2018submodular,li2020quadratic,liu2021strongly}: $\langle \Mat{y}, \varsigma(\Mat{H}_e) \rangle^p$, $p\in\{1,2\}$ where $\Mat{y}=\begin{bmatrix} ...,\Mat{y}_j,... \end{bmatrix}^\top\in\mathbb{R}^{|e|}$ is a constant vector and $\varsigma(\Mat{H}_e)$ sorts the values of $\Mat{H}_e$ in a decreasing order.% is also in a decreasing order, i.e., $y_j\geq \Mat{y}_{j+1}$, $\forall j\in[e-1]$. %Here, suppose  $\Mat{y}_{|e|+1}=0$\, for convenience.
    %\item Lov\'{a}sz Extension for cardinality-based set functions  (LE)~\cite{lovasz1983submodular,jegelka2013reflection,li2018revisiting,li2018quadratic}: $\sum_{i=1}^F\max_{\Mat{y}_i\in \Set{B}_e}\langle \Mat{y}_i, \Mat{H}_e[i] \rangle^p$, $p\in\{1,2\}$, where  $\Set{B}_e\subset\mathbb{R}^{|e|}$ is the base polytope induced by a submodular function defined on $e$. This generalizes total variation. 
\end{itemize}\vspace{-2mm}
\end{example}
One may reproduce TV by using LEC and setting $\Mat{y}_1=-\Mat{y}_{|e|}=1$.
To reveal more properties of these hyperedge potentials $g(\cdot)$, we list the following formal definitions.

%Heuristic $g(\cdot)$'s are complicated while they all satisfies permutation invariance defined as follows.  %To reveal more properties of $g(\cdot)$, we list the following formal definitions:

% \begin{definition} \label{def:permutation}
% Let $\pi: [K] \rightarrow [K]$ be an automorphism, then permutation matrix  is defined as $\Mat{P}_{\pi}$ who has value one at entries $(\pi(i),i), \forall i \in [K]$ while taking zero at any other positions.
% A permutation group $\Pi[K]$ is defined as a set which collects all of such $\Mat{P}_\pi$.
% \end{definition}

% \begin{definition}[Permutation Invariance \& Equivariance] \label{def:permutation_ivariant} 
% Function $\psi: \mathbb{R}^{K\times F} \rightarrow \real^{F'}$ is permutation-invariant if for any $K$-dim permutation matrix $\Mat{P}\in\Pi[K]$, %$\,\forall \Mat{P} \in \Pi[K]$ denote permutation matrix, 
% $\psi(\Mat{P} \Mat{Z}) = \psi(\Mat{Z})$ for all $\Mat{Z} \in \mathbb{R}^{K\times F}$. Function $\psi: \mathbb{R}^{K\times F} \rightarrow \mathbb{R}^{K\times F'}$ is permutation-equivariant if for any $K$-dim permutation matrix $\Mat{P}\in\Pi[K]$, $\psi(\Mat{P} \Mat{Z}) = \Mat{P}\psi(\Mat{Z})$ for all $\Mat{Z} \in \mathbb{R}^{K\times F}$.
% \end{definition}
\begin{definition}[Permutation Invariance \& Equivariance] \label{def:permutation_ivariant} 
Function $\psi: \mathbb{R}^{K} \rightarrow \real$ is permutation-invariant if for any $K$-dim permutation matrix $\Mat{P}\in\Pi[K]$, %$\,\forall \Mat{P} \in \Pi[K]$ denote permutation matrix, 
$\psi(\Mat{P} \Mat{Z}) = \psi(\Mat{Z})$ for all $\Mat{Z} \in \mathbb{R}^{K}$. Function $\psi: \mathbb{R}^{K} \rightarrow \mathbb{R}^{K}$ is permutation-equivariant if for any $K$-dim permutation matrix $\Mat{P}\in\Pi[K]$, $\psi(\Mat{P} \Mat{Z}) = \Mat{P}\psi(\Mat{Z})$ for all $\Mat{Z} \in \mathbb{R}^{K}$.
\end{definition}

%\begin{definition} \label{def:permutation_equivariant} (Permutation Equivariance)
%Let $f: \real^k \rightarrow \real^k$ be a permutation-equivariant function, then $\forall \Mat{P} \in \Grp{P}_k$, $f(\Mat{P} \Mat{x}) = \Mat{P} f(\Mat{x})$ for all $\Mat{x} \in \real^k$.
%\end{definition}

%Here, $F,F'$ could be any positive integers, which become clear based on the context. 
We may easily verify permutation invariance of the hyperedge potentials in Example~\ref{exp:potential}. The physical meaning behind this observation is that the prediction goal of an application is often independent of node identities in a hyperedge so practical $g$'s often keep invariant w.r.t. the node ordering~\cite{veldt2020hypergraph}.
%affect the diffusion results.   

%We note that potential function $g(\cdot)$ should be permutation-invariant since row permutation of the edge feature matrix results in an equivalent class. \pan{This may be more natural put with g definition together.}
%No matter in which order we arrange data inside $\Mat{H}_e$, $g(\cdot)$ should give the identical potential value. 




% Here are a few examples. 
% \begin{example}[Node potentials]
% The node potential $f(\Mat{h}_v; \Mat{x}_v)$ often corresponds to a negative-log kernel of the latent features and the initial attributes: (a) Hypergraph PageRank diffusion~\cite{li2018quadratic,takai2020hypergraph}, $\|\Mat{h}_v - \Mat{x}_v\|_2^2$; (b) Hypergraph min-cut diffusion~\cite{stobbe2010efficient}, $-\Mat{h}_v^T\Mat{x}_v$.
% \end{example}

% For example, node potential $f(\Mat{h}_v; \Mat{x}_v)$ could be $\|\Mat{h}_v - \Mat{x}_v\|_2^2$ when to compute hypergraph PageRank diffusion~\cite{li2018quadratic,takai2020hypergraph} or $-\Mat{h}_v^T\Mat{x}_v$ to compute hypergraph cut~\cite{stobbe2010efficient}. Examples of edge potentials $g(\Mat{H}_e)$ include a combination of clique expansion and pairwise potentials $\sum_{u,v\in e} \|\Mat{x}_v-\Mat{x}_u\|_2^2$, Lov\'{a}sz extension and \cite{tudisco2021nonlinear}.   

% (Heuristics, cannot apply to heterophilic)

% hypergraph diffusion include hypergraph  

% Node potential: $f_v(\cdot ;x_v)$: $\mathbb{R}^{m} \rightarrow \mathbb{R}.$ %We assume that $f_v = f_{u}$ if the node degree $d_v = d_{u'}$.
%     \item hyperedge potential: $g_e(\cdot): \mathbb{R}^{|e|\times m}\times \mathbb{R}$. %We
%     %Denote $\bar{z} =(z_1,z_2^{(e)},...,z_|e|^{(e)})$ where $z_{i}^{(e)}$ is the block of the input vector $\bar{z}_e$ associated with node $v_{i}^{(e)}$.
    
%     \item In hypergraphs, we often do not have node identities so $f_v=f_u$ if $d_v= d_{u}$. We also assume that $g_e = g_{e'}$ if $|e| = |e'|$ and $g_{e}$ is permutation invariant: $g_e(\bar{h}_e) = g_e(\bar{h}'_e)$ if $\{\Mat{h}_v|v\in e\}=\{\Mat{h}_v'|v\in e\}$. As the information of node degrees and hyperedge sizes are clear, we simply use $f$ and $g$ to uniformly denote node potentials and hyperedge potentials respectively.

% Unlike ordinary graphs, a hyperedge can connect with more than two nodes, i.e., $\lvert e \rvert \ge 2$.
% To attain node adjacent matrix (i.e., an $n$ by $n$ matrix whose non-zero entries indicate which two nodes are connected), one can use $\Mat{K}\Mat{K}^\top$ that transforms hyperedges into cliques.
% \begin{definition}[Node features] \label{def:node_feat}
% Let $\Mat{h}_i \in \real^d$  \pan{revise to $F$} be the node embedding of the node $v_i \in \Set{V}$. We organize all the node features into the rows of a feature matrix $\Mat{H} = \begin{bmatrix} \Mat{h}_{1} & \cdots & \Mat{h}_{n} \end{bmatrix}^\top \in \real^{n \times d}$. Suppose each node has initial features $\Mat{x}_i \in \real^d$ which are organized by initial feature matrix $\Mat{X} \in \real^{n \times d}$.
% \end{definition}

% % Similarly, we let matrix $\Mat{H} = \begin{bmatrix} \Mat{h}_{1} & \cdots & \Mat{h}_{n} \end{bmatrix}^\top \in \real^{n \times d}$ concatenates all the node features after diffusion.
% \begin{definition}[Edge features] \label{def:edge_feat}
% % Given an hyperedge $e \in \Set{E}$, the 
% Let edge feature matrix $\Mat{H}_e = \begin{bmatrix} \Mat{h}_{e, 1} & \cdots & \Mat{h}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert \times d}$ collect all the feature vectors of nodes within edge $e$, where $\Mat{h}_{e,i}$ corresponds to the node features of node $v_i^{(e)}$ inside hyperedge $e$. \pan{Define the relation between $\Mat{h}_{e}$ and $\Mat{h}$. Denote an implicit mapping between $(e,i)$ and $(e,v)$.}
% \end{definition}

% Hypergraph diffusion algorithms solve node embeddings \pan{unify the terminology} $\Mat{H}$ to minimize some potential functions \pan{add some background} defined over hypergraphs.
% We proposed a general hypergraph diffusion model \pan{Review hypergraph diffusion instead of proposing a model; Also motivates the applications of this is crucial.} that accumulates potential of individual node embeddings and the joint potential among nodes connected by each hyperedge in a hypergraph $\Set{G}$:
% \begin{align} \label{eqn:diffusion}
%     \min_{\Mat{H}} \sum_{v \in \Set{V}} f(\Mat{h}_v; \Mat{x}_v) + \sum_{e \in \Set{E}} g(\Mat{H}_e),
% \end{align}
% where $f: \real^{d} \rightarrow \real$ denotes the node potential function, which defines an independent likelihood of each node representation, $g
% : \real^{\lvert e \rvert \times d} \rightarrow \real$ is the hyperedge potential function \pan{different hyperedges may have different sizes}, which specifies a joint constraints on the embeddings of nodes connected by one hyperedge.
% \textcolor{red}{High-Order Page Rank}.
% \textcolor{red}{High-Order Markov Random Field}.

% To optimize Eq.~\eqref{eqn:diffusion}, it is often to use gradient-based methods which we will elaborate in Sec. \ref{sec:model} \pan{Need better motivations, add references and discuss previous approaches; Okay, we should put this into the next section.}. 
% Suppose $f(\cdot)$ and $g(\cdot)$ are differentiable, then we denote the gradient of $f(\cdot)$ taking value at $\Mat{h}_v$ as: $\nabla f(\Mat{h}_v; \Mat{x}) = \frac{\partial f(\Mat{z}; \Mat{x})}{\partial \Mat{z}} \lvert_{\Mat{z} = \Mat{h}_v}$,
% and since $g(\cdot)$ is a function of a set of nodes, its partial derivative with respect to node $v$ taking value at $\Mat{H}_e$ is defined as: $\nabla_v g(\Mat{H}_e) = \nabla_v g\left(\Mat{h}_{e, 1}, \cdots, \Mat{h}_{e,\lvert e \rvert}\right) = \frac{\partial_v g\left(\Mat{z}_{e, 1}, \cdots, \Mat{z}_{e, \lvert e \rvert}\right)}{\partial \Mat{z}_{e, v}} \Big\lvert_{\Mat{z}_{e,i} = \Mat{h}_{e,i}}$ \pan{I think this notation may have some issues.}.
% To reveal more properties of $g(\cdot)$, we list the following formal definitions:

% \begin{definition} \label{def:permutation}
% Let $\pi: [k] \rightarrow [k]$ be an automorphism, then permutation matrix  is defined as $\Mat{P}_{\pi}$ who has value one at entries $(i, \pi(i)), \forall i \in [k]$ while taking zero at any other positions.
% A permutation group $\Grp{P}_k$ \pan{revise to $\Pi[k]$} is defined as a set which collects all of such $\Mat{P}_\pi$.
% \end{definition}

% \begin{definition} \label{def:permutation_ivariant} (Permutation Invariance)
% Let $f: \real^k \rightarrow \real$ be a permutation-invariant function, then $\forall \Mat{P} \in \Grp{P}_k$, $f(\Mat{P} \Mat{x}) = f(\Mat{x})$ for all $\Mat{x} \in \real^k$.
% \end{definition}

% \begin{definition} \label{def:permutation_equivariant} (Permutation Equivariance)
% Let $f: \real^k \rightarrow \real^k$ be a permutation-equivariant function, then $\forall \Mat{P} \in \Grp{P}_k$, $f(\Mat{P} \Mat{x}) = \Mat{P} f(\Mat{x})$ for all $\Mat{x} \in \real^k$.
% \end{definition}

% We note that potential function $g(\cdot)$ should be permutation-invariant since row permutation of the edge feature matrix results in an equivalent class. \pan{This may be more natural put with g definition together.}
% No matter in which order we arrange data inside $\Mat{H}_e$, $g(\cdot)$ should give the identical potential value. 



% \begin{itemize}
%     \item Attributed hypergraphs: $\gG=(V,E,X)$.  $X\in\mathbb{R}^{|V|\times m}$. $x_v$ denotes the attributes for node $v$. A hyperedge $e\in E$ is a subset of nodes $e=\{v_1^{(e)},...,v_{|e|}^{(e)}\}\subseteq V$ where $|e|$ is the hyperedge size. %(Start from 1-dim case for simplicity).
    
%     \item Define node-diffused matrix $H\in\mathbb{R}^{|V|\times m}$ where $\Mat{h}_v$ denotes the row for node $v$. Given $e\in E$, we use notation bar-subscript $\bar{h}_e\in \mathbb{R}^{|e|\times m}$ to denote  concatenation $\oplus_{v\in e} \Mat{h}_v$ whose $i$th block is $\Mat{h}_{v_i^{(e)}}$. We also use the subscript without bar $q_e\in \mathbb{R}^{|e|\times m}$ to denote concatenation of $\oplus_{v\in e} q_{e,v}$ where $q_{e,v}\in \mathbb{R}^{m}$ which is a representation for a hyperedge-node pair.
    
    
%     %= (\Mat{h}_{v_1^{(e)}},...,\Mat{h}_{v_|e|^{(e)}})$. %where $z_i = \Mat{h}_{v_i^{(e)}}$ for $i\in[e]$.
    
%     \item Node potential: $f_v(\cdot ;x_v)$: $\mathbb{R}^{m} \rightarrow \mathbb{R}.$ %We assume that $f_v = f_{u}$ if the node degree $d_v = d_{u'}$.
%     \item hyperedge potential: $g_e(\cdot): \mathbb{R}^{|e|\times m}\times \mathbb{R}$. %We
%     %Denote $\bar{z} =(z_1,z_2^{(e)},...,z_|e|^{(e)})$ where $z_{i}^{(e)}$ is the block of the input vector $\bar{z}_e$ associated with node $v_{i}^{(e)}$.
    
%     \item In hypergraphs, we often do not have node identities so $f_v=f_u$ if $d_v= d_{u}$. We also assume that $g_e = g_{e'}$ if $|e| = |e'|$ and $g_{e}$ is permutation invariant: $g_e(\bar{h}_e) = g_e(\bar{h}'_e)$ if $\{\Mat{h}_v|v\in e\}=\{\Mat{h}_v'|v\in e\}$. As the information of node degrees and hyperedge sizes are clear, we simply use $f$ and $g$ to uniformly denote node potentials and hyperedge potentials respectively.% by removing the subscripts for simplicity.
    
    
%     %where $Z_e\in \mathbb{R}^{|e|\times m}$ and $P$ is a $|e|$-by-$|e|$ permutation matrix. As the information of node degrees and hyperedge sizes are clear, we simply use $f$ and $g$ by removing the subscripts for simplicity.
%     %if $\{z_1^{(e)},z_2^{(e)},...,z_{|e|}^{(e)}\}=\{z_1'^{(e)},z_2'^{(e)},...,z_{|e|}'^{(e)}\}$. %In the following, for simplicity, our discussion focus on uniform hypergraphs, though experiments may have non-uniform hypergraphs. So we denote $g_e = g$ for simplicity.
% \end{itemize}

% \paragraph{Hypergraph Convolutional Networks}
% Graph neural networks (GNN) are broadly adopted for learning problems on graphs.
% Recent works \cite{feng2019hypergraph, bai2021hypergraph, yadati2019hypergcn, dong2020hnhn, huang2021unignn} have generalized various GNNs for ordinary graphs onto hypergraphs.
% Nevertheless, most of existing hypergraph convolution are based on clique expansion propagation with degree normalization and nonlinear transformation.
% Taking HGNN \cite{feng2019hypergraph} for an example, it has the following node-wise update formula for each layer:
% \begin{align} \label{eqn:hgnn}
%     \Mat{h}_v^{(t+1)} = \sigma\left( \frac{1}{\sqrt{d_v}} \sum_{e: v \in e} \frac{1}{\lvert e \rvert} \sum_{u: u \in e} \frac{\Mat{h}_u^{(t)}}{\sqrt{d_u}} \Mat{\Theta}^{(t)} + \Mat{b}^{(t)} \right),
% \end{align}
% where $\Mat{h}_v^{(t)}$ denotes the features of node $v$ at the $t$-th layer, $d_v$ denotes the degree of node $v$, $\sigma$ is a non-linear activation, and $\Mat{\Theta}^{(t)}, \Mat{b}^{(t)}$ are parameters of linear transformation and bias, respectively.
% We argue that each layer's update (Eq. \ref{eqn:hgnn}) can be regarded as an optimization step of a special case of objective Eq. \ref{eqn:diffusion}.
% We show this by letting $g(\Mat{Z}_e) = \sum_{(v, u) \in e} \lVert \Mat{h}_v^{(e)}/\sqrt{d_v} - \Mat{h}_u^{(e)}/\sqrt{d_u} \rVert_2^2$ and $f(\Mat{h}_v; \Mat{x}_v) = 0$.
% Since $g$ is strongly convex, we can reach optimum by gradient descent. And the gradient step will coincide with Eq. \ref{eqn:hgnn} in form.
% \textcolor{red}{need a derivation and correction later.}
% \textcolor{red}{add AllSet?}

% \paragraph{Nonlinear Hypergraph Diffusion (HyperND)}




==> neurips 2022/section_tex_files/003-model.tex <==
 % \vspace{-2mm}
\section{Neural Equivariant Diffusion Operators and \proj} \label{sec:model}
 % \vspace{-1mm}
Previous design of hyperedge potential functions is tricky. Early works adopted clique or star expansion by reducing hyperedges into (weighted) edges~\cite{zhou2007learning,agarwal2006higher,li2017inhomogeneous} and further used edge potentials. Later, researchers proved that those hyperedge reduction techniques cannot well represent higher-order relations~\cite{li2017inhomogeneous,chien2019hs}. Therefore, Lov\'{a}sz extensions of set-based cut-cost functions on hyperedges have been proposed recently used as the potential functions~\cite{hein2013total,li2018submodular,li2020quadratic,takai2020hypergraph,liu2021strongly,fountoulakis2021local}. However, designing those set-based cut cost is practically hard and needs a lot of trials and errors. Other types of handcrafted hyperedge potentials to model information propagation can be found in~\cite{neuhauser2022consensus,neuhauser2021opinion}. %which again are handcrafted and heavily based on heuristics and evaluation performance. 

%~\cite{li2018submodular}, and  Lov\'{a}sz extensions of those set functions are further
%Hypergraph diffusion has been widely used in applications. However, heuristic design of the potential functions requires significant insights into the applications. For example, early works often adopted clique or star expansion by reducing hypergraphs into graphs~\cite{zhou2007learning,star}. Later, researchers found that such graph reduction techniques often generate huge distortion of hypergraph cut functions ~\cite{li2017inhomogeneous}, so total variation was proposed and behaved well in the case with large hyperedges~\cite{hein2013total,zhang2017re}. Recently, to model complex higher-order patterns, e.g., the hierarchy of foodweb networks~\cite{}, hyperedges have been associated with set functions and Lov\'{a}sz extension-based potentials have found greatly useful~\cite{}. Particularly for node classification tasks, as opposed to the edge case that connects two nodes from either the same or different categories, hyperedges may consist of nodes from multiple categories with various ratios, which makes handcrafting potentials far more complicated.    

Our idea uses data-driven approaches to model such potentials, which naturally brings us to HNNs. On one hand, we expect to leverage the extreme expressive power of NNs to learn the desired hypergraph diffusion automatically from the data. On the other hand, we are interested in having novel hypergraph NN (HNN) architectures inspired by traditional hypergraph diffusion solvers. 

To achieve the goals, next, we show by the gradient descent algorithm (GD) or alternating direction method of multipliers (ADMM)~\cite{boyd2011distributed}, solving objective Eq.~\ref{eqn:diffusion} amounts to iteratively applying some hyperedge diffusion operators. Parameterizing such operators using NNs by each step can unfold hypergraph diffusion into an HNN. We make the key observation that the diffusion operators are inherently \textit{permutation-equivariant}. To universally represent them, we propose a standard form to design  equivariant NN-based operators and use it to build \proj via an efficient implementation. %By repeating this computational unit, we construct our Equivariant Diffusion-based HNN, dubbed \proj.

%To the best of our knowledge, \proj is the first one to adopt equivariant hyperedge-processing architecture. All previous HGNN models adopt permutation-invariant hyperedge operation, which limits their power to represent general hypergraph diffusion. Although a very recent work proposed to view each hyperedge as a multi-set so building multi-set equivariant operator is a natural thought~\cite{chien2021you}, no specific equivariant achitecture was proposed albeit universally representable as \proj guarantees. As a by product, our representation theory complements the previous studies on set-function representation~\cite{segol2020universal} and~\cite{zaheer2017deepset}. Our proof technique avoids using equivariant polynomial approximation and thus allows a precise representation of continuous equivariant set functions by composing a continuous function and the sum of another continuous function on each set entry.         



%Theoretically, 

%hypergraph diffusion process.   

%Specifically, given a hypergraph with initial values defined on the nodes, design potential functions that characterize higher-order relations reflected by the hyperedges. Then, diffuse the node values across hyperedges to decrease the total potential of the hypergraph. The convergent values that achieve minimal total potential encode all the higher-order relations and can be further used to make prediction. Hypergraph diffusion is significant due to the transparency of the algorithms and has found applications in  clustering~\cite{zhou2007learning,li2017inhomogeneous,li2018submodular}, semi-supervised learning~\cite{hein2013total,zhang2017re,tudisco2021nonlinear}, ranking aggregation~\cite{li2017inhomogeneous,chitra2019random}, network analysis~\cite{li2018quadratic,liu2021strongly,fountoulakis2021local,takai2020hypergraph}, signal denoising~\cite{zhang2019introducing,schaub2021signal} and image processing~\cite{komodakis2009beyond,werner2008high}.

%However, designing good potential functions often requires significant insights into the applications. Early works often adopted clique or star expansion by reducing hypergraphs into graphs~\cite{zhou2007learning,star,li2017inhomogeneous} and adopt  graph potentials. Later, researchers proved that those graph reduction techniques can hardly well represent higher-order relations~\cite{li2017inhomogeneous,chien2019}. Therefore, recently, set-based costs on hyperedges have been proposed~\cite{}, and  Lov\'{a}sz extension of those set functions can be used as the potential functions~\cite{}. However, how to design those set-based costs are practically hard and need a lot of trials and errors. Other types of hyperedge potentials to model the divergence of node values and information propagation can be found in~\cite{}, which are all handcrafted and heavily based on heuristics. 

% We show that hypergraph diffusion operators are inherently \textit{permutation-equivariant}.


% the traditional solvers of Eq.~\eqref{eqn:diffusion} based on the gradient descent algorithm (GD) and alternating direction method of multipliers (ADMM). We observe that 

% show by using gradient descent algorithm or Douglas-Rachford splitting algorithm, solving objective Eq. \ref{eqn:diffusion} amounts to iteratively applying hypergraph diffusion operators.
% Parameterizing such diffusion operators using neural networks by each step can unfold the optimization algorithm to be a Hypergraph Neural Network (HGNN).  \pan{Inspire our work}
% We show that hypergraph diffusion operators are inherently \textit{permutation-equivariant}.
% To universally represent them, we propose a standard form of equivariant mapping and follow this form to design our permutation-equivariant neural networks.
% By repeating this computational unit, we construct our Equivariant Diffusion-based Hypergraph Neural Network, dubbed ED-HGNN.

% Therefore, the key motivation of our approaches is whether we may use data-driven approaches, neural networks specifically, to automatically learn the desired hypergraph diffusion. On the other hand, we are also interested in having novel hypergraph neural network architectures inspired by traditional hypergraph diffusion solvers. 

% %inspire the design of hypergraph neural network models?


% %\pan{Claim how to implement equi hyperedge operator is non-trivial. Previous works are regular. Moreover, standard model, do not need to worry this.}


% We are interested in supervised representation learning on hypergraphs.
% In this section, we show by using gradient descent algorithm or Douglas-Rachford splitting algorithm, solving objective Eq. \ref{eqn:diffusion} amounts to iteratively applying hypergraph diffusion operators.
% Parameterizing such diffusion operators using neural networks by each step can unfold the optimization algorithm to be a Hypergraph Neural Network (HGNN).  \pan{Inspire our work}
% We show that hypergraph diffusion operators are inherently \textit{permutation-equivariant}.
% To universally represent them, we propose a standard form of equivariant mapping and follow this form to design our permutation-equivariant neural networks.
% By repeating this computational unit, we construct our Equivariant Diffusion-based Hypergraph Neural Network, dubbed ED-HGNN.
\vspace{-2mm}
\subsection{Emerging Equivariance in Hypergraph Diffusion}
\label{sec:emerge_equivariance}
\vspace{-1mm}
We start with discussing the traditional solvers for Eq. \ref{eqn:diffusion}. If $f$ and $g$ are both differentiable, one straightforward optimization approach is to adopt gradient descent. The node-wise update of each iteration can be formulated as below:
\begin{align} \label{eqn:gd}
    \Mat{h}_v^{(t+1)} \leftarrow \Mat{h}_v^{(t)} - \eta (\nabla f(\Mat{h}_v^{(t)}; \Mat{x}_v) + \sum_{e: v\in e} [\nabla g(\Mat{H}_e^{(t)})]_v), \quad \text{for}\; v\in \Set{V},
\end{align}
where $[\nabla g(\Mat{H}_e)]_v$ denotes the gradient w.r.t. $\Mat{h}_v$ for $v\in e$. We use the supscript $t$ to denote the number of the current iteration, $\Mat{h}_v^{(0)} = \Mat{x}_v$ is the initial features, and $\eta$ is known as the step size.

For general $f$ and $g$, we may adopt ADMM~\cite{boyd2011distributed}: For each $e\in\Set{E}$, we introduce an auxiliary variable $\Mat{Q}_e = \begin{bmatrix} \Mat{q}_{e,1} & \cdots & \Mat{q}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert}$. We initialize $\Mat{h}_v^{(0)}=\Mat{x}_v$ and $\Mat{Q}_e^{(0)}=\Mat{H}_e^{(0)}$. And then, iterate 
%We introduce $\Mat{Q}_e = \Mat{S}_e^{(t)} + \Mat{R}_e^{(t+1)}$ as an intermediate auxiliary variable. 
%This problem can be solved via ADMM: Introducing $\Mat{Q}_e = \Mat{S}_e^{(t)} + \Mat{R}_e^{(t+1)}$ an intermediate variable,
\begin{align} \label{eqn:admm-q}
    \Mat{Q}_e^{(t+1)} &\leftarrow  \prox_{\eta g}(2\Mat{H}_e^{(t)} - \Mat{Q}_e^{(t)}) - \Mat{H}_e^{(t)} + \Mat{Q}_e^{(t)}, \quad \text{for}\; e\in \Set{E}, \\ \label{eqn:admm-h}
    \Mat{h}_v^{(t+1)} &\leftarrow  
    \prox_{\eta f(\cdot;\Mat{x}_v)/d_v}(\sum_{e:v\in e}\Mat{q}_{e,v}^{(t+1)}/d_v), \quad \text{for}\; v\in \Set{V},
\end{align}
where $\prox_{\psi}(\Mat{h}) \triangleq \arg\min_{\Mat{z}} \psi(\Mat{z}) + \frac{1}{2}\|\Mat{z}-\Mat{h}\|_2^2$ is the proximal operator. The detailed derivation can be found in Appendix~\ref{sec:ADMM-derive}. Note that hypergraph diffusion algorithms based on primal-dual hybrid gradient descent~\cite{hein2013total} or alternative projection~\cite{li2018revisiting,li2020quadratic} are close variants of ADMM. 
The operator $\prox_{\psi}(\cdot)$ has nice  properties as reviewed in Proposition~\ref{prop:prox}, which enables the NN-based approximation even if $f$ and $g$ are not differentiable, e.g., the LEC case when $g(\Mat{H}_e)=\langle \Mat{y}, \varsigma(\Mat{H}_e) \rangle^p$. %However, previous heuristics of $g$ expect divergence to the mean are convex.
\begin{proposition}[\cite{parikh2014proximal,polson2015proximal}]\label{prop:prox}
If $\psi(\cdot):\mathbb{R}^K\rightarrow \mathbb{R}$ is a lower semi-continuous convex function, then $\prox_{\psi}(\cdot)$ is 1-Lipschitz continuous. 
\end{proposition}



The node-side operations, gradient $\nabla f(\cdot;\Mat{x}_v)$ and proximal gradient $\prox_{\eta f(\cdot;\Mat{x}_v)}(\cdot)$ are relatively easy to model, while the operations on hyperedges are more complicated. We name gradient $\nabla g(\cdot):\mathbb{R}^{|e|}\rightarrow \mathbb{R}^{|e|}$ and proximal gradient $\prox_{\eta g}(\cdot):\mathbb{R}^{|e|}\rightarrow \mathbb{R}^{|e|}$ as  \textit{hyperedge diffusion operators}, since they summarize the collection of node features inside a hyperedge and dispatch the aggregated information to interior nodes individually. %These hyperedge diffusion operators can be intuitively interpreted as a (one-hop) information fusion among nodes connected by some hyperedge.
Next, we reveal one crucial property of those hyperedge diffusion operators by the following propostion (see the proof in Appendix~\ref{sec:proof-equi-op}):
\begin{proposition} \label{prop:equivariant_op}
 Given any permutation-invariant hyperedge potential function $g(\cdot)$, hyperedge diffusion operators $\prox_{\eta g}(\cdot)$ and $\nabla g(\cdot)$  are permutation equivariant.
\end{proposition}
%We provide the proof of Proposition \ref{prop:equivariant_op} in Appendix~\ref{sec:proof-equi-op}. 
It states that an operator defined on a hyperedge should not only aggregate features regardless of the node order, but also pass messages to different nodes in a permutation-equivariant way. 






% We initialize $\Mat{h}_v^{(0)}=\Mat{x}_v$ and $\Mat{Q}_e^{(0)}=\Mat{H}_e^{(0)}$. 

% . Then, 


% A common strategy to solve Eq. \ref{eqn:alm} is to minimize $\Mat{H}_e$ and $\Mat{R}_e$ alternatively, which induces a form of Alternating Direction Method of Multipliers (ADMM) as below \pan{reference, node degree was not defined.}:
% \begin{align} \label{eqn:admm}
%     \Mat{Q}_e^{(t+1)} &\leftarrow  \prox_{g,\frac{1}{\lambda}}(2\Mat{H}_e^{(t)} - \Mat{Q}_e^{(t)}) - \Mat{H}_e^{(t)} + \Mat{Q}_e^{(t)} \\
%     \Mat{h}_v^{(t+1)} &\leftarrow  
%     \prox_{\frac{1}{f,\lambda d_v}}\left(\frac{1}{d_v}\sum_{e:e\in v}\Mat{q}_{e,v}^{(t)};\pan{x_v}\right),
% \end{align}
% where we introduce $\Mat{Q}_e = \Mat{S}_e^{(t)} + \Mat{R}_e^{(t+1)} = \begin{bmatrix} \Mat{q}_{e,1} & \cdots & \Mat{q}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert \times d} $ as an intermediate auxiliary variable. The detailed derivation can be found in the \textcolor{red}{Appendix}.





% %$\Mat{R}_e = \Mat{H}_e$ for every $e \in \Set{E}$.

% not necessarily differentiable (e.g., $g$ penalizes the maximal element), which hinders us to reach the minimum via simple gradient descent.
% When $g(\Mat{H}_e)$ is non-differentiable, we solve this problem using Augmented Lagrangian Method (ALM) \pan{reference}.
% We first introduce dual variables $\Mat{S}_e \in \real^{\lvert e \rvert \times d}$ and duplicate the hyperedge features $\Mat{H}_e$ into $\Mat{R}_e = \begin{bmatrix} \Mat{r}_{e,1} & \cdots & \Mat{r}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert \times d}$ such that $\Mat{R}_e = \Mat{H}_e$ for every $e \in \Set{E}$.
% Then by ALM, our primal problem can be derived as:
% \begin{align} \label{eqn:alm}
% \pan{\max_{S_e}\min_{R_e,H}}\sum_{v\in \Set{V}} f(\Mat{h}_v; \Mat{x}_v) + \sum_{e\in \Set{E}} g(\Mat{R}_e) +  \frac{\lambda}{2}\sum_{e\in \Set{E}}\lVert \Mat{R}_e - \Mat{H}_e + \Mat{S}_e\ \Vert_2^2 - \frac{\lambda}{2}\sum_{e\in \Set{E}} \lVert \Mat{S}_e \rVert^2.
% \end{align}
% A common strategy to solve Eq. \ref{eqn:alm} is to minimize $\Mat{H}_e$ and $\Mat{R}_e$ alternatively, which induces a form of Alternating Direction Method of Multipliers (ADMM) as below \pan{reference, node degree was not defined.}:
% \begin{align} \label{eqn:admm}
%     \Mat{Q}_e^{(t+1)} &\leftarrow  \prox_{g,\frac{1}{\lambda}}(2\Mat{H}_e^{(t)} - \Mat{Q}_e^{(t)}) - \Mat{H}_e^{(t)} + \Mat{Q}_e^{(t)} \\
%     \Mat{h}_v^{(t+1)} &\leftarrow  
%     \prox_{\frac{1}{f,\lambda d_v}}\left(\frac{1}{d_v}\sum_{e:e\in v}\Mat{q}_{e,v}^{(t)};\pan{x_v}\right),
% \end{align}
% where we introduce $\Mat{Q}_e = \Mat{S}_e^{(t)} + \Mat{R}_e^{(t+1)} = \begin{bmatrix} \Mat{q}_{e,1} & \cdots & \Mat{q}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert \times d} $ as an intermediate auxiliary variable. The detailed derivation can be found in the \textcolor{red}{Appendix}.

% We name gradient $\nabla_{v} g(\cdot)$ and proximal gradient $\prox_{\frac{1}{\lambda} g}(\cdot)$ as \textit{hypergraph diffusion operator} \pan{hyperedge diffusion operator}, since they summarize the collection of node features inside a hyperedge and dispatch the aggregated information to interior nodes individually.
% These hypergraph diffusion operators can be intuitively interpreted as a (one-hop) information fusion among nodes connected by some hyperedge.
% We reveal one crucial property of hypergraph diffusion operators by the following propostion:
% \begin{proposition} \label{prop:equivariant_op}
% Hypergraph diffusion operators $\prox_{\frac{1}{\lambda},g}(\Mat{H}_e)$ (\pan{Use the full}) and $\nabla_v g(\Mat{H}_e)$ \pan{I do not think this is an okay notation. We need to consider defining $\nabla g() = [\nabla_v g]_{v\in e}$} are permutation-equivariant operators with respect to node features $\Mat{h}_v$ for any potential function $g(\cdot)$.
% \end{proposition}
% We provide the proof of Proposition \ref{prop:equivariant_op} in \textcolor{red}{Appendix}. It states that hypergraph diffusion operator $\nabla_v g(\Mat{H}_e)$ and $\prox_{\frac{1}{\lambda},g}(\Mat{H}_e)$ should not only aggregate features regardless of the node order, but should also pass distinctive messages to different nodes.
% This means the operator $\prox_{\frac{1}{\lambda},g}(\Mat{H}_e)$ and $\nabla_v g(\Mat{H}_e)$ are both equivariant set functions.

% After reviewing different forms of hypergraph diffusion, now we assume both node-wise and hyperedge potential functions are unknown.

\subsection{Building Equivariant Hyperedge Diffusion Operators}
\vspace{-1mm}
\label{sec:build_equivariance}
%Hyperedge diffusion operators are essentially permutation-equivariant operators as shown above. 
To model permutation-equivariant diffusion operators, we may resort to previous studies on NN architectures to represent equivariant multi-set functions~\cite{zaheer2017deepset,maron2018invariant,segol2020universal}. However, there are still some gaps when we apply their approaches in the hypergraph setting. In practice, these works focus on the case with separate multi-sets, such as prediction over  separate collections of images or 3-D points, while hypergraphs contain a large number of coupled hyperedges. As  hyperedges could be large and irregular in practice, how to build scalable equivariant NN architectures on hyperedges is challenging. Note that although graphs also couple many edges, edges in graphs are of regular size two. Building equivariant edge operation in graphs is often much less crucial or challenging. %much more  challenging than that in traditional GNN design. %In theory, although previous works proved the universal approximation of their proposed architecture~\cite{segol2020universal}, the construction uses the universality of equivariant polynomials as a bridge, which induces two issues of the obtained conclusion. First, the theory does not provide a precise representation of a permutation-equivariant function. Second, the needed latent dimension is exponential w.r.t. the input feature dimension, which conflicts with the scalability requirement in hypergraph models.

%Specifically, for an equivariant function $\psi(\cdot):\mathbb{R}^{K\times F} \rightarrow \mathbb{R}^{K\times F}$, they suggest 
% \begin{align}\label{eqn:equivariant}
%     \psi(\cdot) = L_m\circ \sigma \circ L_{m-1}\circ  \cdots \circ \sigma \circ L_{1},\, \text{where}\, L_i(\Mat{Z})= \Mat{Z}\Mat{W}_i^{(1)} +  \mathbf{1}\mathbf{1}^T\Mat{Z}\Mat{W}_i^{(2)} + \mathbf{1}\Mat{W}_i^{(3)T},
% \end{align}
% $\sigma$ is entry-wise nonlinear activation. 
% $\Mat{W}_i^{(j)}\in\mathbb{R}^{F\times F}$ for $j\in\{1,2\}$ and $\Mat{W}_i^{(3)}\in\mathbb{R}^{F}$ are parameters

% %$\Mat{W}_i^{(j)}\in\mathbb{R}^{F_{\text{in}}^{(i)}\times F_{\text{out}}^{(i)}}$ for $j\in\{1,2\}$ and $\Mat{W}_i^{(3)}\in\mathbb{R}^{F_{\text{out}}^{(i)}}$ are parameters where $F_{\text{in}}^{(1)}=F_{\text{out}}^{(m)}=F$ and $F_{\text{in}}^{(i+1)}=F_{\text{out}}^{(i)}$ for $i\in 1,2,...,m-1$.

% However, there are still some gaps when applying Eq.~\ref{eqn:equivariant} to the hypergraph setting. Practically, $\psi$ is used to make prediction for decoupled multi-sets, such as prediction over each separate collection of images or 3-D points, while hypergraphs contain a large number of coupled multi-sets. As a hypergraph may contain thousands of hyperedges and a node may appear in hundreds of hyperedges, how to build scalable equivariant operators for all hyperedges is crucial. Note that graphs also couple thousands of edges while edges are of regular size two so building equivariant edge operation is not that crucial and challenging in traditional GNN design. In theory, although previous work proved the universal approximation of the architecture Eq.~\ref{eqn:equivariant}~\cite{segol2020universal}, the construction uses the universality of equivariant polynomials as a bridge, which induces two issues. First, the conclusion may not allow a precise representation of $\psi(\cdot)$. Second, the needed latent dimension is exponential w.r.t. the dimensions $K$ and $F$, which conflicts with the scalability requirement in hypergraph models. 

Our design is built upon the following Theorem~\ref{thm:equivarnt_form_1dim}. We leave the proof in Appendix~\ref{sec:proof-equi-1dim}. %and \ref{sec:proof-equi-Fdim}.

%As shown below, we formally specifies a general form that equivariant function must have:
\begin{theorem} \label{thm:equivarnt_form_1dim}
 $\psi(\cdot): [0,1]^K \rightarrow \mathbb{R}^K$ is a continuous permutation-equivariant function, if and only if it can be represented as  $[\psi(\Mat{Z})]_i = \rho(\Mat{z}_i, \sum_{j=1}^K \phi(\Mat{z}_j))$, $i\in [K]$ for any $\Mat{Z} = \begin{bmatrix} ...,\Mat{z}_i,...\end{bmatrix}^\top\in [0,1]^{K}$, 
% \begin{align}
%     \psi(x_1, x_2,\cdots,x_k) =
%      \begin{bmatrix} 
%     \rho(x_1, \sum_{i=1}^K \phi(x_i)) \\
%     \rho(x_2, \sum_{i=1}^K \phi(x_i)) \\
%     \vdots\\
%     \rho(x_3, \sum_{i=1}^K \phi(x_i)) \\
%     \end{bmatrix}
% \end{align}
where $\rho: \real^{K'} \rightarrow \real$, $\phi: \real \rightarrow \real^{K'-1}$ are two continuous functions, and $K'$ could be as small as $K$. 
\end{theorem}  \vspace{-1mm}

Theorem~\ref{thm:equivarnt_form_1dim} indicates that any continuous permutation-equivariant function is a compositions of a continuous function $\rho$ and the sum of another continuous function $\phi$ on each input entry. This result generalizes the representation of permutation-invariant functions by $\rho(\sum_{i=1}^K\phi(\Mat{z}_i))$ in~\cite{zaheer2017deepset} to the equivariant case. An architecture with a similar spirit was proposed in~\cite{segol2020universal} for non-coupled multi-set representations. However, their proof used the universality of equivariant polynomials as a bridge so their construction $\hat{\psi}(\Mat{Z})$ only allows approximation, i.e., small $\|\psi(\Mat{Z})-\hat{\psi}(\Mat{Z})\|$ instead of precise representation in Theorem~\ref{thm:equivarnt_form_1dim}. Also, $K'\geq K$ is tight by generalizing the proof for invariant set function representation~\cite{wagstaff2019limitations}. Note that, in practice, $\rho$ and $\phi$ often need to be further approximated by NNs. So, Theorem~\ref{thm:equivarnt_form_1dim} has more theoretical significance than practice given the results in~\cite{segol2020universal}. %Also, $K'\geq K$ is tight by generalizing the proof for invariant set function representation~\cite{wagstaff2019limitations}. 

% More practical significance can be achieved when we consider multiple feature dimensions:
% \begin{theorem} \label{thm:equivarnt_form_Fdim}
%  $\psi(\cdot): [0,1]^{K\times F} \rightarrow \mathbb{R}^{K}$ is a  permutation-equivariant function, if and only if it can be represented as  $[\psi(\Mat{Z})]_i = \rho(\Mat{z}_i, \sum_{j=1}^K \phi(\Mat{z}_j))$, $i\in [K]$, for any $\Mat{Z} = \begin{bmatrix} ...,\Mat{z}_i,...\end{bmatrix}^\top\in [0,1]^{K\times F}$.
% % \begin{align}
% %     \psi(x_1, x_2,\cdots,x_k) =
% %      \begin{bmatrix} 
% %     \rho(x_1, \sum_{i=1}^K \phi(x_i)) \\
% %     \rho(x_2, \sum_{i=1}^K \phi(x_i)) \\
% %     \vdots\\
% %     \rho(x_3, \sum_{i=1}^K \phi(x_i)) \\
% %     \end{bmatrix}
% % \end{align}
% where $\rho: \real^{K'+1} \rightarrow \real$, $\phi: \real^F \rightarrow \real^{K'}$ are two  functions, and $K'$ could be as small as $K^4F^2$. 
% \end{theorem}
% The construction in~\cite{segol2020universal} that adopts equivariant polynomials needs the latent dimension to representation each entry $\phi(\Mat{z}_i)$ to be in the order of $K'\geq {K+F \choose F}$ to achieve even just approximate representations, which is practically infeasible. Note that $K^4F^2$ in Theorem~\ref{thm:equivarnt_form_Fdim} is not still tight.

The above theoretical observation inspires the design of equivariant hyperedge diffusion operators. Specifically, for an operator $\hat{\psi}(\cdot):\mathbb{R}^{|e|}\rightarrow \mathbb{R}^{|e|}$ that may denote either gradient $\nabla g(\cdot)$ or proximal gradient $\prox_{\eta g}(\cdot)$ for each hyperedge $e$, we may parameterize it as: \vspace{-1mm}
\begin{align}\label{eq:equi-form}
    [\hat{\psi}(\Mat{H}_e)]_v=\hat{\rho}(\Mat{h}_v, \sum_{u\in e} \hat{\phi}(\Mat{h}_u)),\,\text{for $v\in e$,}\, \text{where $\hat{\rho},\,\hat{\phi}$ are multi-layer perceptions (MLPs). }
\end{align}
Intuitively, the inner sum collects the $\hat{\phi}$-encoding node features within a hyperedge and then $\hat{\rho}$ combines the collection with the features from each node further to perform separate operation. 

The implementation of the above $\hat{\psi}$ is not trivial. A naive implementation is to generate an auxillary node to representation each $(v,e)$-pair for  $v\in\Set{V}$ and $e\in\Set{E}$ and learn its representation as adopted in  \cite{yadati2020neural,arya2020hypersage,yang2020hypergraph}. However, this may substantially increases the model complexity. 

Our implementation is built upon the widely-used bipartite representations~\cite{dong2020hnhn,huang2021unignn,chien2021you} (or  star expansion~\cite{zien1999multilevel,agarwal2006higher}, equivalently) of hypergraphs paired with the standard message passing NN (MPNN)~\cite{gilmer2017neural} that can be efficiently implemented via the commonly-used GNN platforms~\cite{FeyPyG,wang2019dgl}. Specifically, we build a bipartite graph $\Set{\bar{G}} = (\Set{\bar{V}}, \Set{\bar{E}})$. The node set $\Set{\bar{V}}$ contains two parts $\Set{V}\cup\Set{V_{\Set{E}}}$ where $\Set{V}$ is the original node set while $\Set{V_{\Set{E}}}$ contains nodes corresponding to original hyperedges $e\in\Set{E}$. Then, add an edge between $v\in\Set{V}$ and $e\in\Set{E}$ if $v\in e$. The model \textbf{\proj} is implemented by following \textbf{Algorithm 1}.
% For different 
% \begin{enumerate}[leftmargin=4mm]
%     \item Designing the messages from $\Set{V}$ to $\Set{E}$:\quad  $\Mat{m}_{u\rightarrow e}^{(t)} = \hat{\phi}(\Mat{h}_u^{(t)})$, for all $u\in\Set{V}$. 
%     \item Sum $\Set{V}\rightarrow \Set{E}$ messages over hyperedges $\Mat{m}_{e}^{(t)} = \sum_{u\in e} \Mat{m}_{u\rightarrow e}^{(t)}$, for all $e\in\Set{E}$.
%     \item Broadcast $\Mat{m}_{e}^{(t)}$ and design the messages from $\Set{E}$ to $\Set{V}$: $\Mat{m}_{e\rightarrow v}^{(t)} = \hat{\rho}(\Mat{h}_v^{(t)},\Mat{m}_{e}^{(t)})$, for all $v\in e$.% and $e\in\Set{E}$. 
%     \item Update $\Mat{h}_v^{(t+1)}= \hat{\varphi}(\Mat{h}_v^{(t)}, \sum_{e:u\in e}\Mat{m}_{e\rightarrow u}^{(t)}, \Mat{x}_v, d_v)$, for all $v\in\Set{V}$,  where $\hat{\varphi}$ is another MLP. 
% \end{enumerate}


\begin{table}[t]
\begin{tabular}{l}
\hline 
\textbf{Algorithm 1: \proj} \\
\hline
\textbf{Initialization:} $\Mat{H}^{(0)}=\Mat{X}$ \textbf{and three MLPs $\hat{\phi},\,\hat{\rho},\, \hat{\varphi}$ (shared across $L$ layers).} \\
%\textbf{Output:} $\Mat{H}^{(L)}$.\\
\textbf{For} $t=0,1,2,...,L-1$, \textbf{do:}\\
1. Designing the messages from $\Set{V}$ to $\Set{E}$:\quad  $\Mat{m}_{u\rightarrow e}^{(t)} = \hat{\phi}(\Mat{h}_u^{(t)})$, for all $u\in\Set{V}$. \\ 
2. Sum $\Set{V}\rightarrow \Set{E}$ messages over hyperedges $\Mat{m}_{e}^{(t)} = \sum_{u\in e} \Mat{m}_{u\rightarrow e}^{(t)}$, for all $e\in\Set{E}$.\\
3. Broadcast $\Mat{m}_{e}^{(t)}$ and design the messages from $\Set{E}$ to $\Set{V}$: $\Mat{m}_{e\rightarrow v}^{(t)} = \hat{\rho}(\Mat{h}_v^{(t)},\Mat{m}_{e}^{(t)})$, for all $v\in e$. \\% and $e\in\Set{E}$.\\
4. Update $\Mat{h}_v^{(t+1)}= \hat{\varphi}(\Mat{h}_v^{(t)}, \sum_{e:u\in e}\Mat{m}_{e\rightarrow u}^{(t)}, \Mat{x}_v, d_v)$, for all $v\in\Set{V}$. \\
\hline 
\end{tabular}
\vspace{-0.4cm}
\end{table}

The equivariant diffusion operator $\hat{\psi}$ can be naturally constructed via steps 1-3. The last step is to update the node features to accomplish the first two terms in Eq.~\ref{eqn:gd} or the ADMM update Eq.~\ref{eqn:admm-h}. The initial attributes $\Mat{x}_v$ and node degrees are included to match the diffusion algorithm by design. As the diffusion operators are shared across iterations, \proj shares parameters across layers. Now, we summarize the joint contribution of our theory and  efficient implementation as follows.

\begin{proposition}\label{prop:universal}
MPNNs on bipartite representations (or star expansions) of hypergraphs are  expressive enough to learn any continuous diffusion operators induced by invariant hyperedge potentials.   
\end{proposition}

\proj can well approximate the GD algorithm (Eq.~\ref{eqn:gd}), while \proj does not perfectly match ADMM unless we assume $\Mat{Q}_e^{(t)}=\Mat{H}_e^{(t)}$ in Eq.~\ref{eqn:admm-q} for a practical consideration. This assumption may reduce the performance of the algorithm while \proj has already achieved good enough empirical performance. Tracking $\Mat{Q}_e^{(t)}$ means recording the messages from $\Set{E}$ to $\Set{V}$ for every iteration, which is not  supported by the current GNN platforms~\cite{FeyPyG,wang2019dgl} and may consume more memory. We leave the incorporation of $\Mat{Q}_e^{(t)}$ as a future study. A co-design of the algorithm and the system may be needed.  

\textbf{Extension.} Our \proj can be naturally extended to build equivariant node operators because of the duality between hyperedges and nodes, though this is not necessary in the traditional hypergraph diffusion problem Eq.~\ref{eqn:diffusion}. Specifically, we call this model \projtwo, which simple revises the step 1 in \proj as $\Mat{m}_{u\rightarrow e}^{(t)} = \hat{\phi}(\Mat{h}_u^{(t)}, \Mat{m}_e^{(t-1)})$ for any $e$ such that $u\in e$. Due to the page limit, we put some experiment results on \projtwo in Appendix~\ref{sec:expr_edgnn2}.


\subsection{Discussion: Advantages of \proj in Heterophilic Settings and Deep Models}
\label{sec:dis_heterophily}
Here, we discuss several advantages of \proj due to the design of equivariant diffusion operators. 

Heterophily describes the network phenomenon where nodes with different labels and attributes are more likely to connect to each other directly~\cite{rogers2010diffusion}. %A direct example of network heterophily is intimate relationships where people with different genders are more likely to build a family in a social network. 
Predicting node labels in heterophilic networks is known to be more challenging than that in homophilic networks, and thus has recently become a hot research direction in the community~\cite{pei2020geom,zhu2020beyond,chien2021adaptive,lim2021large}. Heterophily has been proved  as a more common phenomenon in hypergraphs than in graphs since it is hard to expect that all nodes in a gaint hyperedge  share a common label~\cite{li2017inhomogeneous,veldt2021higher}. Moreover, predicting node labels in heterophilic hypergraphs is more challenging than in graphs as a hyperedge may consist of the nodes from multiple categories.% in different ratios. %(see Fig.~\ref{fig:heterophily}).

Learnable equivariant diffusion operators are expected to be superior in predicting heterophilic node labels. For example, if a hyperedge $e$ of size 3 is known to cover two nodes $v,u$ from class $\Set{C}_1$ while one node $w$ from class $\Set{C}_0$. We may use the LEC potential $\langle\Mat{y},\varsigma(\Mat{H}_e)\rangle^2$ by setting $\Mat{y} = [1,-1,0]^\top$. Suppose the three nodes' attibutes are $\Mat{H}_e=[\Mat{h}_v, \Mat{h}_u, \Mat{h}_w]^\top=[0.7, 0.5, 0.3]^\top$, where $\Mat{h}_v$, $\Mat{h}_u$ are close as they are from the same class. One may check the hyperedge diffusion operator gives $\nabla g(\Mat{H}_e) = [0.4, -0.4, 0]^\top$. One-step gradient descent $\Mat{h}_v - \eta [\nabla g(\Mat{H}_e)]_v$ with a proper step size ($\eta < 0.5$) drags $\Mat{h}_v$ and $\Mat{h}_u$ closer while keeping $\Mat{h}_w$ unchanged. However, invariant diffusion that allocates every node with the same change does not help with the classification. If the ground truth is different, say $w,u$ from the same class and $v$ from the other, using the above $\Mat{y}$ may increase the error. However, learnable operators can solve the problem, e.g., by learning another $\Mat{y}=[0,1,-1]^\top$. 

Moreover, equivariant hyperedge diffusion operators are also good at building deep models. GNNs tend to degenerate the performance when going deep, which is often attributed to their oversmoothing~\cite{li2018deeper,oono2019graph} and overfitting problems~\cite{cong2021provable}. Equivariant operators allocating different messages to different nodes helps with overcoming the oversmoothing issue. On the other hand, diffusion operators by sharing parameters across different layers may reduce the risk of overfitting.     


\subsection{Previous Hypergraph Neural Networks for Representing Hypergraph Diffusion}\label{sec:previous}

\proj is the first HNN inspired by the general class of hypergraph diffusion and provably achieves  universal approximation of hyperedge diffusion operators. So, how about previous HNNs representing hypergraph diffusion? We temporarily ignore the big difference in whether parameters are shared across layers and give analysis as follows. HGNN~\cite{feng2019hypergraph} runs graph convolution~\cite{kipf2016semi} on clique expansions of hypergraphs, which directly assumes the hyperedge potentials follow CE plus pairwise potentials and cannot learn other operations on hyperedges. HyperGCN~\cite{yadati2019hypergcn} essentially leverages the total variation potential by adding mediator nodes to each hyperedge, which adopts a transformation technique in~\cite{chan2018spectral,chan2020generalizing}. A few works view hyperedges as multi-sets of nodes and nodes as multi-sets of hyperedges~\cite{dong2020hnhn,huang2021unignn,chien2021you,bai2021hypergraph,arya2020hypersage,yadati2020neural,yang2020hypergraph,jo2021edge}. 
Among them, HNHN~\cite{dong2020hnhn}, UniGNNs~\cite{yang2020hypergraph}, EHGNN~\cite{jo2021edge} and AllSet~\cite{chien2021you} build two invariant set-pooling functions on both the hyperedge and node sides, which cannot represent equivariant functions. One subtle point is that Uni\{GIN,GraphSAGE,GCNII\}~\cite{yang2020hypergraph} adopt jump link to pass node features from the last layer to the next and may expect to use a complicated node-side invariant function $\hat{\psi}'(\Mat{h}_v^{(t)},\sum_{e:v\in e} \Mat{m}_e^{(t)})$ to approximate our $\hat{\psi}(\Mat{h}_v^{(t)},\sum_{e:v\in e} \Mat{m}_{e\rightarrow v}^{(t)})=\hat{\psi}(\Mat{h}_v^{(t)},\sum_{e:v\in e} \hat{\rho}(\Mat{h}_v^{(t)},\Mat{m}_e^{(t)}))$ in Step 4 of \textbf{Algorithm 1} directly. This may be doable in theory. However, the jump-link solution may expect to have a higher dimension of $\Mat{m}_e^{(t)}$ (dim=$|\cup_{e:v\in e} e|$) so that the sum pooling $\sum_{e:v\in e} \Mat{m}_e^{(t)}$ does not lose anything from the neighboring nodes of $v$ before interacting with $\Mat{h}_v^{(t)}$, while in \proj,  $\Mat{m}_e^{(t)}$ needs dim=$|e|$ according to Theorem~\ref{thm:equivarnt_form_1dim}. Our empirical experiments also verify more expressiveness of \proj. HCHA~\cite{bai2021hypergraph} and UniGAT~\cite{yang2020hypergraph} compute attention weights as a result of combining node features and hyperedge messages, which looks like our $\rho$ operation. However, a scalar attention weight is too limited to represent the potentially complicated $\rho$. HyperSAGE~\cite{arya2020hypersage},   MPNN-R~\cite{yadati2020neural} and LEGCN~\cite{yang2020hypergraph} may learn hyperedge equivariant operators, while they need many auxillary nodes that represent node-hyperedge pairs. Of course, none of these works have mentioned any theoretical arguments on universal representation as ours.  

% $\mathcal{N}_{v}$    

% %, by inheriting from GIN~\cite{xu2018how} and GraphSAGE~\cite{hamilton2017inductive}


% designing message from $V$ to $E$ as $\Set{M}_{\Set{V}\rightarrow \Set{E}} = \hat{\phi}(\Mat{h}_u)$. 

% %=\Set{V}\cup\Set{V_{\Set{E}}}$. 



% To prove Theorem \ref{thm:equivarnt_form}, we sequentially adopt Lemma \ref{lem:equivariant_form} and results of invariant set functions in \cite{zaheer2017deepset}.
% We defer the detailed proof into \textcolor{red}{Appendix}.
% Theorem \ref{thm:equivarnt_form} demonstrates that an equivariant set function can be modeled by a pair-wise relationship between each element and a summarized vector of the whole set.
% Note that our proof avoids equivariant polynomials used in \cite{segol2019universal}, thus we can restrict the dimension of the summarized vector to be $d$.





% But their construction requires an exponential hidden dimension with respect to set cardinality to represent hyperedge features, which is infeasible to implement.
% In this section, we propose a more plausible solution to uniformly approximate equivariant operators capable of representing any type of hypergraph diffusions.


% However, there are still some gaps when applying their techniques to the hypergraph setting. Practically, most previous works focus on building models for multi-sets that are not coupled, such as a set of images or 3-D points, while hypergraphs contain coupled multi-sets as a node may appear in multiple hyperedges. Graphs couple edges that can be viewed as sets of nodes while edges in graphs are of regular size two so building equivariant edge operation is not that crucial and challenging in GNN design. In theory, previous works proposed the form of linear layer composed with the entry-wise nonlinear activation to build equivariant multi-set representation~\cite{zaheer2017deepset,maron2018invariant}, which has later been proved to achieve universal approximation~\cite{segol2020universal}. However, the proof in~\cite{segol2020universal} uses equivariant polynomials as a bridge, which induces two issues of the obtained conclusion. The statement is always an approximation statement and the  


% Hence, how to build computationally efficient equivariant hyperedge operations in HGNN?

% Hence, how to efficiently build equivariant hyperedge operations in HGNN 

% No previous works have proposed the coupled ones as we observed in hypergraphs.

% Hyperedge operaters are set eqvariant, then how to build them? Building equivariant set neural network architecture has been studied in xxx. Practically, they mostly focus on building separate sets. No previous works have proposed the coupled ones as we observed in hypergraphs. Theoretically, deepset and Maron proposes the form of linear layer composed with the entry-wise nonlinear activation to build equivariant set representation. Segol proves the unverival approximation of it, while Segol's proof is built upon equivariant polynomial so there is only approximation result. However, we may have precise argument as following theorem, though learning $\rho$ and $\phi$ via NN still needs approximation.  

% The crucial thing is how to efficiently implement it. Bipartite framework: One cannot record everything and do invariance. The key is to invariant pooling on hyperedge side. When message passes from hyperedge to nodes, do equivariant before pooling. Overall the processing is equivariant. Different from Allsets, Allset first invariant pool and second jump link. However, such invariant pool may need to enlarge the dimension to record the entire receptive field. 

% \subsection{} 
% further build double equivariant.

% build attention equivariant (All set uses a single vector) 

% \cite{yadati2020neural} build new nodes for node hyperedge pair (too complicated)

% \cite{arya2020hypersage} use complement $e/v$ to build rep

% \cite{dong2020hnhn} double invariant sets no jump link

% \cite{huang2021unignn} double invariant sets with jump link

% \cite{chien2021you} double invariant no jump link

% \cite{yadati2019hypergcn} use a mediator.

% It seems that~\cite{bai2021hypergraph} considers the attention equi. (also double invariant)

% \subsection{}



% %maron discuss the general linear layers to build equivariant set representation while there is no universal guarantee. Segol   


% The choice of $g(\cdot)$ varies from different tasks. For real-world data, it is intractable to handcraft a potential function that precisely express prior distribution over hyperedges.
% Recent works \cite{gregor2010learning, liu2019alista, chen2018theoretical, yang2021graph, liu2021elastic} have shown that unrolling and parameterizing each iteration of an optimization problem with neural networks can express more universal objectives and achieve faster convergence.
% Motivated by this line of works, we intend to construct a parametric hypergraph diffusion operator that can be learned from data. \pan{Claim how to implement equi hyperedge operator is non-trivial. Previous works are regular. Moreover, standard model, do not need to worry this.}

% \pan{Build a bipartite graph by following HNHN and allset. However, we show that invariant sum pooling when message  The sum pooling over hyperedges. When message passes from hyperedges to nodes, we do an additional operation. This techniques have been used in xxx while no hypergraph NN has used this to build eq.  Moreover, our results are not approximation results. The needed dimension is polynomial w.r.t.... }
% A handy choice to parameterize hypergraph diffusion operator is neural networks. However, typical architectures, such as Multi-Layer Perceptrons (MLP), would not be the candidate as they do not satisfy the equivariance property.
% % Zaheer \etal \cite{zaheer2017deepset} proposed a sum-pooling based architecture that can represent any set functions, 
% To achieve order invariance, one may consider DeepSet \cite{zaheer2017deepset} which introduces a sum-pooling scheme to represent arbitrary set functions.
% However, it is subject to invariant operators, which are essentially less expressive than equivariant operators.
% Segol \etal \cite{segol2019universal} adopted symmetric polynomials as a tool to approximate equivariant set function.
% But their construction requires an exponential hidden dimension with respect to set cardinality to represent hyperedge features, which is infeasible to implement.
% In this section, we propose a more plausible solution to uniformly approximate equivariant operators capable of representing any type of hypergraph diffusions.


% % In previous section, we already know to approximate hypergraph diffusion operator, we need to build a permutation-equivariant set function.
% % Even though it is well-known that building a permutation-invariant set function is as simple as raising the input elements into a high-dimension space, summing over the set to obtain a summarized vector, and projecting it to the output space, how to constructing a permutation-equivariant function remains elusive in the literature.

% Our follow-up discussion falls on how to represent permutation-equivariant functions in general. To this end, we first provide the following lemma:
% \begin{lemma} \label{lem:equivariant_form}
% $f: \mathbb{R}^k \rightarrow \mathbb{R}^k$ is an equivariant function if and only if $f(\cdot)$ can be represented as the following form, 
% \begin{align}
%     f(x_1, x_2, \cdots , x_{k-1}, x_k) = 
%     \begin{bmatrix} 
%     p(x_1, x_2, \cdots, x_{k-1}, x_k) \\
%     p(x_2, x_3, \cdots, x_k, x_1) \\
%     \vdots \\
%     p(x_N, x_1, \cdots, x_{k-2}, x_{k-1}) \\
%     \end{bmatrix}
% \end{align}
% where $p(\cdot): \mathbb{R}^k \rightarrow \mathbb{R}$ is permutation-invariant with respect to the last $k-1$ elements of inputs. 
% \end{lemma}
% We give a proof in the \textcolor{red}{Appendix}.
% Lemma \ref{lem:equivariant_form} implies that an equivariant function can be element-wisely decomposed into partially invariant mappings, which bridges the construction of invariant and equivariant functions.
% Prior works \cite{zaheer2017deepset, wagstaff2019limitations} have guaranteed a finite-dimension and continuous construction of invariant functions.
% Using Lemma \ref{lem:equivariant_form}, we are about to compose width-limited and continuous equivariant functions using such invariant functions.
% As shown below, we formally specifies a general form that equivariant function must have:
% \begin{theorem} \label{thm:equivarnt_form}
% $g(\cdot): \mathbb{R}^k \rightarrow \mathbb{R}^k$ is a continuous equivariant function,if and only if $g(\cdot)$ can be represented as the following form, 
% \begin{align}
%     g(x_1, x_2,\cdots,x_k) =
%      \begin{bmatrix} 
%     \rho(x_1, \sum_{i=1}^k \phi(x_i)) \\
%     \rho(x_2, \sum_{i=1}^k \phi(x_i)) \\
%     \vdots\\
%     \rho(x_3, \sum_{i=1}^k \phi(x_i)) \\
%     \end{bmatrix}
% \end{align}
% where $\rho: \real^d \rightarrow \real$, $\phi: \real \rightarrow \real^d$ are all continuous functions. \pan{fill in the F dim case.}
% \end{theorem}
% To prove Theorem \ref{thm:equivarnt_form}, we sequentially adopt Lemma \ref{lem:equivariant_form} and results of invariant set functions in \cite{zaheer2017deepset}.
% We defer the detailed proof into \textcolor{red}{Appendix}.
% Theorem \ref{thm:equivarnt_form} demonstrates that an equivariant set function can be modeled by a pair-wise relationship between each element and a summarized vector of the whole set.
% Note that our proof avoids equivariant polynomials used in \cite{segol2019universal}, thus we can restrict the dimension of the summarized vector to be $d$.
% % \textcolor{red}{emphasize the difference between ICLR 2019 and ours. Ours does not need equivariant polynomial, and the dimension can be reduced to d}

% \subsection{Unfolding Hypergraph Diffusion as HGNN}
% \pan{Suggest to directly merge this section with the previous one.}
% We observe that each diffusion step for both differentiable (Eq. \ref{eqn:gd}) and non-differentiable (Eq. \ref{eqn:admm}) potential functions can be unified into the following form:
% \begin{align} \label{eqn:neural_diffusion}
%     \Mat{h}_v^{(t+1)} = \rho\left(\Mat{h}_v^{(t)}, \sum_{e:v \in e} \phi_v(\Mat{H}_e^{(t)}) \right)
% \end{align}
% where $\phi: \real^{|e| \times d} \rightarrow \real^{|e| \times d}$ corresponds to gradient operators over hyperedges $\nabla_{v} g(\cdot)$ and $\prox_{\frac{1}{\rho} g}(\cdot)$ that aggregates node features to be hyperedge-level features and dispatches them to each node, $\phi_v(\cdot)$ indexes the value at node $v$, while $\rho: \real^{d} \times \real^{d} \rightarrow \real^{d}$ combines hyperedge features with node features.
% The choice of $f(\cdot)$ and $g(\cdot)$ varies from different tasks. For real-world data, handcrafting potential functions that precisely express prior distribution over hyperedges can be intractable.
% Recent works \textcolor{red}{Cite LISTA and other unrolling graph papers} have shown that unrolling each iteration in an optimization problem can naturally derive similar structures to multi-layer neural networks, that introduces a group of learnable parameters to express more universal objectives and achieve faster convergence.
% Motivated by this line of works, we intend to construct a parametric hypergraph diffusion operator that can be learned from data.
% Thereby we parameterize $\rho(\cdot)$ and $\phi(\cdot)$ with some learnable parameters $\Mat{\Theta}$, then Eq. \ref{eqn:neural_diffusion} can be viewed as the $t$-th layer of hypergraph neural networks.
% Unfolding $L$ iterations results in an $L$-layer hypergraph neural networks.

% \subsection{Implementing Equivariant Diffusion HGNN}

% With Theorem \ref{thm:equivarnt_form}, we can borrow neural networks to parameterize $\rho(\cdot)$ and $\phi(\cdot)$ due to the universal approximation theorem.
% This implies we can build a neural hypergraph diffusion operator in the following form: 
% \begin{align} \label{eqn:neural_nd}
% \nabla_v g\left(\Mat{h}^{(e)}_1, \Mat{h}^{(e)}_2,....,\Mat{h}^{(e)}_{|e|}\right) =
%  \begin{bmatrix} 
% \MLP_2(\Mat{h}^{(e)}_1, \sum_{i=1}^{|e|} \MLP_1(\Mat{h}^{(e)}_i)) \\
% \MLP_2(\Mat{h}^{(e)}_2, \sum_{i=1}^{|e|} \MLP_1(\Mat{h}^{(e)}_i)) \\
% \vdots\\
% \MLP_2(\Mat{h}^{(e)}_{|e|}, \sum_{i=1}^{|e|} \MLP_1(\Mat{h}^{(e)}_i)) \\
% \end{bmatrix},
% \end{align}
% where $\MLP_1: \real^d \rightarrow \real^{|e|d}$ raises the dimension of each node feature, and $\MLP_2: \real^d \times \real^{|e|d} \rightarrow \real^{d'}$ concatenates the feature of the first input and the summarized vector and projects them into the output space.
% During the training stage, we iteratively invoke Eq. \ref{eqn:neural_nd} for $L$ times, and optimize MLP parameters by back propagating loss of some downstream tasks.

% \subsection{Comparison with Hypergraph Neural Networks}


% \begin{proposition} (Informal)
% AllSet, HGNN, HyperGNN are permutation-invariant but not permutation-equivariant.
% \end{proposition}

% \textcolor{red}{discuss difference between other models AllSet, HyperGCN, HGNN.}

% \textcolor{red}{another clue is first propose our model, and then discuss existing models, how our model degenerate to their model.}


% \textcolor{red}{discuss a variant of our model: two equivariant set functions (allset)}

% \textcolor{red}{our model can go deeper to achieve better performance due to diffusion model}

% \textbf{Introduce how we implement the equivariant diffusion via neural networks. Overall, we have \proj.}


% Suppose we are to approximate $H_v^{(1)}$ where $H^{(0)} = X$, initial $q_e^{(0)}=0$. (put into appendix)
% \begin{align*}
%         q_e^{(1)} &\leftarrow  \prox_{\frac{1}{\rho},g}(2\bar{h}_e^{(0)}) - \bar{h}_e^{(0)}\\
%         h_v^{(1)} &\leftarrow  
%         \prox_{\frac{1}{\rho d_v},f}(p_v),\quad \text{where}\; p_v=\frac{1}{d_v}\sum_{e:e\in v}q_{e,v}^{(1)}%\\
%         %s_e^{(t+1)} &\leftarrow s_e^{(t)} + r_e^{(t+1)} - \bar{h}_v^{(t+1)}
%     \end{align*} 

% Or you may choose Gradient-descent (main text):
%     \begin{align*}
%         h_v^{(t+1)} \leftarrow  h_v^{(t)} - \alpha \left(\nabla f(h_v^{(t)};x_v) + \sum_{e: v\in e} q_{e,v}^{(t)}\right), \quad \text{where}\; q_{e,v}^{(t)} = \nabla g(\bar{h}_e^{(t)}),\; \text{for}\; v\in V.
%     \end{align*}
    

% % If we consider the update as a hypergraph operator $\psi: h_v^{(t)} \rightarrow h_v^{(t+1)}$, both settings essentially correspond to a mapping function
% % %\begin{align*}
% % %    h_v^{(t+1)} = \psi_1(h_v^{(t)}, \oplus_{e:v\in e} q_{e,v}^{(t+1)}),\,\text{where}\;q_{e,v}^{(t+1)} = \psi_2(h_v^{(t)}, \oplus_{u\in e/v} h_u^{(t)})  
% % %\end{align*}
% % \begin{align*}
% %     z = \psi(x, \oplus_{e:v\in e}\oplus_{u\in e/v} s_{e,u}),\; \text{where}\; s_{e,u} = h_{u}^{(t)}. %q_{e,v}^{(t+1)}),\,\text{where}\;q_{e,v}^{(t+1)} = \psi_2(h_v^{(t)}, \oplus_{u\in e/v} h_u^{(t)})  
% % \end{align*}
% % which is invariance with respect to the permutation $\pi_v$ over $\{e|v\in e\}$ and the  permutations $\pi_{v,e}$ over $\{u\in e|u\neq v\}$, i.e., 





% \textbf{3. Prove dimension argument: vs ID, vs jump link + ID}

% %I use $[\nabla g(\bar{x}_e)]_v$ to denote the gradient w.r.t. $x_v$ of the invariant function $g(\cdot)$ with $|e|$-dim input $\bar{x}_e = (...,x_u,...)_{u\in e}$. 




% Our proposal: 
% \begin{itemize}
%     \item Equivariant operator:
% \begin{align*}
%     \text{MLP}_3(x_v,x_v^{(0)},\sum_{e:v\in e} \text{MLP}_2(x_v, \sum_{u\in e}\text{MLP}_1(x_u))).
% \end{align*}
% Theoretically, we just need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2) $\text{MLP}_2: \mathbb{R}^{|e|+1} \rightarrow \mathbb{R}$; (3) $\text{MLP}_3: \mathbb{R}^3 \rightarrow \mathbb{R}$



% \item Jump-link + Invariant operator: 
% \begin{align*}
%     \text{MLP}_3(x_v, \sum_{e:v\in e} \text{MLP}_2(\sum_{u\in e}\text{MLP}_1(x_u))).
% \end{align*}
% Theoretically, we need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2)
% $\text{MLP}_2: \mathbb{R}^{|e|} \rightarrow \mathbb{R}^{(|e|-1)*d_v+1}$; (3) $\text{MLP}_3: \mathbb{R}^{(|e|-1)*d+1} \rightarrow \mathbb{R}$.

% % \item Small invariant operator (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% % \begin{align*}
% %     \text{MLP}_2(\sum_{e:v\in e} \sum_{u\in e}\text{MLP}_1(x_u)).
% % \end{align*}
% % We know this cannot give universal approximation. But the parameter selection should be at least the same as equivariant operator.


% \item Big invariant operator: 
% \begin{align*}
%     \text{MLP}_3(\sum_{e:v\in e} \text{MLP}_2(\sum_{u\in e}\text{MLP}_1(x_u))).
% \end{align*}
% We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

% \item Attention-based (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% \begin{align*}
%     Attention_2(\text{MLP}_2(Attention_1(\{\text{MLP}_1(x_u)|u\in e\}))|e:v\in e).
% \end{align*}
% We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

% \end{itemize}

% Empirical comparison: We study the dependence on $k$ from 20-200. We should consider alternative projection and subgradient descent. We should consider the following models with degree and node feature fixed.

% %We also add the following three models.

% % \begin{itemize}
% % \item Small equivariant operator (In sec 3, we do not need to discuss this, which is just for fair comparison):
% % \begin{align*}
% %     \sum_{e:v\in e} \text{MLP}_2(x_v, \sum_{u\in e}\text{MLP}_1(x_u)).
% % \end{align*}

% % \item Small invariant operator (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% % \begin{align*}
% %     \text{MLP}_2(\sum_{e:v\in e} \sum_{u\in e}\text{MLP}_1(x_u)).
% % \end{align*}

% %\end{itemize}

% \begin{itemize}
%     \item Equivariant operator:
% \begin{align*}
%     \text{Linear}_3(x_v,\log d_v,\text{mean}_{e:v\in e} \text{MLP}_2(x_v, \log |e|, \text{mean}_{u\in e}\text{MLP}_1(x_u,\log d_v))).
% \end{align*}
% %Theoretically, we just need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2) $\text{MLP}_2: \mathbb{R}^{|e|+1} \rightarrow \mathbb{R}$; (3) $\text{MLP}_3: \mathbb{R} \rightarrow \mathbb{R}$



% \item Jump-link + Invariant operator: 
% \begin{align*}
%     \text{Linear}_3(x_v, \log d_v,  \text{mean}_{e:v\in e} \text{MLP}_2(\log |e|,\text{mean}_{u\in e}\text{MLP}_1(x_u,\log d_v))).
% \end{align*}
% %Theoretically, we need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2)
% %$\text{MLP}_2: \mathbb{R}^{|e|} \rightarrow \mathbb{R}^{(|e|-1)*d+1}$; (3) $\text{MLP}_3: \mathbb{R}^{(|e|-1)*d+1} \rightarrow \mathbb{R}$.

% % \item Small invariant operator (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% % \begin{align*}
% %     \text{MLP}_2(\sum_{e:v\in e} \sum_{u\in e}\text{MLP}_1(x_u)).
% % \end{align*}
% % We know this cannot give universal approximation. But the parameter selection should be at least the same as equivariant operator.


% \item Big invariant operator: 
% \begin{align*}
%     \text{Linear}_3(\log d_v,\text{mean}_{e:v\in e} \text{MLP}_2(\log |e|, \text{mean}_{u\in e}\text{MLP}_1(x_u,\log d_u))).
% \end{align*}
% We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

% \item Attention-based (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% \begin{align*}
%     Attention_2(\log d_v,\text{MLP}_2(Attention_1(\log |e|,\{\text{MLP}_1(x_u)|u\in e\}))|e:v\in e).
% \end{align*}
% We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

% \end{itemize}



% \begin{itemize}
%     \item Equivariant operator: $\text{MLP}_1: 2\times 200, 200\times k$, $\text{MLP}_2: k+2\times 200,  200\times k+2$, $\text{Linear}_3: k+2\times 1$.
    
%     \item Fair equivariant operator: $\text{MLP}_1: 1\times 200, 200\times k$, $\text{MLP}_2: k+2\times 200, 200\times 200$. $\text{Linear}_3: 200\times 1$.
    
%     \item Jump-link + Invariant operator: $\text{MLP}_1: 1\times 200, 200\times k$,
%     $\text{MLP}_2: k+1\times 200, 200\times 200$
%     $\text{Linear}_3: 200+2\times 1$.

%     %\item Small Invariant operator: $\text{MLP}_1: 1\times 200, 200\times k$,
%     %$\text{MLP}_2: k\times 200, 200\times 1$.

%     \item Big Invariant operator: $\text{MLP}_1: 1\times 200, 200\times k$,
%     $\text{MLP}_2: k+1\times 200, 200\times 200$,
%     $\text{Linear}_3: 201\times 1$.   

%     \item Attention: $\text{MLP}_1: 1\times 200, 200\times k$,
%     $\text{Attention}_1: {k+1}\times {k+1}$,
%     $\text{MLP}_2: {k+1}\times 200, 200\times 200$,
%     $\text{Attention}_2: 201\times 1$.

% \end{itemize}

==> neurips 2022/section_tex_files/004-related.tex <==
\vspace{-2mm}
\section{Further Discussion on Related Works} \label{sec:related}
\vspace{-1mm}
We have discussed the most relevant works on HNN architectures and hypergraph diffusion algorithms in Sec.~\ref{sec:model}. Here, we review some relevant works on optimization-inspired NNs. Optimization-inspired NNs often get praised for their interpretability~\cite{monga2021algorithm,chen2021learning} and certified convergence under certain conditions of the learned operators~\cite{ryu2019plug,teodoro2017scene,chan2016plug}. Early works that adopt optimization-inspired NNs focus on the applications such as compressive sensing~\cite{gregor2010learning,xin2016maximal,liu2019alista, chen2018theoretical}, speech processing~\cite{hershey2014deep,wang2018end}, image denoising~\cite{zhang2017learning,meinhardt2017learning,rick2017one,chen2016trainable}, partitioning~\cite{zheng2015conditional,liu2017deep}, deblurring~\cite{schuler2015learning,li2020efficient} and so on. Recently, optimization-inspired NNs have also been applied to graphs~\cite{yang2021graph,liu2021elastic,chen2021graph,klicpera2019predict}. They unroll either learnable~\cite{yang2021graph,chen2021graph},  fixed $\ell_1$-norm~\cite{liu2021elastic} or fixed $\ell_2$-norm pair-wise potentials~\cite{klicpera2019predict} to formulate GNNs. Some works also view the graph diffusion as an ODE~\cite{chamberlain2021grand,thorpe2022grand++}, which essentially corresponds to our gradient descent Eq.~\ref{eqn:gd}. As there are only pairwise relations in graphs, the GNN design is often much simpler than the HNN counterpart. Neither expressivity nor equivariance has been investigated in these works. Implicit NNs~\cite{bai2019deep,el2021implicit} are to directly parameterize the optimum of an optimization problem. Implicit NNs have also been applied to graphs~\cite{dai2018learning,liu2021eignn,gu2020implicit,yang2021implicit} but not to hypergraphs. So, a future study of this work is to develop implicit models that can directly parameterize the solution to Eq.~\ref{eqn:diffusion}.    

%Recent works~\cite{gregor2010learning, liu2019alista, chen2018theoretical} that have shown that unrolling and parameterizing each iteration of an optimization problem with neural networks can express more universal objectives and achieve faster convergence, motivated by this line of works, we intend to construct a parametric hypergraph diffusion operator that can be learned from data. 

%Janossy pooling and others???

==> neurips 2022/section_tex_files/005-experiments.tex <==
\vspace{-2mm}
\section{Experiments} \label{sec:exp}
\vspace{-3mm}
\begin{table}[t]
\small{\caption{Dataset statistics. CE homophily is the homophily score~\cite{pei2020geom} based on CE of hypergraphs.}
\label{tab:dataset_stats}}
\centering
\resizebox{0.90\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
& Cora & Citeseer & Pubmed & Cora-CA & DBLP-CA & Congress & Senate & Walmart & House \\
\midrule
\# nodes & 2708 & 3312 & 19717 & 2708 & 41302 & 1718 & 282 & 88860 & 1290 \\
\# edges & 1579 & 1079 & 7963 & 1072 & 22363 & 83105 & 315 & 69906 & 340 \\
%\# features & 1433 & 3703 & 500 & 1433 & 1425 & 100 & 100 & 100 & 100 \\
\# classes & 7 & 6 & 3 & 7 & 6 & 2 & 2 & 11 & 2 \\
%avg. $d_v$ & 2.767 & 2.043 & 2.756 & 2.693 & 3.411 & 427.251 & 20.177 & 6.184 & 10.180 \\
avg. $|e|$ & 1.748 & 1.541 & 1.963 & 1.929 & 2.213 & 8.654 & 9.531 & 3.461 & 8.056 \\
CE Homophily & 0.897 & 0.893 & 0.952 & 0.803 & 0.869 & 0.555 & 0.498 & 0.530 & 0.509 \\
\bottomrule
\end{tabular}}
\vspace{-5mm}
\end{table}




\subsection{Results on Benchmarking Datasets} \label{sec:real-data-exp}
\vspace{-1mm}
\textbf{Experiment Setting.}
In this subsection, we evaluate \proj on nine real-world benchmarking hypergraphs. We focus on the semi-supervised node classification task. %in the transductive setting.
The nine datasets include co-citation networks (Cora, Citeseer, Pubmed), co-authorship networks (Cora-CA, DBLP-CA) \cite{yadati2019hypergcn}, Walmart \cite{amburg2020clustering}, House \cite{chodrow2021hypergraph}, Congress and Senate~\cite{fowler2006legislative,fowler2006connecting}. More details of these datasets can be found in Appendix~\ref{sec:dataset_detail}. Since the last four hypergraphs do not contain node attributes, we follow the method of \cite{chien2021you} to generate node features from label-dependent Gaussian distribution \cite{deshpande2018contextual}.

As we show in Table \ref{tab:dataset_stats}, these datasets already cover sufficiently diverse hypergraphs in terms of scale, structure, and homo-/heterophily.
We compare our method with top-performing models on these benchmarks, including HGNN \cite{feng2019hypergraph}, HCHA \cite{bai2021hypergraph}, HNHN \cite{dong2020hnhn}, HyperGCN \cite{yadati2019hypergcn}, %HyperSAGE \cite{arya2020hypersage}, 
UniGCNII \cite{huang2021unignn}, AllDeepSets \cite{chien2021you}, and AllSetTransformer \cite{chien2021you}.
All the hyperparameters for baselines follow from \cite{chien2021you} and we fix the learning rate, weight decay and other training recipes same with the baselines. Other model specific hyperparameters are obtained via grid search (see Appendix \ref{sec:hparam}). We randomly split the data into training/validation/test samples using 50\%/25\%/25\% splitting percentage by following \cite{chien2021you}. We choose prediction accuracy as the evaluation metric. We run each model for ten times with different training/validation splits to obtain the standard deviation. \vspace{-1mm}

\textbf{Performance Analysis.}
Table \ref{tab:real_data} shows the results. Our \proj uniformly outperforms all the compared models on all the datasets. We observe that the top-performing baseline models are AllSetTransformer, AllDeepSets and UniGCNII. %where the former two represent HNNs using two invariant multiset functions, while the later one improves traditional HNNs by initial and jumping links.
As having been analyzed in Sec.~\ref{sec:previous}, they model invariant set functions on both node and hyperedge sides. UniGCNII also adds initial and jump links, which accidentally resonates with our design principle (the step 4 in Algorithm 1). However, their performance has large variation across different datasets.
For example, UniGCNII attains promising performance on citation networks, however, has subpar results on Walmart dataset.
In contrast, our model achieves stably superior results, surpassing AllSet models by 12.9\% on Senate and UniGCNII by 12.5\% on Walmart.
We owe our empirical significance to the theoretical design of exact equivariant function representation. 
%While adopting set functions, AllSet models cannot capture equivariance.
%UniGCNII adopts jump links, but it is not as expressive as our \proj. 
Regarding the computational efficiency, we report the wall-clock times for training (for 100 epochs) and testing of all models over the largest hypergraph Walmart, where all models use the same hyperparameters that achieve the reported performance on the left. Our model achieves efficiency comparable to AllSet models~\cite{chien2021you} and is much faster than UniGCNII. So, the implementation of equivariant computation in \proj is still efficient. 
\begin{table}[t]
\small{\caption{Prediction Accuracy (\%). \textbf{Bold font$^\dagger$} highlights when \proj significantly (difference in means > 0.5 $\times$ std) outperforms all baselines. The \underline{best baselines} are underlined. The training and testing times are test on Walmart by using the same server with one GPU NVIDIA RTX A6000.}
\label{tab:real_data}}
\centering
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{cccccc|c}
\toprule
& Cora & Citeseer & Pubmed & Cora-CA & DBLP-CA & Training Time ($10^{-1}$ s) \\
\midrule
HGNN \cite{huang2021unignn} & \underline{79.39 $\pm$ 1.36} & 72.45 $\pm$ 1.16 & 86.44 $\pm$ 0.44 & 82.64 $\pm$ 1.65 & 91.03 $\pm$ 0.20 & 0.24 $\pm$ 0.51 \\
HCHA \cite{bai2021hypergraph} & 79.14 $\pm$ 1.02 & 72.42 $\pm$ 1.42 & 86.41 $\pm$ 0.36 & 82.55 $\pm$ 0.97 & 90.92 $\pm$ 0.22 & 0.24 ± 0.01 \\
HNHN \cite{dong2020hnhn} & 76.36 $\pm$ 1.92 & 72.64 $\pm$ 1.57 & 86.90 $\pm$ 0.30 & 77.19 $\pm$ 1.49 & 86.78 $\pm$ 0.29 & 0.30 $\pm$ 0.56 \\
HyperGCN \cite{yadati2019hypergcn} & 78.45 $\pm$ 1.26 & 71.28 $\pm$ 0.82 & 82.84 $\pm$ 8.67 & 79.48 $\pm$ 2.08 & 89.38 $\pm$ 0.25 & 0.42 $\pm$ 1.51 \\
%HyperSAGE \cite{arya2020hypersage} & 78.23 $\pm$ 1.30 & 73.06 $\pm$ 1.48 & 88.72 $\pm$ 0.53 & 81.92 $\pm$ 1.04 & 91.49 $\pm$ 0.21 & 0.71 $\pm$ 0.81 \\
UniGCNII \cite{huang2021unignn} & 78.81 $\pm$ 1.05 & 73.05 $\pm$ 2.21 & 88.25 $\pm$ 0.40 & \underline{83.60 $\pm$ 1.14} & \underline{91.69 $\pm$ 0.19} & 4.36 $\pm$ 1.18 \\
AllDeepSets \cite{chien2021you} & 76.88 $\pm$ 1.80 & 70.83 $\pm$ 1.63 & \underline{88.75 $\pm$ 0.33} & 81.97 $\pm$ 1.50 & 91.27 $\pm$ 0.27 & 1.23 $\pm$ 1.09\\
AllSetTransformer \cite{chien2021you} & 78.58 $\pm$ 1.47 & \underline{73.08 $\pm$ 1.20} & 88.72 $\pm$ 0.37 & 83.63 $\pm$ 1.47 & 91.53 $\pm$ 0.23 & 1.64 $\pm$ 1.63 \\
\midrule
\proj (ours) & \textbf{80.31 $\pm$ 1.35}$^\dagger$ & \textbf{73.70 $\pm$ 1.38}$^\dagger$ & \textbf{89.03 $\pm$ 0.53}$^\dagger$ & 83.97 $\pm$ 1.55 & \textbf{91.90 $\pm$ 0.19}$^\dagger$ & 1.71 $\pm$ 1.13 \\
% \projtwo & 77.47 $\pm$ 1.62 & 72.65 $\pm$ 1.56 & 88.86 $\pm$ 0.40 & 82.17 $\pm$ 1.68 & 91.62 $\pm$ 0.29 \\
% ED-HNN Attn. & 78.63 $\pm$ 1.55 & 71.21 $\pm$ 1.37 & 88.74 $\pm$ 0.37 & 82.33 $\pm$ 1.74 & 91.84 $\pm$ 0.25 \\
\bottomrule
& Congress & Senate & Walmart & House & Avg. Rank & Inference Time ($10^{-2}$ s)\\
\midrule
HGNN \cite{huang2021unignn} & 91.26 $\pm$ 1.15 & 48.59 $\pm$ 4.52 & 62.00 $\pm$ 0.24 & 61.39 $\pm$ 2.96  & 4.89 & 1.01 $\pm$ 0.04 \\
HCHA \cite{bai2021hypergraph} & 90.43 $\pm$ 1.20 & 48.62 $\pm$ 4.41 & 62.35 $\pm$ 0.26 & 61.36 $\pm$ 2.53 & 5.44 & 1.54 $\pm$ 0.18 \\
HNHN \cite{dong2020hnhn} & 53.35 $\pm$ 1.45 & 50.93 $\pm$ 6.33 & 47.18 $\pm$ 0.35 & 67.80 $\pm$ 2.59 & 7.11 & 6.11 $\pm$ 0.05\\
HyperGCN \cite{yadati2019hypergcn} & 55.12 $\pm$ 1.96 & 42.45 $\pm$ 3.67 & 44.74 $\pm$ 2.81 & 48.32 $\pm$ 2.93 & 7.33 & 0.87 $\pm$ 0.06 \\
%HyperSAGE \cite{arya2020hypersage} & 92.12 $\pm$ 0.94 & \underline{55.56 $\pm$ 5.27} & 59.14 $\pm$ 0.45 & 68.40 $\pm$ 3.07 & 4.33 & 1.17 $\pm$ 0.02 \\
UniGCNII \cite{huang2021unignn} & \underline{94.81 $\pm$ 0.81} & 49.30 $\pm$ 4.25 & 54.45 $\pm$ 0.37 & 67.25 $\pm$ 2.57 & 3.67 & 21.22 $\pm$ 0.13\\
AllDeepSets \cite{chien2021you} & 91.80 $\pm$ 1.53 & 48.17 $\pm$ 5.67 & 64.55 $\pm$ 0.33 & 67.82 $\pm$ 2.40  & 4.89 & 5.35 $\pm$ 0.33 \\
AllSetTransformer \cite{chien2021you} & 92.16 $\pm$ 1.05 & \underline{51.83 $\pm$ 5.22} & \underline{65.46 $\pm$ 0.25} & \underline{69.33 $\pm$ 2.20} & 2.67 & 6.06 $\pm$ 0.67 \\
\midrule
\proj (ours) & 95.00 $\pm$ 0.99 & \textbf{64.79 $\pm$ 5.14}$^\dagger$ & \textbf{66.91 $\pm$ 0.41}$^\dagger$ & \textbf{72.45 $\pm$ 2.28}$^\dagger$ & 1.00 & 5.87 $\pm$ 0.36 \\
% \projtwo & 95.19 $\pm$ 1.34 & 65.01 $\pm$ 6.17 & 65.24 $\pm$ 0.45 & 70.95 $\pm$ 1.97 \\
% ED-HNN Attn. & 95.24 $\pm$ 1.48 & 65.32 $\pm$ 6.72 & 67.06 $\pm$ 0.53 & 71.10 $\pm$ 2.65 \\
\bottomrule
\end{tabular}}
\vspace{-4mm}
\end{table}

%\paragraph{Efficiency Analysis}


\vspace{-2mm}
\subsection{Results on Synthetic Heterophilic Hypergraph Dataset}
\vspace{-2mm}
\begin{table}[t]
\small{\caption{Prediction Accuracy (\%) over Synthetic Hypergraphs with Controlled Heterophily $\alpha$.}
\label{tab:syn_node_data}}
\centering
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{} & \multicolumn{2}{c}{Homophily} & \multicolumn{4}{c}{Heterophily} \\
& $\alpha = 1$ & $\alpha = 2$ & $\alpha = 3$ & $\alpha = 4$ & $\alpha = 6$ & $\alpha = 7$ \\
\midrule
HGNN \cite{huang2021unignn} & 99.86 $\pm$ 0.05 & 90.42 $\pm$ 1.14 & 66.60 $\pm$ 1.60 & 57.90 $\pm$ 1.43 & 50.77 $\pm$ 1.94 & 48.68 $\pm$ 1.21 \\
HGNN + JumpLink \cite{huang2021unignn} & 99.29 $\pm$ 0.19 & 92.61 $\pm$ 0.97 & 79.59 $\pm$ 2.32 & 64.39 $\pm$ 1.55 & 55.39 $\pm$ 2.01 & 51.14 $\pm$ 2.05 \\
AllDeepSets \cite{chien2021you} & 99.86 $\pm$ 0.07 & 99.13 $\pm$ 0.31 & 92.39 $\pm$ 1.68 & 80.12 $\pm$ 2.31 & 56.42 $\pm$ 0.85 & 52.14 $\pm$ 2.88 \\
AllDeepSets + JumpLink \cite{huang2021unignn} & 99.95 $\pm$ 0.07 & 99.08 $\pm$ 0.24 & 93.52 $\pm$ 1.31 & 83.45 $\pm$ 2.64 & 59.68 $\pm$ 1.27 & 52.21 $\pm$ 2.36 \\
AllSetTransformer \cite{chien2021you} & 98.60 $\pm$ 0.48 & 95.89 $\pm$ 0.90 & 88.38 $\pm$ 1.81 & 83.34 $\pm$ 1.33 & 54.13 $\pm$ 4.83 & 50.15 $\pm$ 1.73 \\
\midrule
\proj (ours)  & 99.95 $\pm$ 0.08 & \textbf{99.68 $\pm$ 0.13}$^{\dagger}$ & \textbf{95.37 $\pm$ 1.23}$^{\dagger}$ & \textbf{90.35 $\pm$ 0.83}$^{\dagger}$ & \textbf{65.58 $\pm$ 0.76}$^{\dagger}$ & \textbf{54.31 $\pm$ 2.40}$^{\dagger}$ \\
\bottomrule
\end{tabular}}
\vspace{-6mm}
\end{table}

\paragraph{Experiment Setting.} As discussed, \proj is expected to perform well on heterophilic hypergraphs. We evaluate this point by using synthetic datasets with controlled heterophily.
%In this section, we verify our argument by synthetic datasets with controlled heterophily.
We generate data by using contextual hypergraph stochastic block model~\cite{deshpande2018contextual,ghoshdastidar2014consistency,chien2018community}. Specifically, we draw two classes of $2,500$ nodes each and then randomly sample 1,000 hyperedges. Each hyperedge consists of 15 nodes, among which $\alpha_i$ many are sampled from class $i$. We use $\alpha=\min\{\alpha_1,\alpha_2\}$ to denote the heterophily level. % from two classes with respect to a ratio $\alpha$.
%This ratio determines how many nodes with the same label will be connected by a hyperedge, which controls the homo-/heterophily of the hypergraphs. 
Afterwards, we generate label-dependent Gaussian node features.
We test both homophilic ($\alpha=1,2$ or CE homophily$\ge 0.7$) and heterophilic ($\alpha=4\sim 7$ or CE homophily $\le 0.7$) cases.
We compare \proj with HGNN \cite{feng2019hypergraph}, AllSet models \cite{chien2021you} and their variants with jump links. We follow previous 50\%/25\%/25\% data splitting methods and repeated 10 times the experiment.

\textbf{Results.} Table \ref{tab:syn_node_data} shows the results.
On homophilic datasets, all the models can achieve good results, while \proj keeps slightly better than others. Once $\alpha$ surpasses 3, i.e., entering the heterophilic regime, the superiority of \proj is more obvious. The jump-link trick indeed also helps, while building equivariance as \proj does directly provides more significant improvement.  
% Even for $\alpha = 0.3$ case, where half of neighboring nodes are labelled differently \pan{why this is half?}, our \proj can achieve 90.35\% prediction accuracy.
%Even for $\alpha = 4$ case, our \proj can still achieve 90.35\% prediction accuracy.
%Another interesting finding is that $\alpha = 7$ reaches the maximum tolerance to heterophily of all presented works.
\vspace{-2mm}
\subsection{Benefits in Deepening Hypergraph Neural Networks} \label{sec:depth_benefit}
\vspace{-1mm}
We also demonstrate that by using diffusion models and parameter tying, \proj can benefit from deeper architectures, while other HNNs cannot. % to achieve.
Fig.~\ref{fig:expr_depth} illustrates the performance of different models versus the number of network layers.
We compare with HGNN \cite{feng2019hypergraph}, AllSet models \cite{chien2021you}, and UniGCNII \cite{huang2021unignn}. UniGCNII inherits from~\cite{chen2020simple} which is known to be effective to counteract oversmoothness. The results reveal that AllSet models suffer from going deep. %Once the depth grows larger than 2, their performance declines rapidly.
HGNN working through more lightweight mechanism has better tolerance to depth. However, none of them can benefit from deepening.
On the contrary, \proj successfully leverages deeper architecture to achieve higher accuracy. For example, adding more layers boosts \proj by \textasciitilde1\% in accuracy on Pubmed and House, while elevating \proj from 58.01\% to 64.79\% on Senate dataset.

\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{images/depth.pdf}
\vspace{-3mm}
\small{\caption{Comparing Deep Achitectures across Different Models: Test Acc. v.s. \# Layers}\label{fig:expr_depth}}
\vspace{-3mm}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{images/dim_reduction.pdf}
\vspace{-2mm}
\small{\caption{Comparing the Powers to Represent known Diffusion: MAE v.s. Latent Dimensions}
\label{fig:expr_width}}
\vspace{-10mm}
\end{figure}
\vspace{-2mm}
\subsection{Expressiveness Justification on the Synthetic Diffusion Dataset}
\vspace{-1mm}
We are to evaluate the ability of \proj to express given hypergraph diffusion. We generate semi-synthetic diffusion data using the Senate hypergraph~\cite{chodrow2021hypergraph} and synthetic node features. The data consists of 1,000 pairs $(\Mat{H}^{(0)}, \Mat{H}^{(1)})$. The initial node features $\Mat{H}^{(0)}$ are sampled from 1-dim Gaussian distributions. To obtain $\Mat{H}^{(1)}$ we apply the gradient step in Eq.~\ref{eqn:gd}. For non-differential cases, we adopt subgradients for convenient computation. We fix node potentials as $f(\Mat{h}_v; \Mat{x}_v) = (\Mat{h}_v - \Mat{x}_v)^2$ and consider 3 different edge potentials in Example~\ref{exp:potential} with varying complexities: a) CE, b) TV ($p$=2) and c) LEC. The goal is to let one-layer models $\mathcal{V}\rightarrow\mathcal{E}\rightarrow\mathcal{V}$ to recover $\Mat{H}^{(1)}$.  We compare \proj with our implemented baseline (Invariant) with parameterized invariant set functions on both the node and hyperedge sides, and AllSet models \cite{chien2021you} that also adopt invariant set functions. We keep the scale of all models almost the same to give fair comparison, of which more details are given in Appendix~\ref{sec:diffusion_dataset}. The results are reported in Fig.~\ref{fig:expr_width}. The CE case gives invariant diffusion so all models can learn it well. The TV case mostly shows the benefit of the equivariant architecture, where the error almost does not increase even when the dimension decreases to 32. The LEC case is challenging for all models, though \proj is still the best. The reason, we think, is that learning the sorting operation in LEC via the sum pooling in Eq.~\ref{eq:equi-form} is empirically challenging albeit theoretically doable. A similar phenomenon has been observed in previous literatures~\cite{murphy2018janossy,wagstaff2019limitations}.  



% \begin{itemize}
% \item Equivariant operator:
% \begin{align*}
%     (x_v, x_v^{(0)}, \log d_v,\text{mean}(\text{MLP}_2(x_v, \log |e|, \text{mean}(\text{MLP}_1(x_u))))).
% \end{align*}

% \begin{align*}
% h_e^{(t)} = \text{mean}_u(\text{MLP}_1(h_u^{(t-1)}))\\
% m_{v\leftarrow e}^{(t)}=(h_v^{(t-1)}, \log |e|, h_e^{(t)}) \\
% h_v'^{(t)}= \text{mean}_{e:v\in e}\text{MLP}_2 (m_{v\leftarrow e}^{(t)})\\
% h_v^{(t)}= 
% (h_v^{(t-1)},x_v^{(0)}, \log d_v,h_v'^{(t)})
% \end{align*}

% \item double equi. 
% \begin{align*}
% h_e^{(t)} = \text{mean}_u(\text{MLP}_1(m_{u\rightarrow e}^{(t-1)}))\\
% m_{v\leftarrow e}^{(t)}=(h_v^{(t-1)}, \log |e|, h_e^{(t)}) \\
% h_v^{(t)}= \text{mean}_{e:v\in e}\text{MLP}_2 (m_{v\leftarrow e}^{(t)})\\
% m_{v\rightarrow e}^{(t)}= 
% (h_v^{(t-1)},h_e^{(t)}, x_v^{(0)}, \log d_v, h_v^{(t)})
% \end{align*}

% \end{itemize}

% 1. Synthetic data on one-step hypergraph diffusion to demonstrate the theory. Study the dependence on the model size. 

% 2. Synthetic data on node classification across different heterophilic levels of hypergraphs generated by stochastic block models. 

% 3. Real datasets experiments. 

==> neurips 2022/section_tex_files/006-conclusion.tex <==
\vspace{-3mm}
\section{Conclusion} 
\vspace{-2mm}
This work introduces a new hypergraph neural network \proj that can model   hypergraph diffusion process. We show that any hypergraph diffusion with permutation-invariant potential functions can be represented by iterating equivariant diffusion operators. \proj provides an efficient way to model such operators based on the commonly-used GNN platforms. \proj shows superiority in processing heterophilic hypergraphs and constructing deep models. In the future, we would like to apply \proj to other tasks such as hypergraph regression tasks and develop implicit HNNs that can directly optimize the optima of hypergraph diffusion problems.   

==> neurips 2022/section_tex_files/008-other-proofs.tex <==
\section{Proof of Theorem~\ref{thm:equivarnt_form_Fdim}} \label{sec:proof-equi-Fdim}
Suppose $X = [x_1^T, x_2^T, ..., x_F^T]^T\in \mathbb{R}^{kF}$. Define $W=[w_{ij}]\in\mathbb{R}^{K\times F}$ and $Z = [\bar{z}_1^T,\bar{z}_2^T,...,\bar{z}_K^T]^T\in\mathbb{R}^{KF}$, where 
\begin{align*}
    \bar{z}_i = \sum_{j=1}^F w_{ij}x_j.
\end{align*}
So, $\bar{Z} = (W\otimes I) X$. Define $A = W\otimes I$. Choose $\text{rank}(W)= F$ and let $\text{rank}(A) = F\times M$. 

Define $Z_P = [(P_1\bar{z}_1)^T,(P_2\bar{z}_2)^T,...,(P_K\bar{z}_K)^T]^T$, for some $P = \text{diag}(P_1, P_2, ..., P_K)$. What we have observed is one $Z_{P^*}$ for some $P^* = \text{diag}(P_1^*, P_2^*, ..., P_K^*)$.

For any $P$, we consider doing regression
\begin{align*}
    \hat{X}_P = \arg\min_X \|Z_P - AX\|_2^2.
\end{align*}
And compute $l_P=\|Z_P - A\hat{X}_P\|_2$. We have to check whether there are equivalence between (i) $l_P = 0$ and (ii) $P = P^*\text{diag}(Q,Q,...,Q)$ if there are no elements in $x_i$ are equal.

Let us measure $l_P$. First, $Z_P = PAX$. $\hat{X}_P = A^{\dagger}Z_P = (A^TA)^{-1}AZ_P = (A^TA)^{-1}APAX$. Therefore,
\begin{align*}
    l_{P} &= \|Z_P - AA^{\dagger}Z_P\| \\ 
    & = \|Z_P - A(W^{\dagger}\otimes I) Z_P\| \\
    & = \|PAX - A(A^TA)^{-1}APAX\| \\
    & = \|P(W\otimes I)X - ((WW^{\dagger})\otimes I) P(W\otimes I)X\| \\
\end{align*}

Here,\[P(W\otimes I)=
\begin{bmatrix}
    w_{11}P_1 & w_{12}P_1 & ... & w_{1F}P_1 \\
    w_{21}P_2 & w_{22}P_2 & ... & w_{2F}P_2 \\
    ... & ... & ... & ... \\
    w_{K1}P_K & w_{K2}P_K & ... & w_{KF}P_K \\
\end{bmatrix}\]
And suppose $W = U\Sigma V^T$ define \[WW^{\dagger} = UU^T  = 
\begin{bmatrix}
    s_{11} & s_{12} & ... & s_{1K} \\
    s_{21} & s_{22} & ... & s_{2K} \\
    ... & ... & ... & ... \\
    s_{K1} & s_{K2} & ... & s_{KK} \\
\end{bmatrix}, \text{where}\,s_{ij} = U_i U_j^T.
\]
As $WW^{\dagger}W = W$, we have $\sum_{k=1}^Ks_{ik}w_{kj} = w_{ij}$. And $WW^{\dagger}WW^{\dagger}=WW^{\dagger}$ so $\sum_{k=1}^Ks_{ik}s_{kj} = s_{ij}$. Moreover, $s_{ij} = s_{ji}$. So $\sum_{k=1}^Ks_{ik}s_{jk} = s_{ij}$ and $\sum_{k\neq i}s_{ik}^2 = s_{ii} - s_{ii}^2$.

\[((WW^{\dagger})\otimes I) P(W\otimes I)=
\begin{bmatrix}
    s_{11}P_1 & s_{12}P_2 & ... & s_{1K}P_K \\
    s_{21}P_1 & s_{22}P_2 & ... & s_{2F}P_K \\
    ... & ... & ... & ... \\
    s_{K1}P_1 & s_{K2}P_2 & ... & s_{KF}P_K \\
\end{bmatrix}\begin{bmatrix}
    w_{11} & w_{12} & ... & w_{1F} \\
    w_{21} & w_{22} & ... & w_{2F} \\
    ... & ... & ... & ... \\
    w_{K1} & w_{K2} & ... & w_{KF} \\
\end{bmatrix}\]
\[=\begin{bmatrix}
    \sum_{k=1}^K s_{1k}w_{k1}P_k & \sum_{k=1}^K s_{1k}w_{k2}P_k & ... & \sum_{k=1}^K s_{1k}w_{kF}P_k \\
    \sum_{k=1}^K s_{2k}w_{k1}P_k & \sum_{k=1}^K s_{2k}w_{k2}P_k & ... & \sum_{k=1}^K s_{2k}w_{kF}P_k \\
    ... & ... & ... & ... \\
    \sum_{k=1}^K s_{Kk}w_{k1}P_k & \sum_{k=1}^K s_{Kk}w_{k2}P_k & ... & \sum_{k=1}^K s_{Kk}w_{kF}P_k \\
\end{bmatrix}
\]
\[=\begin{bmatrix}
    \sum_{k=1}^K s_{1k}w_{k1}P_k & \sum_{k=1}^K s_{1k}w_{k2}P_k & ... & \sum_{k=1}^K s_{1k}w_{kF}P_k \\
    \sum_{k=1}^K s_{2k}w_{k1}P_k & \sum_{k=1}^K s_{2k}w_{k2}P_k & ... & \sum_{k=1}^K s_{2k}w_{kF}P_k \\
    ... & ... & ... & ... \\
    \sum_{k=1}^K s_{Kk}w_{k1}P_k & \sum_{k=1}^K s_{Kk}w_{k2}P_k & ... & \sum_{k=1}^K s_{Kk}w_{kF}P_k \\
\end{bmatrix}
\]
So $P(W\otimes I) - ((WW^{\dagger})\otimes I) P(W\otimes I)$
\[=\\
\begin{bmatrix}
    \sum_{k\neq 1} s_{1k}w_{k1}(P_k-P_1) & \sum_{k\neq 2} s_{1k}w_{k2}(P_k-P_1) & ... & \sum_{k\neq F} s_{1k}w_{kF}(P_k-P_1) \\
    \sum_{k\neq 1} s_{2k}w_{k1}(P_k-P_2) & \sum_{k\neq 2} s_{2k}w_{k2}(P_k-P_2) & ... & \sum_{k\neq F} s_{2k}w_{kF}(P_k - P_2) \\
    ... & ... & ... & ... \\
    \sum_{k\neq 1} s_{Kk}w_{k1}(P_k-P_K) & \sum_{k\neq 2} s_{Kk}w_{k2}(P_k-P_K) & ... & \sum_{k\neq F} s_{Kk}w_{kF}(P_k - P_K) \\
\end{bmatrix}
\]
So $[P(W\otimes I) - ((WW^{\dagger})\otimes I) P(W\otimes I)]X$
\[=\\
\begin{bmatrix}
    \sum_{k} s_{1k}(P_k-P_1)\sum_{j=1}^F w_{kj}x_j  \\
    \sum_{k} s_{2k}(P_k-P_2)\sum_{j=1}^F w_{kj}x_j \\
    ... &  \\
    \sum_{k} s_{Kk}(P_k-P_K)\sum_{j=1}^F w_{kj}x_j \\
\end{bmatrix}
=\begin{bmatrix}
    \sum_{k} s_{1k}(P_k-P_1)\bar{z}_k  \\
    \sum_{k} s_{2k}(P_k-P_2)\bar{z}_k \\
    ... &  \\
    \sum_{k} s_{Kk}(P_k-P_K)\bar{z}_k \\
\end{bmatrix}
\]

As $\bar{Z} = (W\otimes I)X$, so $X = (W^{\dagger}\otimes I)\bar{Z}$ and $\bar{Z} = (WW^{\dagger}\otimes I)\bar{Z}$. And thus $\bar{z}_i = \sum_{j=1}^K s_{ij} \bar{z}_j$. So we also have $P(W\otimes I) - ((WW^{\dagger})\otimes I) P(W\otimes I)X$
\[\begin{bmatrix}
    \sum_{k} s_{1k}P_k\bar{z}_k  - P_1 \bar{z}_1  \\
    \sum_{k} s_{2k}P_k\bar{z}_k - P_2 \bar{z}_2 \\
    ... &  \\
    \sum_{k} s_{Kk}P_k\bar{z}_k - P_K \bar{z}_K \\
\end{bmatrix}
\]
As, we only care about $l_P = \|P(W\otimes I) - ((WW^{\dagger})\otimes I) P(W\otimes I)X\|_2^2$. So, we may check
\[\begin{bmatrix}
    \sum_{k} s_{1k}(P_1^TP_k)\bar{z}_k  - \bar{z}_1  \\
    \sum_{k} s_{2k}(P_2^TP_k)\bar{z}_k - \bar{z}_2 \\
    ... &  \\
    \sum_{k} s_{Kk}(P_K^TP_k)\bar{z}_k - \bar{z}_K \\
\end{bmatrix}
=\begin{bmatrix}
    \sum_{k} s_{1k}(P_1^TP_k - I)\bar{z}_k\\
    \sum_{k} s_{2k}(P_2^TP_k - I)\bar{z}_k\\
    ... &  \\
    \sum_{k} s_{Kk}(P_K^TP_k - I)\bar{z}_k \\
\end{bmatrix}
\]

$l_p=0$ means 
\[\begin{matrix}
    \sum_{k} s_{1k}(P_1^TP_k)\bar{z}_k  = \bar{z}_1  \\
    \sum_{k} s_{2k}(P_2^TP_k)\bar{z}_k = \bar{z}_2 \\
    ...\\
    \sum_{k} s_{Kk}(P_K^TP_k)\bar{z}_k = \bar{z}_K \\
    \end{matrix}
\]
Let $S = WW^{\dagger}\otimes I$. That is 
\[ P^TSP \bar{Z} = \bar{Z}. 
\]
That is 
\[ P^T(S - I)P \bar{Z} = 0. 
\]
That is 
\[ (S - I)P \bar{Z} = 0.
\]
That is 
\[ (S - I)P AX = 0.
\]
That is 
\[ [(WW^{\dagger} - I) \otimes I] P [W\otimes I] X = 0.
\]
That is 
\[\begin{bmatrix}
    (s_{11} - 1)P_1 & s_{12}P_2 & ... & s_{1K}P_K  \\
     s_{21}P_1  & (s_{22} - 1)P_2 & ... & s_{2K}P_K  \\
    ... & ... & ... & ...\\
 s_{K1}P_1  & s_{K2}P_2 & ... & (s_{KK} - 1)P_K  \\
    \end{bmatrix} 
 \begin{bmatrix}
    w_{11}I & w_{12}I & ... & w_{1F}I  \\
     w_{21}I  & w_{22}I & ... & w_{2F}I  \\
    ... & ... & ... & ...\\
 w_{K1}I  & w_{K2}I & ... & w_{KF} I  \\
    \end{bmatrix} X = 0   
\]
% \[\begin{bmatrix}
%     \sum_{k}w_{k1}s_{1k}P_k - w_{11}P_1 & s_{12}P_2 & ... & s_{1K}P_K  \\
%      s_{21}P_1  & (s_{22} - 1)P_2 & ... & s_{2K}P_K  \\
%     ... & ... & ... & ...\\
%  s_{K1}P_1  & s_{K2}P_2 & ... & (s_{KK} - 1)P_K  \\
%     \end{bmatrix} 
%  \begin{bmatrix}
%     w_{11}I & w_{12}I & ... & w_{1F}I  \\
%      w_{21}I  & w_{22}I & ... & w_{2K}I  \\
%     ... & ... & ... & ...\\
%  w_{K1}I  & w_{K2}I & ... & w_{KK} I  \\
%     \end{bmatrix} X = 0
% \]
To make $\text{rank}(WW^{\dagger} - I) \geq F$ where we need to have $K\geq 2F$. 

We need to prove that for any $X$ without trivial perm (entry-pair different), for any $P\neq I$, $[(WW^{\dagger} - I) \otimes I] P [W\otimes I] X\neq 0$. 

If one $P\neq I$ or $Q$ makes $[(WW^{\dagger} - I) \otimes I] P [W\otimes I] X= 0$, then $X$ exists two same rows.

Note that as $Z_P = P [W\otimes I] X$. $[(WW^{\dagger} - I) \otimes I]Z_P =0$ means 
$Z_P'(WW^{\dagger} - I)=0$ where $Z_P'$ reshapes $Z_P$, as $Z_P' = [P_1z_1, P_2z_2,...,P_Kz_K]$. This further means there exists an $Y_P = [y_{1,P}, y_{2,P},...,y_{F,P}]$ such that \[
Z_P' = Y_P W^T.
\]
Moreover, let $\bar{Z}' = [z_1, z_2,...,z_K]$ and $X = [x_1,x_2,...,x_F]$.
\[
\bar{Z}' = X' W^T.
\]


Optionally include extra information (complete proofs, additional experiments and plots) in the appendix.
This section will often be part of the supplemental material.

\begin{definition} [Pair-wise Alignment]
Consider two vectors $x, y\in\mathbb{R}^{M}$ and two permutation matrices $P_x,P_y\in \Pi(M)$. If there exists a permutation matrix $Q\in \Pi(M)$ such that $QP_xx = x$ and $QP_yy=y$, we call $(P_x,P_y)$ is $(x,y)$-aligned.  
\end{definition}

Vector-pair alignment has the following properties. 
\begin{remark}
If both $x$ and $y$ have no duplicated entries, $(P_x,P_y)$ is $(x,y)$-aligned, then $P_x = P_y$. 
\end{remark}

\pan{I find the next lemma that uses pairwise alignment to provide all alignment is generally wrong. Think about one example: $x_1 = [2,1,1,2]$  and  $P_{x_1}x_1 = [1,2,1,2]$, $x_2=[1,2,1,2]$ and $P_{x_2}x_2=[1,2,1,2]$, $x_3=[1,1,2,2]$ and $P_{x_3}x_3 = [1,1,2,2]$. We can see that $(P_{x_i},P_{x_j})$ is $(x_{i},x_{j})$-aligned but they are not jointly aligned.
\begin{lemma} [Alignment Union]
Consider multiple vectors $x_1, x_2, ..., x_F\in\mathbb{R}^{M}$ and the corresponding permutation matrices $P_{x_1},P_{x_2},..., P_{x_F}\in \Pi(M)$. If for any two vectors $x_i,x_j$, $(P_{x_i}, P_{x_j})$ is $(x_i,x_j)$-aligned, then there exists a $Q$ such that $QP_{x_k}x_k = x_k$ for all $k\in[F]$. $(P_{x_1}, P_{x_2},..., P_{x_F})$ is called $(x_1,x_2,...,x_F)$-aligned.
\end{lemma}
\begin{proof}
We use induction. It is trivial when $F=2$. Suppose the statement is true when $F< k$, for some $k\geq 3$. We consider the case $F = k$. 

Without loss of generality, we may assume $P_{x_k}=I$ because the statement is equivalent when we replace all $P_{x_i}$ with $P_{x_k}^T P_{x_i}$.
%$(P_{x_1}, P_{x_2},..., P_{x_k})$ being $(x_1,x_2,...,x_k)$-aligned is equivalent to $(P_{x_k}^T P_{x_1}, P_{x_k}^T P_{x_2},..., I)$ being $(x_1,x_2,...,x_k)$-aligned.
As when $F\leq k$, the statement is true. We know there exists a $Q\in \Pi(M)$ such that $QP_{x_i}x_i = x_i$ for all $i\in[k-1]$. Moreover, for $i\in[k-1]$, there exists $Q_iP_{x_{i}}x_i = x_i$ and $Q_ix_k = x_k$. Next, we are to use $Q$ and $Q_i$, $i\in[k-1]$ to construct a $Q'\in \Pi(M)$ such that $Q'x_k=x_k$ and $Q'P_{x_{i}}x_i = x_i$ for all $i\in[k-1]$.

We partition the index set $[M]$ into several blocks $B_1, B_2, ..., B_m$ such that the indices $i,j\in[M]$ are in the same block if and only if $x_{k,i}=x_{k,j}$. Therefore, for any permutation matrix $P$, $Px_k = x_k$, if and only if for any $h\in[m]$ and for for any $j\in B_h$, $\pi_{P}(j)\in B_h$. Here, $\pi_P:[M]\rightarrow [M]$ is the permutation function corresponding to the permutation matrix $P$ in the sense that $P_{ij}=1$ if and only if $i = \pi_P(j)$. We call this permutation matrix that satisfies the previous condition as an $x_k$-friendly matrix. So, for any $i\in[k-1]$, $Q_i$ is an $x_k$-friendly matrix.

For the permutation matrix $Q$, we define a conflicting score $C_Q = \sum_{h=1}^m \sum_{j\in B_h} 1_{\pi_Q(j)\notin B_h}$. If $C_Q=0$, then $Q$ is an $x_k$-friendly matrix so $Qx_k = x_k$, which proves what we need. If $C_Q>0$, we define a way to adjust $Q$ to monotonically decrease $C_Q$.

As $C_Q>0$, there is one $h\in[m]$ and $j\in B_h$, $\pi_Q(j)\in B_{h'}$ where $h'\neq h$. As for all $i\in[k-1]$, $QP_{x_i}x_i = x_i$, $(P_{x_i}x_i)_{j} = (x_i)_{\pi_Q(j)}$. Moreover, $Q_iP_{x_i}x_i = x_i$, $(P_{x_i}x_i)_{j} = (x_i)_{\pi_{Q_i}(j)}$. So, for all $i\in[k-1]$, $(x_i)_{\pi_Q(j)} = (x_i)_{\pi_{Q_i}(j)}$. 


%We define a new $Q'$ such that $\pi_{Q'}(k) = $

%for any $j\in B_h$, $\pi_{Q_i}(j)\in B_h$ for any $i\in[k-1], h\in[m]$. Here, $\pi_P:[M]\rightarrow [M]$ is the permutation function corresponding to the permutation matrix $P$. 
\end{proof}}

\begin{definition} [Active Index Pairs]
Consider multiple vectors $x_1, x_2, ..., x_F\in\mathbb{R}^{M}$, we call an un-ordered pair $\{m,k\}\in[M]^2$ is an \emph{active index pair}, if there exists at least $i\in[F]$ such that $x_{i,m}\neq x_{i,k}$. Let the set $\mathcal{I_{\text{AIP}}}\subset [M]^2$ group all active index pairs.
\end{definition}

\begin{definition} [Anchor]
Consider multiple vectors $x_1, x_2, ..., x_F\in\mathbb{R}^{M}$. Let $\mathcal{I_{\text{AIP}}}\subset [M]^2$ be the set of active index pairs of $(x_1, x_2, ..., x_F)$.
For a vector, $x_0\in \mathbb{R}^{M}$, if $x_{0,m}\neq x_{0,k}$ for any active index pair $\{m,k\}\in\mathcal{I_{\text{AIP}}}$, we call $x_0$ is an \emph{anchor} of $(x_1, x_2, ..., x_F)$.
\end{definition}

\begin{lemma} [Alignment Union] \label{lm:union}
Consider multiple vectors $x_0, x_1, x_2, ..., x_F\in\mathbb{R}^{M}$ and the corresponding permutation matrices $P_{x_0}, P_{x_1},P_{x_2},..., P_{x_F}\in \Pi(M)$. If $x_0$ is an anchor of $(x_1, x_2, ..., x_F)$ and for any $i\in[F]$, $(P_{x_0}, P_{x_i})$ is $(x_0,x_i)$-aligned, then there exists a $Q$ such that $QP_{x_k}x_k = x_k$ for all $k\in[F]$. $(P_{x_1}, P_{x_2},..., P_{x_F})$ is called $(x_1,x_2,...,x_F)$-aligned.
\end{lemma}
\begin{proof}
As  $(P_{x_0}, P_{x_i})$ is $(x_0,x_i)$-aligned, there exists $Q_i\in\Pi(M)$, $Q_iP_{x_0}x_0 = x_0$ and $Q_iP_{x_i}x_i = x_i$. As $x_0$ is an anchor of $(x_1, x_2, ..., x_F)$, for any $Q\in\Pi(M)$ if $Qx_0 = x_0$, $Qx_i = x_i$ for any $i$. So, for each $i$, we may choose $Q_i'= P_{x_0}^TQ_i^T$ so $Q_i'x_0 = x_0$ and $Q_i'x_i=x_i$. Further, $Q_i'Q_iP_{x_i}x_i=x_i$, which means $P_{x_0}^TP_{x_i}x_i=x_i$. Therefore, $Q = P_{x_0}^T$ can make $QP_{x_k}x_k = x_k$ for all $k\in[F]$.
\end{proof}

\begin{lemma} [Anchor Construction] \label{lm:anchor}
Consider multiple vectors $x_1, x_2, ..., x_F\in\mathbb{R}^{M}$. Consider a set of weights $W =[w_{ji}]^{F\times K}$ where $K\geq M(M-1)(F-1)/2+1$ and for any $F$-sized subset of $[K]$, denoted by $\mathcal{I}$,  $\{w_{\cdot i}|i\in\mathcal{I}\}$ is linearly independent. Then, there exists one $i\in[K]$, $\sum_{j=1}^F x_{j}w_{ji}$ is an anchor of $(x_1, x_2, ..., x_F)$. 
\end{lemma}
\begin{proof}
    %As for any $F+1$-sized subset of $[K]$, denoted by $\mathcal{I}$, $\{w_{i\cdot}|i\in\mathcal{I}\}$ is linearly independent, $w_{ij}x_j$
    We consider an $F$-sized subset of $[K]$, denoted by $\mathcal{I}$.
    Because $\{w_{\cdot i}|i\in\mathcal{I}\}$ is linearly independent, for any active index pair $\{m,k\}\in\mathcal{I_{\text{AIP}}}$, there must exist $i\in\mathcal{I}$ such that $\sum_{j=1}^Fx_{j,m}w_{ji}\neq \sum_{j=1}^Fx_{j,k}w_{ji}$. Otherwise, there are $F$ equations on $a\in\mathbb{R}^F$ such that $\sum_{j=1}^Fw_{ji}a_j=0$, which implies $a=0$ and conflicts the fact that $x_{i,m}\neq x_{i,k}$ for some $i$.
    
    Therefore, for any active index pair $\{m,k\}\in\mathcal{I_{\text{AIP}}}$, at most $F-1$ many indices $i$ in $[K]$ such that $\sum_{j=1}^Fx_{j,m}w_{ji}= \sum_{j=1}^Fx_{j,k}w_{ji}$. Based on the pigeon-hole principle, as $K\geq (F-1){M \choose 2}+1\geq (F-1)|\mathcal{I_{\text{AIP}}}|+1$, there exists $i\in[K]$, $\sum_{j=1}^Fx_{j,m}w_{ji}\neq \sum_{j=1}^Fx_{j,k}w_{ij}$ for any any active index pair $\{m,k\}\in\mathcal{I_{\text{AIP}}}$.
\end{proof}

\begin{lemma} [Making Pair-wise Alignment] \label{lm:matching}
Consider two vectors $x, y\in\mathbb{R}^{M}$ and two permutation matrices $P_x,P_y\in \Pi(M)$. Consider a set of weights $\gamma=\{\gamma_1,\gamma_2,...,\gamma_K\}$, $\gamma_i\neq \gamma_j$, $\gamma_i\in\mathbb{R}$, $\gamma_i\neq 0$, $K\geq M(M-1)+1$, satisfy that for any 4  tuples $(\gamma_i,\gamma_j,\gamma_g,\gamma_h)\subset W$, if $\gamma_i\neq \gamma_j, \gamma_i\neq \gamma_g$, then $\gamma_i/\gamma_j \neq \gamma_g/\gamma_h$. If for any $i\in[K]$, there exists $Q_i\in \Pi(M)$ such that $Q_i(x - \gamma_iy) = P_xx-\gamma_iP_yy$, then $(P_x,P_y)$ is $(x,y)$-aligned. 
%If for a set of weights $W=\{\gamma_1,\gamma_2,...,\gamma_K\}$, $\gamma_i\neq \gamma_j$, $K\geq M(M+1)+1$ that satisfies for any 4 pair-wise different tuple $\{\gamma_i,\gamma_j,\gamma_g,\gamma_h\}\subset W$, $\gamma_i\gamma_j \neq \gamma_g\gamma_h$, 
\end{lemma}
\begin{proof}
For $x$, we define $M$ sets of different non-zero pair differences as $D_x^{(m)}=\{x_m-x_k|k\in[M], x_m-x_k\neq 0\}$ for $m\in[M]$. Similarly, we define $D_y^{(m)}$ for $y$, $m\in[M]$.

For $i\in[K]$, as $Q_i\in \Pi(M)$ makes $(I - Q_i^TP_x)x = \gamma_i(I - Q_i^TP_y)y$.
There are $M$ equalities. We consider the case that there exist at least one equality that are induced by $\alpha \in D_x^{(m)}$ (LHS of the equality) and $\beta \in D_y^{(m)}$ (RHS of the equality), for some $m\in[M]$ where $\alpha =  \gamma_i \beta$, $\alpha,\beta\neq 0$. Note that if there are no such an equality, we have $x= Q_i^TP_xx$ and $y = Q_i^TP_yy$, so $(P_x,P_y)$ is $(x,y)$-aligned, which proves the conclusion. Next, we prove that with large enough $K$, there must be an $i\in[K]$ without such an equality. 

Suppose for each $i\in[K]$, such an equality exists. Actually, for each $i\in[K]$, such equalities are at least two, because $1^T (I - Q_i^TP_x)x = 0$. If $\alpha\neq 0$, the sum of the LHS of rest equalites must be $-\alpha$.

Now, we consider pairing the values in $D_x^{(m)}$ and $D_y^{(m)}$. Construct $M$ bipartite graphs $G^{(m)}$, $m\in[M]$ where for each $m\in[M]$, the values in either $D_x^{(m)}$ or $D_y^{(m)}$ correspond to either one partite of nodes of $G^{(m)}$. Connect two nodes if the corresponding values satisfiy $\alpha=\gamma_i\beta$ for some $\gamma_i$, $i\in[K]$. 

For any two values $\alpha_1,\alpha_2 \in D_x^{(m)}$, there are at most one value $\beta\in D_y^{(m)}$. Then, $\alpha_1,\alpha_2$ are connected to $\beta$. Otherwise, suppose there is another $\beta'\in D_y^{(m)}$. Then, we have $\alpha_1 = \gamma_i \beta$, $\alpha_2 = \gamma_j \beta$, $\alpha_1 = \gamma_g \beta'$, $\alpha_2 = \gamma_h \beta'$. As $\alpha_1 \neq \alpha_2$, so $\gamma_i\neq \gamma_j$. Similarly, as $\beta\neq \beta'$, $\gamma_i\neq \gamma_g$. Then, we have the condition $\gamma_j/\gamma_i \neq \gamma_h/\gamma_g$, while it  induces a conflict because $\gamma_j/\gamma_i = \alpha_2/\alpha_1= \gamma_h/\gamma_g$.  

$|D_x^{(m)}|, |D_y^{(m)}|\leq M-1$. For a bipartite graph with at most $M-1$ nodes in each partite, the number of edges is at most $2(M-1)$ to guarantee that there do not exist two nodes sharing two common neighbors. So, overall, there are $2(M-1)M$ edges in $M$ graphs. Each $i\in[K]$ gives at least two edges. So, when $K\geq M(M-1)+1$, there are be a conflict, i.e., for some $i\in[K]$, $x= Q_i^TP_xx$ and $y = Q_i^TP_yy$ so $(P_x,P_y)$ is $(x,y)$-aligned.
\end{proof}

\begin{theorem}[Injective Mapping]\label{thm:injective}
There exists $W=[w_1,w_2,...,w_K]\in\mathbb{R}^{F\times K}$, where $K\geq M^4F^2\geq F+[M(M-1)(F-1)/2+1][M(M-1)F+F+1]$ that satisfies: Given $Z = [z_1, z_2,...,z_K]$ where $z_i = P_iXw_i$ for some unknown $P_i\in\Pi(M)$ and any $X = [x_1, x_2,...,x_F]\in\mathbb{R}^{M\times F}$, $f(Z)= QX$ for some $Q\in \Pi(M)$ exists. Here $Q$ may depend on $X$.
\end{theorem}
\begin{proof}
This proof combines the previous Lemma~\ref{lm:union}, Lemma~\ref{lm:anchor} and Lemma~\ref{lm:matching}.

We consider $W$ that consists of three parts $W=[W^{(1)}, W^{(2)}, W^{(3)}]$ as follows. 
\begin{itemize}
    \item For $W^{(1)}=[w_1^{(1)},...,w_{K_1}^{(1)}]\in\mathbb{R}^{F\times K_1}$ where $K_1 = F$, $w_i^{(1)}$ is 0-1 vector with only the $i$th component as 1 and others as 0.
    \item For $W^{(2)}=[w_1^{(2)},...,w_{K_2}^{(2)}]\in\mathbb{R}^{F\times K_2}$ where $K_2= M(M-1)(F-1)/2+1$, where $W^{(2)}$ satisfies the condition in Lemma~\ref{lm:anchor}, i.e., for any $F$-sized index subset $\mathcal{I}$ of $W^{(2)}$, $\{w_{i}^{(2)}|i\in \mathcal{I}\}$ is linearly independent. We know $W^{(2)}$ can be constructed with high probability by sampling entry-wise independent Gaussian random matrix. 
    \item $W^{(3)}$ can be further partitioned into $FK_2= F(M(M-1)(F-1)/2+1))$ blocks. $W^{(3)} = [W^{(3,1,1)},W^{(3,1,2)},...,W^{(3,1,F)},...,W^{(3,K_2,F)}]$ where each $W^{(3,i,j)}=[w_{1}^{(3,i,j)},...,w_{K_3}^{(3,i,j)}]\in\mathbb{R}^{F\times K_3}$ where $K_3 = M(M-1)+1$. Let $w_{k}^{(3,i,j)} = w_i^{(2)} - \gamma_kw_j^{(1)}$ where $\{\gamma_k\}_{k\in[K_3]}$ satisfy the condition in Lemma~\ref{lm:matching}. $\{\gamma_k\}_{k\in[K_3]}$ exists by setting $\gamma_k$ as the $k$th positive prime number. 
\end{itemize}

For the first block, for any $j\in[F]$, we have $z_j^{(1)}= Q_jXw_j^{(1)} = Q_jx_j$ for some unknown $Q_j\in\Pi(M)$. 

By using Lemma~\ref{lm:anchor}, there exists $\bar{z}_{i}^{(2)} = Xw_{i}^{(2)}$, for some $i\in[K_2]$, which is an anchor of $(x_1, x_2,...,x_F)$. And, there exists an unknown $U_z\in\Pi(M)$ such that in $Z$, we observe $ z_i^{(2)}=U_z\bar{z}_{i}^{(2)}$. So $z_i^{(2)}$ is an anchor of $(U_zx_1, U_zx_2,...,U_zx_F)$

Next, given the above $i$, we are to find the permutation matrices $P_{1}, P_{2},...,P_{F}$ such that $(I, P_{j}Q_jU_z^T)$ is $(z_i^{(2)}, U_zx_j)$-aligned for all $j\in[F]$. Because if so according to Lemma~\ref{lm:union}, there exists $Q\in\Pi(M)$ such that $QP_{j}Q_jU_z^TU_zx_j=U_zx_j$ which indicates $P_{j}z_j^{(1)}=Q^TU_zx_j$ for all $j\in [F]$. 

Next, we use $Z^{(3,i,j)}$ to find $P_{j}$ such that  $(I, P_{j}Q_jU_z^T)$ is $(z_i^{(2)}, U_zx_j)$-aligned. For each column of $Z^{(3,i,j)}$, say $z_k^{(3,i,j)}= \Sigma_kXw_{k}^{(3,i,j)}=\Sigma_kX(w_i^{(2)} - \gamma_kw_j^{(1)}) = \Sigma_k(\bar{z}_{i}^{(2)}- \gamma_k x_j)=\Sigma_kU_z^T(z_i^{(2)} -\gamma_k U_zx_j)$ for some unknown $\Sigma_k\in \Pi(k)$. 

The way to find $P_{j}$ is to check all $Q\in \Pi(M)$ such that for all $k\in[K_3]$, $z_i^{(2)}- \gamma_k Qz_j^{(1)}$ is a permutation of $z_k^{(3,i,j)}$, i.e., there exists $Q_k'\in \Pi(M)$ such that $z_i^{(2)}- \gamma_k Qz_j^{(1)} = Q_k'z_k^{(3,i,j)} = Q_k'\Sigma_kU_z^T(z_i^{(2)} -\gamma_k U_zx_j)$. We know at least one such $Q$ exists because we can set $Q=U_z$ (in this case, $Q_k'=\Sigma_k^TU_z$ satisfies the requirement). So, this procedure must have a solution. Once such $P_{j}$ is found, because $Q_k'\Sigma_kU_z^T(z_i^{(2)} -\gamma_k U_zx_j) = z_i^{(2)}- \gamma_k P_jz_j^{(1)} = z_i^{(2)}- \gamma_k P_jQ_jU_z^TU_zx_j$, we have that $(I, P_jQ_jU_z^T)$ is $(z_i^{(2)}, U_zx_j)$-aligned according to Lemma~\ref{lm:matching}. 

Overall, we construct $f(Z)$ via three steps: (1) Check $z_{i}^{(2)}$ for all $i\in[K_2]$ and find one $i \in \arg\max_{j\in[K_2]} \sum_{m,k\in[M]} z_{j,m}^{(2)}\neq z_{j,m}^{(2)}$; (2) For each $j\in[F]$, find $P_{j}$ by checking all $P_j\in \Pi(M)$ and find one $P_j$ such that for all $k\in[K_3]$, $z_i^{(2)}- \gamma_k P_jz_j^{(1)}$ is a permutation of $z_k^{(3,i,j)}$; (3) Output $(P_{1}z_1^{(1)}, P_{2}z_2^{(1)},...,P_{F}z_F^{(1)})$. The output will equal $Q(x_1,x_2,...,x_F)$ for some $Q\in \Pi(M)$, which satisfies the conclusion.

\end{proof}

\begin{corollary}[Precise Reconstruction]
For any permutation invariant function $f:\in\mathbb{R}^{M\times F}\rightarrow \mathbb{R}$ such that for any $P\in\Pi(M), \,X\in\mathbb{R}^{M\times F}$, $f(PX)=f(X)$. There exists an continuous function $\phi:\mathbb{R}^F\rightarrow \mathbb{R}^{MK}$ where $K\geq M^4F^2$, and a function $\rho: \mathbb{R}^{MK}\rightarrow\mathbb{R}$ such that $f(X)= \rho(\sum_{i=1}^M\phi(X_{i\cdot}))$ for any $X\in\mathbb{R}^{M\times F}$, where $X_{i\cdot}$ denotes the $i$th row of $X$.
\end{corollary}

\begin{proof}
The proof can be achieved by combing ~\cite{zaheer2017deepset} and Theorem~\ref{thm:injective}.
\end{proof}

\begin{lemma}[Injective Mapping with Anchor] \label{lm:injective-anchor}
There exists $W=[w_1,w_2,...,w_K]\in\mathbb{R}^{F\times K}$, where $K\geq M^2F\geq F+(F-1)[M(M-1)+1]$ such that given $Z = [z_1, z_2,...,z_K]$ where $z_i = P_iXw_i$ for some unknown $P_i\in\Pi(M)$ and any $X = [x_1, x_2,...,x_F]\in\mathbb{R}^{M\times F}$ with $x_{F}$ having no duplicated entries, a mapping $f(Z)= QX$ for some $Q\in \Pi(M)$ exists. Here $Q$ may depend on $X$.
\end{lemma}

\begin{proof}
The proof is similar to Theorem~\ref{thm:injective}. As one can directly use $x_1$ as the anchor, we just need to construct $W = [W^{(1)}, W^{(3)}]$ where $W^{(1)}$ is the same as the one in the proof of Theorem~\ref{thm:injective}. $W^{(3)}=[W^{(3,1)},W^{(3,2)},...,W^{(3,F-1)}]$ and $W^{(3,j)}$ just works as one $W^{(3,i,j)}$ in  Theorem~\ref{thm:injective}. Let $W^{(3,j)}=[w_1^{(3,j)},w_2^{(3,j)},...,w_{K_3}^{(3,j)}]\in\mathbb{R}^{F\times K_3}$ where $K_3\geq M(M-1)+1$. Here, $w_k^{(3,j)}= w_{F}^{(1)} - \gamma_kw_j^{(1)}$.
\end{proof}


\begin{theorem}[Approximate Continuous Reconstruction]
Consider $\epsilon>0$.  There exists $W=[w_1,w_2,...,w_K]\in\mathbb{R}^{F\times K}$ where $K\geq M^2F\geq F+(F-1)[M(M-1)+1]$ such that given $Z = [z_1, z_2,...,z_K]$ where $z_i = P_iXw_i$ for some unknown $P_i\in\Pi(M)$ and any $X = [x_1, x_2,...,x_F]\in[0,1]^{M\times F}$, there exists a continuous mapping $g(Z)$ such that $\min_{Q\in \Pi(M)}\|g(Z)-QX\|_F\leq\epsilon$.
\end{theorem}


% \begin{proof}
% The proof will use Lemma~\ref{lm:injective-anchor}.
% \end{proof}

\begin{corollary}[Approximate Continuous Reconstruction]
For any continuous permutation invariant function $f:[0,1]^{M\times F}\rightarrow \mathbb{R}$ such that for any $P\in\Pi(M), \,X\in\mathbb{R}^{M\times F}$, $f(PX)=f(X)$. There exists an continuous function $\phi:[0,1]^F\rightarrow    \mathbb{R}^{MK}$ where $K\geq M^2F$, and a continuous function $\rho: \mathbb{R}^{MK}\rightarrow\mathbb{R}$ such that $|f(X)- \rho(\sum_{i=1}^M\phi(X_{i\cdot}))|<\epsilon$, where $X_{i\cdot}$ denotes the $i$th row of $X$.
\end{corollary}

==> neurips 2022/section_tex_files/old-002-prelim.tex <==
\section{Hypergraphs, Hyperedge Operators and Hypergraph Diffusion} \label{sec:prelim}

% We are interested in supervised learning problems on hypergraphs by a diffusion model, in which we are given nodes with features and labels, as well as hyperedges connecting them.

In this section, we formulate the hypergraph diffusion problem, along the way, introduce the notations.
\begin{definition}[Hypergraph] \label{def:hypergraph}
Let $\Set{G} = (\Set{V}, \Set{E})$ be a hypergraph where $\Set{V} = \{v_1, \cdots, v_n\}$ is the set of $n$ \pan{revise to $N$} nodes and $\Set{E} = \{e_1, \cdots, e_m\}$ is the set of $m$ hyperedges  \pan{revise to $M$}. Each hyperedge $e = \{v_1^{(e)},...,v_{\lvert e \rvert}^{(e)}\} \in \Set{E}$ is a subset of node set $\Set{V}$, i.e., $e \subseteq \Set{V}$. 
Let $\Mat{K} \in \{0, 1\}^{n \times m}$ be the associated incident matrix where $\Mat{K}_{ij} = 1$ if and only if $v_i \in e_j$.
\end{definition}

Unlike ordinary graphs, a hyperedge can connect with more than two nodes, i.e., $\lvert e \rvert \ge 2$.
To attain node adjacent matrix (i.e., an $n$ by $n$ matrix whose non-zero entries indicate which two nodes are connected), one can use $\Mat{K}\Mat{K}^\top$ that transforms hyperedges into cliques.
\begin{definition}[Node features] \label{def:node_feat}
Let $\Mat{h}_i \in \real^d$  \pan{revise to $F$} be the node embedding of the node $v_i \in \Set{V}$. We organize all the node features into the rows of a feature matrix $\Mat{H} = \begin{bmatrix} \Mat{h}_{1} & \cdots & \Mat{h}_{n} \end{bmatrix}^\top \in \real^{n \times d}$. Suppose each node has initial features $\Mat{x}_i \in \real^d$ which are organized by initial feature matrix $\Mat{X} \in \real^{n \times d}$.
\end{definition}

% Similarly, we let matrix $\Mat{H} = \begin{bmatrix} \Mat{h}_{1} & \cdots & \Mat{h}_{n} \end{bmatrix}^\top \in \real^{n \times d}$ concatenates all the node features after diffusion.
\begin{definition}[Edge features] \label{def:edge_feat}
% Given an hyperedge $e \in \Set{E}$, the 
Let edge feature matrix $\Mat{H}_e = \begin{bmatrix} \Mat{h}_{e, 1} & \cdots & \Mat{h}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert \times d}$ collect all the feature vectors of nodes within edge $e$, where $\Mat{h}_{e,i}$ corresponds to the node features of node $v_i^{(e)}$ inside hyperedge $e$. \pan{Define the relation between $\Mat{h}_{e}$ and $\Mat{h}$. Denote an implicit mapping between $(e,i)$ and $(e,v)$.}
\end{definition}

Hypergraph diffusion algorithms solve node embeddings \pan{unify the terminology} $\Mat{H}$ to minimize some potential functions \pan{add some background} defined over hypergraphs.
We proposed a general hypergraph diffusion model \pan{Review hypergraph diffusion instead of proposing a model; Also motivates the applications of this is crucial.} that accumulates potential of individual node embeddings and the joint potential among nodes connected by each hyperedge in a hypergraph $\Set{G}$:
\begin{align} \label{eqn:diffusion}
    \min_{\Mat{H}} \sum_{v \in \Set{V}} f(\Mat{h}_v; \Mat{x}_v) + \sum_{e \in \Set{E}} g(\Mat{H}_e),
\end{align}
where $f: \real^{d} \rightarrow \real$ denotes the node potential function, which defines an independent likelihood of each node representation, $g
: \real^{\lvert e \rvert \times d} \rightarrow \real$ is the hyperedge potential function \pan{different hyperedges may have different sizes}, which specifies a joint constraints on the embeddings of nodes connected by one hyperedge.
\textcolor{red}{High-Order Page Rank}.
\textcolor{red}{High-Order Markov Random Field}.

To optimize Eq.~\eqref{eqn:diffusion}, it is often to use gradient-based methods which we will elaborate in Sec. \ref{sec:model} \pan{Need better motivations, add references and discuss previous approaches; Okay, we should put this into the next section.}. 
Suppose $f(\cdot)$ and $g(\cdot)$ are differentiable, then we denote the gradient of $f(\cdot)$ taking value at $\Mat{h}_v$ as: $\nabla f(\Mat{h}_v; \Mat{x}) = \frac{\partial f(\Mat{z}; \Mat{x})}{\partial \Mat{z}} \lvert_{\Mat{z} = \Mat{h}_v}$,
and since $g(\cdot)$ is a function of a set of nodes, its partial derivative with respect to node $v$ taking value at $\Mat{H}_e$ is defined as: $\nabla_v g(\Mat{H}_e) = \nabla_v g\left(\Mat{h}_{e, 1}, \cdots, \Mat{h}_{e,\lvert e \rvert}\right) = \frac{\partial_v g\left(\Mat{z}_{e, 1}, \cdots, \Mat{z}_{e, \lvert e \rvert}\right)}{\partial \Mat{z}_{e, v}} \Big\lvert_{\Mat{z}_{e,i} = \Mat{h}_{e,i}}$ \pan{I think this notation may have some issues.}.
To reveal more properties of $g(\cdot)$, we list the following formal definitions:

\begin{definition} \label{def:permutation}
Let $\pi: [k] \rightarrow [k]$ be an automorphism, then permutation matrix  is defined as $\Mat{P}_{\pi}$ who has value one at entries $(i, \pi(i)), \forall i \in [k]$ while taking zero at any other positions.
A permutation group $\Grp{P}_k$ \pan{revise to $\Pi[k]$} is defined as a set which collects all of such $\Mat{P}_\pi$.
\end{definition}

\begin{definition} \label{def:permutation_ivariant} (Permutation Invariance)
Let $f: \real^k \rightarrow \real$ be a permutation-invariant function, then $\forall \Mat{P} \in \Grp{P}_k$, $f(\Mat{P} \Mat{x}) = f(\Mat{x})$ for all $\Mat{x} \in \real^k$.
\end{definition}

\begin{definition} \label{def:permutation_equivariant} (Permutation Equivariance)
Let $f: \real^k \rightarrow \real^k$ be a permutation-equivariant function, then $\forall \Mat{P} \in \Grp{P}_k$, $f(\Mat{P} \Mat{x}) = \Mat{P} f(\Mat{x})$ for all $\Mat{x} \in \real^k$.
\end{definition}

We note that potential function $g(\cdot)$ should be permutation-invariant since row permutation of the edge feature matrix results in an equivalent class. \pan{This may be more natural put with g definition together.}
No matter in which order we arrange data inside $\Mat{H}_e$, $g(\cdot)$ should give the identical potential value. 



\begin{itemize}
    \item Attributed hypergraphs: $\gG=(V,E,X)$.  $X\in\mathbb{R}^{|V|\times m}$. $x_v$ denotes the attributes for node $v$. A hyperedge $e\in E$ is a subset of nodes $e=\{v_1^{(e)},...,v_{|e|}^{(e)}\}\subseteq V$ where $|e|$ is the hyperedge size. %(Start from 1-dim case for simplicity).
    
    \item Define node-diffused matrix $H\in\mathbb{R}^{|V|\times m}$ where $h_v$ denotes the row for node $v$. Given $e\in E$, we use notation bar-subscript $\bar{h}_e\in \mathbb{R}^{|e|\times m}$ to denote  concatenation $\oplus_{v\in e} h_v$ whose $i$th block is $h_{v_i^{(e)}}$. We also use the subscript without bar $q_e\in \mathbb{R}^{|e|\times m}$ to denote concatenation of $\oplus_{v\in e} q_{e,v}$ where $q_{e,v}\in \mathbb{R}^{m}$ which is a representation for a hyperedge-node pair.
    
    
    %= (h_{v_1^{(e)}},...,h_{v_|e|^{(e)}})$. %where $z_i = h_{v_i^{(e)}}$ for $i\in[e]$.
    
    \item Node potential: $f_v(\cdot ;x_v)$: $\mathbb{R}^{m} \rightarrow \mathbb{R}.$ %We assume that $f_v = f_{u}$ if the node degree $d_v = d_{u'}$.
    \item hyperedge potential: $g_e(\cdot): \mathbb{R}^{|e|\times m}\times \mathbb{R}$. %We
    %Denote $\bar{z} =(z_1,z_2^{(e)},...,z_|e|^{(e)})$ where $z_{i}^{(e)}$ is the block of the input vector $\bar{z}_e$ associated with node $v_{i}^{(e)}$.
    
    \item In hypergraphs, we often do not have node identities so $f_v=f_u$ if $d_v= d_{u}$. We also assume that $g_e = g_{e'}$ if $|e| = |e'|$ and $g_{e}$ is permutation invariant: $g_e(\bar{h}_e) = g_e(\bar{h}'_e)$ if $\{h_v|v\in e\}=\{h_v'|v\in e\}$. As the information of node degrees and hyperedge sizes are clear, we simply use $f$ and $g$ to uniformly denote node potentials and hyperedge potentials respectively.% by removing the subscripts for simplicity.
    
    
    %where $Z_e\in \mathbb{R}^{|e|\times m}$ and $P$ is a $|e|$-by-$|e|$ permutation matrix. As the information of node degrees and hyperedge sizes are clear, we simply use $f$ and $g$ by removing the subscripts for simplicity.
    %if $\{z_1^{(e)},z_2^{(e)},...,z_{|e|}^{(e)}\}=\{z_1'^{(e)},z_2'^{(e)},...,z_{|e|}'^{(e)}\}$. %In the following, for simplicity, our discussion focus on uniform hypergraphs, though experiments may have non-uniform hypergraphs. So we denote $g_e = g$ for simplicity.
\end{itemize}

% \paragraph{Hypergraph Convolutional Networks}
% Graph neural networks (GNN) are broadly adopted for learning problems on graphs.
% Recent works \cite{feng2019hypergraph, bai2021hypergraph, yadati2019hypergcn, dong2020hnhn, huang2021unignn} have generalized various GNNs for ordinary graphs onto hypergraphs.
% Nevertheless, most of existing hypergraph convolution are based on clique expansion propagation with degree normalization and nonlinear transformation.
% Taking HGNN \cite{feng2019hypergraph} for an example, it has the following node-wise update formula for each layer:
% \begin{align} \label{eqn:hgnn}
%     \Mat{h}_v^{(t+1)} = \sigma\left( \frac{1}{\sqrt{d_v}} \sum_{e: v \in e} \frac{1}{\lvert e \rvert} \sum_{u: u \in e} \frac{\Mat{h}_u^{(t)}}{\sqrt{d_u}} \Mat{\Theta}^{(t)} + \Mat{b}^{(t)} \right),
% \end{align}
% where $\Mat{h}_v^{(t)}$ denotes the features of node $v$ at the $t$-th layer, $d_v$ denotes the degree of node $v$, $\sigma$ is a non-linear activation, and $\Mat{\Theta}^{(t)}, \Mat{b}^{(t)}$ are parameters of linear transformation and bias, respectively.
% We argue that each layer's update (Eq. \ref{eqn:hgnn}) can be regarded as an optimization step of a special case of objective Eq. \ref{eqn:diffusion}.
% We show this by letting $g(\Mat{Z}_e) = \sum_{(v, u) \in e} \lVert \Mat{h}_v^{(e)}/\sqrt{d_v} - \Mat{h}_u^{(e)}/\sqrt{d_u} \rVert_2^2$ and $f(\Mat{h}_v; \Mat{x}_v) = 0$.
% Since $g$ is strongly convex, we can reach optimum by gradient descent. And the gradient step will coincide with Eq. \ref{eqn:hgnn} in form.
% \textcolor{red}{need a derivation and correction later.}
% \textcolor{red}{add AllSet?}

% \paragraph{Nonlinear Hypergraph Diffusion (HyperND)}




==> neurips 2022/section_tex_files/old-003-main.tex <==
\section{Neural Equivariant Diffusion and ED-HNN} \label{sec:model}

% As reviewed in Sec. \ref{sec:prelim}, previous works define closed-form potential functions for optimization.
% However, this is not the case in practical scenarios.
% Real-world data are generated from some high-dimensional complicate distributions which are infeasible to be modeled explicitly.
% To this end, we intend to learn such potential functions from the data in the spirit of modern deep learning.
% Instead of directly fitting an agnostic function, we choose to train a neural network that approximates the gradient-based update of each optimization steps.
We are interested in supervised representation learning on hypergraphs.
In this section, we show by using gradient descent algorithm or Douglas-Rachford splitting algorithm, solving objective Eq. \ref{eqn:diffusion} amounts to iteratively applying hypergraph diffusion operators.
Parameterizing such diffusion operators using neural networks by each step can unfold the optimization algorithm to be a Hypergraph Neural Network (HGNN).  \pan{Inspire our work}
We show that hypergraph diffusion operators are inherently \textit{permutation-equivariant}.
To universally represent them, we propose a standard form of equivariant mapping and follow this form to design our permutation-equivariant neural networks.
By repeating this computational unit, we construct our Equivariant Diffusion-based Hypergraph Neural Network, dubbed ED-HGNN.

\subsection{Emerging Equivariance in Hypergraph Diffusion}
\label{sec:emerge_equivariance}

We begin by discussing hypergraph diffusion objective Eq. \ref{eqn:diffusion} with \textit{continuous} potential functions $f$ and $g$.
Suppose $f$ and $g$ are both differentiable, one straightforward method to reach the optimum is to adopt gradient descent. The node-wise update of each iteration can be formulated as below:
\begin{align} \label{eqn:gd}
    \Mat{h}_v^{(t+1)} \leftarrow \Mat{h}_v^{(t)} - \eta \left(\nabla f(\Mat{h}_v^{(t)}; \Mat{x}_v) + \sum_{e: v\in e} \nabla_{v} g(\Mat{H}_e^{(t)})\right), \quad \text{for}\; v\in V,
\end{align}
where we add superscripts to $\Mat{h}_v$ and $\Mat{H}_e$ to denote the number of the current iteration, $\Mat{h}_v^{(0)} = \Mat{x}_v$ is the initial features, and $\eta$ is known as the learning rate.

However, $f$ and $g$ are not necessarily differentiable (e.g., $g$ penalizes the maximal element), which hinders us to reach the minimum via simple gradient descent.
When $g(\Mat{H}_e)$ is non-differentiable, we solve this problem using Augmented Lagrangian Method (ALM) \pan{reference}.
We first introduce dual variables $\Mat{S}_e \in \real^{\lvert e \rvert \times d}$ and duplicate the hyperedge features $\Mat{H}_e$ into $\Mat{R}_e = \begin{bmatrix} \Mat{r}_{e,1} & \cdots & \Mat{r}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert \times d}$ such that $\Mat{R}_e = \Mat{H}_e$ for every $e \in \Set{E}$.
Then by ALM, our primal problem can be derived as:
\begin{align} \label{eqn:alm}
\pan{\max_{S_e}\min_{R_e,H}}\sum_{v\in \Set{V}} f(\Mat{h}_v; \Mat{x}_v) + \sum_{e\in \Set{E}} g(\Mat{R}_e) +  \frac{\lambda}{2}\sum_{e\in \Set{E}}\lVert \Mat{R}_e - \Mat{H}_e + \Mat{S}_e\ \Vert_2^2 - \frac{\lambda}{2}\sum_{e\in \Set{E}} \lVert \Mat{S}_e \rVert^2.
\end{align}
A common strategy to solve Eq. \ref{eqn:alm} is to minimize $\Mat{H}_e$ and $\Mat{R}_e$ alternatively, which induces a form of Alternating Direction Method of Multipliers (ADMM) as below \pan{reference, node degree was not defined.}:
\begin{align} \label{eqn:admm}
    \Mat{Q}_e^{(t+1)} &\leftarrow  \prox_{g,\frac{1}{\lambda}}(2\Mat{H}_e^{(t)} - \Mat{Q}_e^{(t)}) - \Mat{H}_e^{(t)} + \Mat{Q}_e^{(t)} \\
    \Mat{h}_v^{(t+1)} &\leftarrow  
    \prox_{\frac{1}{f,\lambda d_v}}\left(\frac{1}{d_v}\sum_{e:e\in v}\Mat{q}_{e,v}^{(t)};\pan{x_v}\right),
\end{align}
where we introduce $\Mat{Q}_e = \Mat{S}_e^{(t)} + \Mat{R}_e^{(t+1)} = \begin{bmatrix} \Mat{q}_{e,1} & \cdots & \Mat{q}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert \times d} $ as an intermediate auxiliary variable. The detailed derivation can be found in the \textcolor{red}{Appendix}.

We name gradient $\nabla_{v} g(\cdot)$ and proximal gradient $\prox_{\frac{1}{\lambda} g}(\cdot)$ as \textit{hypergraph diffusion operator} \pan{hyperedge diffusion operator}, since they summarize the collection of node features inside a hyperedge and dispatch the aggregated information to interior nodes individually.
These hypergraph diffusion operators can be intuitively interpreted as a (one-hop) information fusion among nodes connected by some hyperedge.
We reveal one crucial property of hypergraph diffusion operators by the following propostion:
\begin{proposition} \label{prop:equivariant_op}
Hypergraph diffusion operators $\prox_{\frac{1}{\lambda},g}(\Mat{H}_e)$ (\pan{Use the full}) and $\nabla_v g(\Mat{H}_e)$ \pan{I do not think this is an okay notation. We need to consider defining $\nabla g() = [\nabla_v g]_{v\in e}$} are permutation-equivariant operators with respect to node features $\Mat{h}_v$ for any potential function $g(\cdot)$.
\end{proposition}
We provide the proof of Proposition \ref{prop:equivariant_op} in \textcolor{red}{Appendix}. It states that hypergraph diffusion operator $\nabla_v g(\Mat{H}_e)$ and $\prox_{\frac{1}{\lambda},g}(\Mat{H}_e)$ should not only aggregate features regardless of the node order, but should also pass distinctive messages to different nodes.
% This means the operator $\prox_{\frac{1}{\lambda},g}(\Mat{H}_e)$ and $\nabla_v g(\Mat{H}_e)$ are both equivariant set functions.

% After reviewing different forms of hypergraph diffusion, now we assume both node-wise and hyperedge potential functions are unknown.

\subsection{Building Equivariant Hypergraph Diffusion Operator}
\label{sec:build_equivariance}

The choice of $g(\cdot)$ varies from different tasks. For real-world data, it is intractable to handcraft a potential function that precisely express prior distribution over hyperedges.
Recent works \cite{gregor2010learning, liu2019alista, chen2018theoretical, yang2021graph, liu2021elastic} have shown that unrolling and parameterizing each iteration of an optimization problem with neural networks can express more universal objectives and achieve faster convergence.
Motivated by this line of works, we intend to construct a parametric hypergraph diffusion operator that can be learned from data. \pan{Claim how to implement equi hyperedge operator is non-trivial. Previous works are regular. Moreover, standard model, do not need to worry this.}

\pan{Build a bipartite graph by following HNHN and allset. However, we show that invariant sum pooling when message  The sum pooling over hyperedges. When message passes from hyperedges to nodes, we do an additional operation. This techniques have been used in xxx while no hypergraph NN has used this to build eq.  Moreover, our results are not approximation results. The needed dimension is polynomial w.r.t.... }
A handy choice to parameterize hypergraph diffusion operator is neural networks. However, typical architectures, such as Multi-Layer Perceptrons (MLP), would not be the candidate as they do not satisfy the equivariance property.
% Zaheer \etal \cite{zaheer2017deepset} proposed a sum-pooling based architecture that can represent any set functions, 
To achieve order invariance, one may consider DeepSet \cite{zaheer2017deepset} which introduces a sum-pooling scheme to represent arbitrary set functions.
However, it is subject to invariant operators, which are essentially less expressive than equivariant operators.
Segol \etal \cite{segol2019universal} adopted symmetric polynomials as a tool to approximate equivariant set function.
But their construction requires an exponential hidden dimension with respect to set cardinality to represent hyperedge features, which is infeasible to implement.
In this section, we propose a more plausible solution to uniformly approximate equivariant operators capable of representing any type of hypergraph diffusions.


% In previous section, we already know to approximate hypergraph diffusion operator, we need to build a permutation-equivariant set function.
% Even though it is well-known that building a permutation-invariant set function is as simple as raising the input elements into a high-dimension space, summing over the set to obtain a summarized vector, and projecting it to the output space, how to constructing a permutation-equivariant function remains elusive in the literature.

Our follow-up discussion falls on how to represent permutation-equivariant functions in general. To this end, we first provide the following lemma:
\begin{lemma} \label{lem:equivariant_form}
$f: \mathbb{R}^k \rightarrow \mathbb{R}^k$ is an equivariant function if and only if $f(\cdot)$ can be represented as the following form, 
\begin{align}
    f(x_1, x_2, \cdots , x_{k-1}, x_k) = 
    \begin{bmatrix} 
    p(x_1, x_2, \cdots, x_{k-1}, x_k) \\
    p(x_2, x_3, \cdots, x_k, x_1) \\
    \vdots \\
    p(x_N, x_1, \cdots, x_{k-2}, x_{k-1}) \\
    \end{bmatrix}
\end{align}
where $p(\cdot): \mathbb{R}^k \rightarrow \mathbb{R}$ is permutation-invariant with respect to the last $k-1$ elements of inputs. 
\end{lemma}
We give a proof in the \textcolor{red}{Appendix}.
Lemma \ref{lem:equivariant_form} implies that an equivariant function can be element-wisely decomposed into partially invariant mappings, which bridges the construction of invariant and equivariant functions.
Prior works \cite{zaheer2017deepset, wagstaff2019limitations} have guaranteed a finite-dimension and continuous construction of invariant functions.
Using Lemma \ref{lem:equivariant_form}, we are about to compose width-limited and continuous equivariant functions using such invariant functions.
As shown below, we formally specifies a general form that equivariant function must have:
\begin{theorem} \label{thm:equivarnt_form}
$g(\cdot): \mathbb{R}^k \rightarrow \mathbb{R}^k$ is a continuous equivariant function,if and only if $g(\cdot)$ can be represented as the following form, 
\begin{align}
    g(x_1, x_2,\cdots,x_k) =
     \begin{bmatrix} 
    \rho(x_1, \sum_{i=1}^k \phi(x_i)) \\
    \rho(x_2, \sum_{i=1}^k \phi(x_i)) \\
    \vdots\\
    \rho(x_3, \sum_{i=1}^k \phi(x_i)) \\
    \end{bmatrix}
\end{align}
where $\rho: \real^d \rightarrow \real$, $\phi: \real \rightarrow \real^d$ are all continuous functions. \pan{fill in the F dim case.}
\end{theorem}
To prove Theorem \ref{thm:equivarnt_form}, we sequentially adopt Lemma \ref{lem:equivariant_form} and results of invariant set functions in \cite{zaheer2017deepset}.
We defer the detailed proof into \textcolor{red}{Appendix}.
Theorem \ref{thm:equivarnt_form} demonstrates that an equivariant set function can be modeled by a pair-wise relationship between each element and a summarized vector of the whole set.
Note that our proof avoids equivariant polynomials used in \cite{segol2019universal}, thus we can restrict the dimension of the summarized vector to be $d$.
% \textcolor{red}{emphasize the difference between ICLR 2019 and ours. Ours does not need equivariant polynomial, and the dimension can be reduced to d}

\subsection{Unfolding Hypergraph Diffusion as HGNN}
\pan{Suggest to directly merge this section with the previous one.}
We observe that each diffusion step for both differentiable (Eq. \ref{eqn:gd}) and non-differentiable (Eq. \ref{eqn:admm}) potential functions can be unified into the following form:
\begin{align} \label{eqn:neural_diffusion}
    \Mat{h}_v^{(t+1)} = \rho\left(\Mat{h}_v^{(t)}, \sum_{e:v \in e} \phi_v(\Mat{H}_e^{(t)}) \right)
\end{align}
where $\phi: \real^{|e| \times d} \rightarrow \real^{|e| \times d}$ corresponds to gradient operators over hyperedges $\nabla_{v} g(\cdot)$ and $\prox_{\frac{1}{\rho} g}(\cdot)$ that aggregates node features to be hyperedge-level features and dispatches them to each node, $\phi_v(\cdot)$ indexes the value at node $v$, while $\rho: \real^{d} \times \real^{d} \rightarrow \real^{d}$ combines hyperedge features with node features.
The choice of $f(\cdot)$ and $g(\cdot)$ varies from different tasks. For real-world data, handcrafting potential functions that precisely express prior distribution over hyperedges can be intractable.
Recent works \textcolor{red}{Cite LISTA and other unrolling graph papers} have shown that unrolling each iteration in an optimization problem can naturally derive similar structures to multi-layer neural networks, that introduces a group of learnable parameters to express more universal objectives and achieve faster convergence.
Motivated by this line of works, we intend to construct a parametric hypergraph diffusion operator that can be learned from data.
Thereby we parameterize $\rho(\cdot)$ and $\phi(\cdot)$ with some learnable parameters $\Mat{\Theta}$, then Eq. \ref{eqn:neural_diffusion} can be viewed as the $t$-th layer of hypergraph neural networks.
Unfolding $L$ iterations results in an $L$-layer hypergraph neural networks.

\subsection{Implementing Equivariant Diffusion HGNN}

With Theorem \ref{thm:equivarnt_form}, we can borrow neural networks to parameterize $\rho(\cdot)$ and $\phi(\cdot)$ due to the universal approximation theorem.
This implies we can build a neural hypergraph diffusion operator in the following form: 
\begin{align} \label{eqn:neural_nd}
\nabla_v g\left(\Mat{h}^{(e)}_1, \Mat{h}^{(e)}_2,....,\Mat{h}^{(e)}_{|e|}\right) =
 \begin{bmatrix} 
\MLP_2(\Mat{h}^{(e)}_1, \sum_{i=1}^{|e|} \MLP_1(\Mat{h}^{(e)}_i)) \\
\MLP_2(\Mat{h}^{(e)}_2, \sum_{i=1}^{|e|} \MLP_1(\Mat{h}^{(e)}_i)) \\
\vdots\\
\MLP_2(\Mat{h}^{(e)}_{|e|}, \sum_{i=1}^{|e|} \MLP_1(\Mat{h}^{(e)}_i)) \\
\end{bmatrix},
\end{align}
where $\MLP_1: \real^d \rightarrow \real^{|e|d}$ raises the dimension of each node feature, and $\MLP_2: \real^d \times \real^{|e|d} \rightarrow \real^{d'}$ concatenates the feature of the first input and the summarized vector and projects them into the output space.
During the training stage, we iteratively invoke Eq. \ref{eqn:neural_nd} for $L$ times, and optimize MLP parameters by back propagating loss of some downstream tasks.

\subsection{Comparison with Hypergraph Neural Networks}


\begin{proposition} (Informal)
AllSet, HGNN, HyperGNN are permutation-invariant but not permutation-equivariant.
\end{proposition}

\textcolor{red}{discuss difference between other models AllSet, HyperGCN, HGNN.}

\textcolor{red}{another clue is first propose our model, and then discuss existing models, how our model degenerate to their model.}


\textcolor{red}{discuss a variant of our model: two equivariant set functions (allset)}

\textcolor{red}{our model can go deeper to achieve better performance due to diffusion model}

\textbf{Introduce how we implement the equivariant diffusion via neural networks. Overall, we have ED-HNN.}


Suppose we are to approximate $H_v^{(1)}$ where $H^{(0)} = X$, initial $q_e^{(0)}=0$. (put into appendix)
\begin{align*}
        q_e^{(1)} &\leftarrow  \prox_{\frac{1}{\rho},g}(2\bar{h}_e^{(0)}) - \bar{h}_e^{(0)}\\
        h_v^{(1)} &\leftarrow  
        \prox_{\frac{1}{\rho d_v},f}(p_v),\quad \text{where}\; p_v=\frac{1}{d_v}\sum_{e:e\in v}q_{e,v}^{(1)}%\\
        %s_e^{(t+1)} &\leftarrow s_e^{(t)} + r_e^{(t+1)} - \bar{h}_v^{(t+1)}
    \end{align*} 

Or you may choose Gradient-descent (main text):
    \begin{align*}
        h_v^{(t+1)} \leftarrow  h_v^{(t)} - \alpha \left(\nabla f(h_v^{(t)};x_v) + \sum_{e: v\in e} q_{e,v}^{(t)}\right), \quad \text{where}\; q_{e,v}^{(t)} = \nabla g(\bar{h}_e^{(t)}),\; \text{for}\; v\in V.
    \end{align*}
    

% If we consider the update as a hypergraph operator $\psi: h_v^{(t)} \rightarrow h_v^{(t+1)}$, both settings essentially correspond to a mapping function
% %\begin{align*}
% %    h_v^{(t+1)} = \psi_1(h_v^{(t)}, \oplus_{e:v\in e} q_{e,v}^{(t+1)}),\,\text{where}\;q_{e,v}^{(t+1)} = \psi_2(h_v^{(t)}, \oplus_{u\in e/v} h_u^{(t)})  
% %\end{align*}
% \begin{align*}
%     z = \psi(x, \oplus_{e:v\in e}\oplus_{u\in e/v} s_{e,u}),\; \text{where}\; s_{e,u} = h_{u}^{(t)}. %q_{e,v}^{(t+1)}),\,\text{where}\;q_{e,v}^{(t+1)} = \psi_2(h_v^{(t)}, \oplus_{u\in e/v} h_u^{(t)})  
% \end{align*}
% which is invariance with respect to the permutation $\pi_v$ over $\{e|v\in e\}$ and the  permutations $\pi_{v,e}$ over $\{u\in e|u\neq v\}$, i.e., 





\textbf{3. Prove dimension argument: vs ID, vs jump link + ID}

%I use $[\nabla g(\bar{x}_e)]_v$ to denote the gradient w.r.t. $x_v$ of the invariant function $g(\cdot)$ with $|e|$-dim input $\bar{x}_e = (...,x_u,...)_{u\in e}$. 




Our proposal: 
\begin{itemize}
    \item Equivariant operator:
\begin{align*}
    \text{MLP}_3(x_v,x_v^{(0)},\sum_{e:v\in e} \text{MLP}_2(x_v, \sum_{u\in e}\text{MLP}_1(x_u))).
\end{align*}
Theoretically, we just need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2) $\text{MLP}_2: \mathbb{R}^{|e|+1} \rightarrow \mathbb{R}$; (3) $\text{MLP}_3: \mathbb{R}^3 \rightarrow \mathbb{R}$



\item Jump-link + Invariant operator: 
\begin{align*}
    \text{MLP}_3(x_v, \sum_{e:v\in e} \text{MLP}_2(\sum_{u\in e}\text{MLP}_1(x_u))).
\end{align*}
Theoretically, we need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2)
$\text{MLP}_2: \mathbb{R}^{|e|} \rightarrow \mathbb{R}^{(|e|-1)*d_v+1}$; (3) $\text{MLP}_3: \mathbb{R}^{(|e|-1)*d+1} \rightarrow \mathbb{R}$.

% \item Small invariant operator (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% \begin{align*}
%     \text{MLP}_2(\sum_{e:v\in e} \sum_{u\in e}\text{MLP}_1(x_u)).
% \end{align*}
% We know this cannot give universal approximation. But the parameter selection should be at least the same as equivariant operator.


\item Big invariant operator: 
\begin{align*}
    \text{MLP}_3(\sum_{e:v\in e} \text{MLP}_2(\sum_{u\in e}\text{MLP}_1(x_u))).
\end{align*}
We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

\item Attention-based (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
\begin{align*}
    Attention_2(\text{MLP}_2(Attention_1(\{\text{MLP}_1(x_u)|u\in e\}))|e:v\in e).
\end{align*}
We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

\end{itemize}

Empirical comparison: We study the dependence on $k$ from 20-200. We should consider alternative projection and subgradient descent. We should consider the following models with degree and node feature fixed.

%We also add the following three models.

% \begin{itemize}
% \item Small equivariant operator (In sec 3, we do not need to discuss this, which is just for fair comparison):
% \begin{align*}
%     \sum_{e:v\in e} \text{MLP}_2(x_v, \sum_{u\in e}\text{MLP}_1(x_u)).
% \end{align*}

% \item Small invariant operator (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% \begin{align*}
%     \text{MLP}_2(\sum_{e:v\in e} \sum_{u\in e}\text{MLP}_1(x_u)).
% \end{align*}

%\end{itemize}

\begin{itemize}
    \item Equivariant operator:
\begin{align*}
    \text{Linear}_3(x_v,\log d_v,\text{mean}_{e:v\in e} \text{MLP}_2(x_v, \log |e|, \text{mean}_{u\in e}\text{MLP}_1(x_u,\log d_v))).
\end{align*}
%Theoretically, we just need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2) $\text{MLP}_2: \mathbb{R}^{|e|+1} \rightarrow \mathbb{R}$; (3) $\text{MLP}_3: \mathbb{R} \rightarrow \mathbb{R}$



\item Jump-link + Invariant operator: 
\begin{align*}
    \text{Linear}_3(x_v, \log d_v,  \text{mean}_{e:v\in e} \text{MLP}_2(\log |e|,\text{mean}_{u\in e}\text{MLP}_1(x_u,\log d_v))).
\end{align*}
%Theoretically, we need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2)
%$\text{MLP}_2: \mathbb{R}^{|e|} \rightarrow \mathbb{R}^{(|e|-1)*d+1}$; (3) $\text{MLP}_3: \mathbb{R}^{(|e|-1)*d+1} \rightarrow \mathbb{R}$.

% \item Small invariant operator (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% \begin{align*}
%     \text{MLP}_2(\sum_{e:v\in e} \sum_{u\in e}\text{MLP}_1(x_u)).
% \end{align*}
% We know this cannot give universal approximation. But the parameter selection should be at least the same as equivariant operator.


\item Big invariant operator: 
\begin{align*}
    \text{Linear}_3(\log d_v,\text{mean}_{e:v\in e} \text{MLP}_2(\log |e|, \text{mean}_{u\in e}\text{MLP}_1(x_u,\log d_u))).
\end{align*}
We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

\item Attention-based (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
\begin{align*}
    Attention_2(\log d_v,\text{MLP}_2(Attention_1(\log |e|,\{\text{MLP}_1(x_u)|u\in e\}))|e:v\in e).
\end{align*}
We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

\end{itemize}



\begin{itemize}
    \item Equivariant operator: $\text{MLP}_1: 2\times 200, 200\times k$, $\text{MLP}_2: k+2\times 200,  200\times k+2$, $\text{Linear}_3: k+2\times 1$.
    
    \item Fair equivariant operator: $\text{MLP}_1: 1\times 200, 200\times k$, $\text{MLP}_2: k+2\times 200, 200\times 200$. $\text{Linear}_3: 200\times 1$.
    
    \item Jump-link + Invariant operator: $\text{MLP}_1: 1\times 200, 200\times k$,
    $\text{MLP}_2: k+1\times 200, 200\times 200$
    $\text{Linear}_3: 200+2\times 1$.

    %\item Small Invariant operator: $\text{MLP}_1: 1\times 200, 200\times k$,
    %$\text{MLP}_2: k\times 200, 200\times 1$.

    \item Big Invariant operator: $\text{MLP}_1: 1\times 200, 200\times k$,
    $\text{MLP}_2: k+1\times 200, 200\times 200$,
    $\text{Linear}_3: 201\times 1$.   

    \item Attention: $\text{MLP}_1: 1\times 200, 200\times k$,
    $\text{Attention}_1: {k+1}\times {k+1}$,
    $\text{MLP}_2: {k+1}\times 200, 200\times 200$,
    $\text{Attention}_2: 201\times 1$.

\end{itemize}

==> neurips 2022/section_tex_files/old-005-exp.tex <==

\begin{table}[t]
\caption{Test time $10^{-2}$ sec, train time in $10^{-1}$ sec. FLOPs in MiB.}
\label{tab:real_data}
\centering
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{cccccc|cc}
\toprule
& Cora & Citeseer & Pubmed & Cora-CA & DBLP-CA & \# Params & Train Time \\
\midrule
HGNN \cite{huang2021unignn} & 79.39 $\pm$ 1.36 & 72.45 $\pm$ 1.16 & 86.44 $\pm$ 0.44 & 82.64 $\pm$ 1.65 & 91.03 $\pm$ 0.20 & 21,963 & 0.24 $\pm$ 0.51 \\
HCHA \cite{bai2021hypergraph} & 79.14 $\pm$ 1.02 & 72.42 $\pm$ 1.42 & 86.41 $\pm$ 0.36 & 82.55 $\pm$ 0.97 & 90.92 $\pm$ 0.22 & 57,355 & 0.24 ± 0.01 \\
HNHN \cite{dong2020hnhn} & 76.36 $\pm$ 1.92 & 72.64 $\pm$ 1.57 & 86.90 $\pm$ 0.30 & 77.19 $\pm$ 1.49 & 86.78 $\pm$ 0.29 & 28,683 & 0.30 $\pm$ 0.56 \\
HyperGCN \cite{yadati2019hypergcn} & 78.45 $\pm$ 1.26 & 71.28 $\pm$ 0.82 & 82.84 $\pm$ 8.67 & 79.48 $\pm$ 2.08 & 89.38 $\pm$ 0.25 \\
HyperSAGE \cite{arya2020hypersage} & & & \\
UniGCNII \cite{huang2021unignn} & 78.81 $\pm$ 1.05 & 73.05 $\pm$ 2.21 & 88.25 $\pm$ 0.40 & 83.60 $\pm$ 1.14 & 91.69 $\pm$ 0.19 & 2,154,507 & 4.36 $\pm$ 1.18 \\
AllDeepSets \cite{chien2021you} & 76.88 $\pm$ 1.80 & 70.83 $\pm$ 1.63 & 88.75 $\pm$ 0.33 & 81.97 $\pm$ 1.50 & 91.27 $\pm$ 0.27 & 850,643 & 1.23 $\pm$ 1.09\\
AllSetTransformer \cite{chien2021you} & 78.58 $\pm$ 1.47 & 73.08 $\pm$ 1.20 & 88.72 $\pm$ 0.37 & 83.63 $\pm$ 1.47 & 91.53 $\pm$ 0.23 & 1,166,859 & 1.64 $\pm$ 1.63 \\
\midrule
\proj & 80.31 $\pm$ 1.35 & 73.70 $\pm$ 1.38 & 89.03 $\pm$ 0.53 & 83.97 $\pm$ 1.55 & 91.90 $\pm$ 0.19 & 1,111,563 & 1.71 $\pm$ 1.13 \\
% \projtwo & 77.47 $\pm$ 1.62 & 72.65 $\pm$ 1.56 & 88.86 $\pm$ 0.40 & 82.17 $\pm$ 1.68 & 91.62 $\pm$ 0.29 \\
% ED-HNN Attn. & 78.63 $\pm$ 1.55 & 71.21 $\pm$ 1.37 & 88.74 $\pm$ 0.37 & 82.33 $\pm$ 1.74 & 91.84 $\pm$ 0.25 \\
\bottomrule
& Congress & Senate & Walmart & House & Avg. Rank & FLOPs & Test Time \\
\midrule
HGNN \cite{huang2021unignn} & 91.26 $\pm$ 1.15 & 48.59 $\pm$ 4.52 & 62.00 $\pm$ 0.24 & 61.39 $\pm$ 2.96  & & \\
HCHA \cite{bai2021hypergraph} & & & 62.35 $\pm$ 0.26 & 61.36 $\pm$ 2.53 & &  \\
HNHN \cite{dong2020hnhn} & & & 47.18 $\pm$ 0.35 & 67.80 $\pm$ 2.59 & & &  0.76 $\pm$ 0.05\\
HyperGCN \cite{yadati2019hypergcn} & & & 44.74 $\pm$ 2.81 & 48.32 $\pm$ 2.93 & & \\
HyperSAGE \cite{arya2020hypersage} & & & \\
UniGCNII \cite{huang2021unignn} & 94.81 $\pm$ 0.81 & 49.30 $\pm$ 4.25 & 54.45 $\pm$ 0.37 & 67.25 $\pm$ 2.57 & & 500,459,520 & 21.22 $\pm$ 0.13\\
AllDeepSets \cite{chien2021you} & 91.80 $\pm$ 1.53 & 48.17 $\pm$ 5.67 & 64.55 $\pm$ 0.33 & 67.82 $\pm$ 2.40  & & 74,577,535,272 &  5.35 $\pm$ 0.33 \\
AllSetTransformer \cite{chien2021you} & 92.16 $\pm$ 1.05 & 51.83 $\pm$ 5.22 & 65.46 $\pm$ 0.25 & 69.33 $\pm$ 2.20 & & 103,114,858,724 & 6.06 $\pm$ 0.67 \\
\midrule
\proj & 95.00 $\pm$ 0.99 & 64.79 $\pm$ 5.14 & 66.91 $\pm$ 0.41 & 72.45 $\pm$ 2.28 & & 322,755,380,680 & 5.87 $\pm$ 0.36 \\
% \projtwo & 95.19 $\pm$ 1.34 & 65.01 $\pm$ 6.17 & 65.24 $\pm$ 0.45 & 70.95 $\pm$ 1.97 \\
% ED-HNN Attn. & 95.24 $\pm$ 1.48 & 65.32 $\pm$ 6.72 & 67.06 $\pm$ 0.53 & 71.10 $\pm$ 2.65 \\
\bottomrule
\end{tabular}}
\end{table}


\section{Experiments} \label{sec:exp}

\subsection{Results on Benchmarking Datasets}

\paragraph{Experiment Setting.}
In this subsection, we validate the effectiveness of \proj on nine real-world benchmarking hypergraphs. We focus on semi-supervised node classification. %in the transductive setting.
We report performance on seven available datasets from the existing hypergraph neural network literature, including co-citation networks (Cora, Citeseer, Pubmed), co-authorship networks (Cora-CA, DBLP-CA) \cite{yadati2019hypergcn}, Walmart \cite{amburg2020clustering}, and House \cite{chodrow2021hypergraph}.
We also involve two new datasets Congress and Senate \textcolor{red}{cite xx} to enrich our experiments.
Since there are no original node features in Walmart, House, Congress and Senate, we follow the method of \cite{chien2021you} to generate node features from label-centered Gaussian distribution \cite{deshpande2018contextual}.
As we show in Table \textcolor{red}{xxx}, these datasets already cover sufficiently diverse hypergraphs in terms of scale, structure, and homo-/heterophily.
We compare our method with top-performing models on the benchmark, including HGNN \cite{feng2019hypergraph}, HCHA \cite{bai2021hypergraph}, HNHN \cite{dong2020hnhn}, HyperGCN \cite{yadati2019hypergcn}, HyperSAGE \cite{arya2020hypersage}, UniGCNII \cite{huang2021unignn}, AllDeepSets \cite{chien2021you}, and AllSetTransformer \cite{chien2021you}.
All the hyper-parameters for baselines follow from \cite{chien2021you} and we fix learning rate, weight decay and other training recipes same with the baselines.
Other model specific hyper-parameters are obtained by grid search (see Appendix \ref{sec:hparam}).
We randomly split the data into training/validation/test sample using 50\%/25\%/25\% splitting percentage following \cite{chien2021you}.
We choose prediction accuracy as the evaluation metric.
We run each model for ten times with different training/validation splits to obtain the standard deviation.

\paragraph{Performance Analysis}
We report our numerical results in Table \ref{tab:real_data}.
Our \proj achieves the state-of-the-art performance among all the compared models on all the tested datasets.
We observe that the top-performing baseline models are AllSetTransformer, AllDeepSets ,and UniGCNII, where the former two represent HNNs using  multiset functions, while the later one improves traditional HNNs by initial and jumping links.
One can see these models accidentally resonate with our design principle.
However, their performance has large variation across different datasets.
For example, UniGCNII attains promising performance on citation networks, however, has subpar results on Walmart dataset.
In contrast, our model achieves stable and consistent superior results, surpassing AllSets models by up to 12.9\% on Senate and UniGCNII by up to 12.5\% on Walmart.
We owe our empirical significance to the theoretical design of exact equivariant function representation.
While adopting set function, AllSets model lack of equivariance.
UniGCNII injects equivariance via jump link, but it is not so expressive as our \proj.


\paragraph{Efficiency Analysis}

\begin{table}[]
\caption{Caption}
\label{tab:syn_node_data}
\centering
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{} & \multicolumn{2}{c}{Homophily} & \multicolumn{3}{c}{Heterophily} \\
& $\alpha = 0.1$ & $\alpha = 0.15$ & $\alpha = 0.2$ & $\alpha = 0.3$ & $\alpha = 0.5$ \\
\midrule
HGNN \cite{huang2021unignn} & 99.86 $\pm$ 0.05 & 90.42 $\pm$ 1.14 & 66.60 $\pm$ 1.60 & 57.90 $\pm$ 1.43 & 48.68 $\pm$ 1.21 \\
HGNN + JumpLink \cite{huang2021unignn} & 99.29 $\pm$ 0.19 & 92.61 $\pm$ 0.97 & 79.59 $\pm$ 2.32 & 64.39 $\pm$ 1.55 & 51.14 $\pm$ 2.05 \\
AllDeepSets \cite{chien2021you} & 99.86 $\pm$ 0.07 & 99.13 $\pm$ 0.31 & 92.39 $\pm$ 1.68 & 80.12 $\pm$ 2.31 & 52.14 $\pm$ 2.88 \\
AllDeepSets + JumpLink \cite{huang2021unignn} & 99.95 $\pm$ 0.07 & 99.08 $\pm$ 0.24 & 93.52 $\pm$ 1.31 & 83.45 $\pm$ 2.64 & 52.21 $\pm$ 2.36 \\
AllSetTransformer \cite{chien2021you} & 98.60 $\pm$ 0.48 & 95.89 $\pm$ 0.90 & 88.38 $\pm$ 1.81 & 83.34 $\pm$ 1.33 & 50.15 $\pm$ 1.73 \\
\midrule
\proj (ours)  & 99.92 $\pm$ 0.08 & 99.68 $\pm$ 0.13 & 95.37 $\pm$ 1.23 & 90.35 $\pm$ 0.83 & 54.31 $\pm$ 2.40 \\
\bottomrule
\end{tabular}}
\end{table}

\subsection{Results on Synthetic Heterophilic Hypergraph Dataset}

\paragraph{Experiment Setting.} As we discussed in \ref{sec:dis_heterophily}, \proj takes advantage in learning on heterophilic hypergraph data.
In this section, we verify our argument by synthetic datasets with controlled heterophily.
We generate hypergraph by contextual hypergraph stochastic block model \cite{deshpande2018contextual}.
Specifically, we first draw two classes of nodes of the same number, then we build hyperedges by randomly sampling nodes from two classes with respect to a ratio $\alpha$.
This ratio determines how many nodes with the same label will be connected by a hyperedge, which controls the homo-/heterophily of the synthetic hypergraph.
Afterwards, we generate node features using label-dependent Gaussian noise.
We test both homophilic ($\alpha=0.1/0.15$ or CE homophily$\ge 0.7$) and heterophilic ($\alpha=0.2/0.3/0.5$ or CE homophily $\le 0.7$) cases.
We compare \proj with HGNN \cite{feng2019hypergraph} and AllSets \cite{chien2021you} as well as their variants with jump link.

\paragraph{Results.} Our experimental results are listed in Table \ref{tab:syn_node_data}.
On homophilic datasets, all the models can achieve good results, especially for $\alpha=0.1$.
However, once $\alpha$ surpasses 0.2, i.e., entering the heterophilic regime, all models except for \proj have a drastic performance drop.
Even for $\alpha = 0.3$ case, where half of neighboring nodes are labelled differently, our \proj can achieve 90.35\% prediction accuracy.
Another interesting finding is that $\alpha = 0.5$ reaches the maximum tolerance to heterophily of all presented works.

\subsection{Benefits in Deepening Hypergraph Neural Networks.}

We also demonstrate that by using diffusion models and parameter tying, \proj can scale up and benefit from deeper architectures which other HNNs fail to achieve.
Figure \ref{fig:expr_depth} illustrates the performance of different models versus the number of network layers.
We compare with vanilla HGNN \cite{feng2019hypergraph}, AllSets models \cite{chien2021you}, and UniGCNII \cite{huang2021unignn}, which is known to be effective counteracting oversmoothness.
Our experimental results reveal that AllSets models have worst scalability. Once the depth grows larger than 2, their performance declines rapidly.
HGNN and UniGCNII working through more lightweight mechanism have better tolerance to depth, however, either of them can benefit from deepening.
On the contrary, \proj successfully leverages deeper architecture to achieve higher accuracy.
For example, adding more layers boost \proj by \textasciitilde1\% in accuracy on Pubmed and House, while elevating \proj from 58.01\% to 64.79\% on Senate dataset.

\subsection{Expressiveness Justification on Synthetic Diffusion Dataset}

We generate semi-synthetic diffusion data using the Senate hypergraph~\cite{chodrow2021hypergraph} and synthetic node features. The data we generate consists of 1,000 pairs $(\Mat{H}^{(0)}, \Mat{H}^{(1)})$. The initial node features $\Mat{H}^{(0)}$ are sampled from Gaussian distributions. To obtain $\Mat{H}^{(1)}$ we apply the gradient step in Eq.~\ref{eqn:gd}. We fix the node potential $f(\Mat{h}_v; \Mat{x}_v) = (\Mat{h}_v - \Mat{x}_v)^2$ and consider 3 different edge potentials in Example~\ref{exp:potential} with varying complexities: a) CE, b) TV ($p$=2) and c) LEC. We provide more details in the appendix.
%with $y_i=2/|e|$ if $i \le |e|/2$ and $-2/|e|$ otherwise (take $|e|-1$ if $|e|$ is odd). 

\begin{figure}
\centering
\includegraphics[width=1.\linewidth]{images/depth.pdf}
\caption{Deepening experiment}
\label{fig:expr_depth}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=1.\linewidth]{images/dim_reduction.pdf}
\caption{Dimension reduction experiment}
\label{fig:expr_width}
\end{figure}

% \begin{itemize}
% \item Equivariant operator:
% \begin{align*}
%     (x_v, x_v^{(0)}, \log d_v,\text{mean}(\text{MLP}_2(x_v, \log |e|, \text{mean}(\text{MLP}_1(x_u))))).
% \end{align*}

% \begin{align*}
% h_e^{(t)} = \text{mean}_u(\text{MLP}_1(h_u^{(t-1)}))\\
% m_{v\leftarrow e}^{(t)}=(h_v^{(t-1)}, \log |e|, h_e^{(t)}) \\
% h_v'^{(t)}= \text{mean}_{e:v\in e}\text{MLP}_2 (m_{v\leftarrow e}^{(t)})\\
% h_v^{(t)}= 
% (h_v^{(t-1)},x_v^{(0)}, \log d_v,h_v'^{(t)})
% \end{align*}

% \item double equi. 
% \begin{align*}
% h_e^{(t)} = \text{mean}_u(\text{MLP}_1(m_{u\rightarrow e}^{(t-1)}))\\
% m_{v\leftarrow e}^{(t)}=(h_v^{(t-1)}, \log |e|, h_e^{(t)}) \\
% h_v^{(t)}= \text{mean}_{e:v\in e}\text{MLP}_2 (m_{v\leftarrow e}^{(t)})\\
% m_{v\rightarrow e}^{(t)}= 
% (h_v^{(t-1)},h_e^{(t)}, x_v^{(0)}, \log d_v, h_v^{(t)})
% \end{align*}

% \end{itemize}

1. Synthetic data on one-step hypergraph diffusion to demonstrate the theory. Study the dependence on the model size. 

2. Synthetic data on node classification across different heterophilic levels of hypergraphs generated by stochastic block models. 

3. Real datasets experiments. 

==> neurips 2022/section_tex_files/old-model.tex <==
\section{Neural Equivariant Diffusion and ED-HNN}
\textbf{0. Gradient for continuously differentiable; Proximal gradient for continuous functions. Prove equivariance.}  

\begin{itemize}
    \item Gradient-descent:
    \begin{align*}
        h_v^{(t+1)} \leftarrow  h_v^{(t)} - \alpha \left(\nabla f(h_v^{(t)};x_v) + \sum_{e: v\in e} \nabla_v g(\bar{h}_e^{(t)})\right), \quad \text{for}\; v\in V.
    \end{align*}
 
    The third term implies the equivariance of $\bar{h}_e^{(t)}\rightarrow \nabla g(\bar{h}_e)$. The first two terms imply jump-link and injection of initial $x_v$.
       
       
    \item For when $f$ and $g$ are  non-smooth, ADMM: Associate each hyperedge with $r_e$ and $s_e$.
    \begin{align*}
        \sum_{v\in V} f(h_v; x_v) + \sum_{e\in E} g(r_e) +  \frac{\rho}{2}\sum_{e\in E}\|r_e - \bar{h}_e+s_e\|^2 
        - \frac{\rho}{2}\sum_{e\in E} \|s_e\|^2
    \end{align*}   
    
    \begin{align*}
        r_e^{(t+1)} &\leftarrow  \text{prox}_{\frac{1}{\rho},g}(\bar{h}_e^{(t)}-s_e^{(t)})\triangleq\arg\min_{z_e} \frac{\rho}{2}\|z_e-\bar{h}_e^{(t)} + s_e^{(t)}\|^2 + g(z_e)\\
        h_v^{(t+1)} &\leftarrow  \arg\min_{z_v} \frac{\rho}{2}\sum_{e:v\in e}\|z_v- s_{e,v}^{(t)} - r_{e,v}^{(t+1)}\|^2 + f(z_v;x_v) \\
        &= \text{prox}_{\frac{1}{\rho d_v},f}(p_v)\triangleq \arg\min_{z_v} \frac{\rho d_v}{2}\|z_v- p_v\|^2 + f(z_v;x_v),\quad \text{where}\; p_v=\frac{1}{d_v}\sum_{e:e\in v}(s_{e,v}^{(t)} + r_{e,v}^{(t+1)})\\
        s_e^{(t+1)} &\leftarrow s_e^{(t)} + r_e^{(t+1)} - \bar{h}_v^{(t+1)}
    \end{align*}   
    If we set $q_e^{(t+1)} = s_e^{(t)} + r_e^{(t+1)}$,
    \begin{align*}
        q_e^{(t+1)} &\leftarrow  \text{prox}_{\frac{1}{\rho},g}(2\bar{h}_e^{(t)}-q_e^{(t)}) + q_e^{(t)} - \bar{h}_e^{(t)}\\
        h_v^{(t+1)} &\leftarrow  
         \text{prox}_{\frac{1}{\rho d_v},f}(p_v),\quad \text{where}\; p_v=\frac{1}{d_v}\sum_{e:e\in v}q_{e,v}^{(t)}%\\
        %s_e^{(t+1)} &\leftarrow s_e^{(t)} + r_e^{(t+1)} - \bar{h}_v^{(t+1)}
    \end{align*}   

Currently, with only edge equivar.
    \begin{align*}
        q_e^{(t+1)} &\leftarrow  \text{prox}_{\frac{1}{\rho},g}(\bar{h}_e^{(t)}) \\
        h_v^{(t+1)} &\leftarrow  
         \text{prox}_{\frac{1}{\rho d_v},f}(p_v),\quad \text{where}\; p_v=\frac{1}{d_v}\sum_{e:e\in v}q_{e,v}^{(t)}%\\
        %s_e^{(t+1)} &\leftarrow s_e^{(t)} + r_e^{(t+1)} - \bar{h}_v^{(t+1)}
    \end{align*} 

% If we set $\phi_e^{(t+1)} = 2\bar{h}_e^{(t)}-q_e^{(t)}$,
%     \begin{align*}
%         q_e^{(t+1)} &\leftarrow  \text{prox}_{\frac{1}{\rho},g}(\phi_e^{(t)}) + q_e^{(t)} - \bar{h}_e^{(t)}\\
%         h_v^{(t+1)} &\leftarrow  
%          \text{prox}_{\frac{1}{\rho d_v},f}(p_v),\quad \text{where}\; p_v=\frac{1}{d_v}\sum_{e:e\in v}q_{e,v}^{(t)}%\\
%         %s_e^{(t+1)} &\leftarrow s_e^{(t)} + r_e^{(t+1)} - \bar{h}_v^{(t+1)}
%     \end{align*}         
    

\textcolor{blue}{I found the current pipeline cannot perfectly implement the above procedure due to $q_e^{(t)}$. The third term means that we need equivariance also on the node side. The $h_v^{(t)}$ needs jump link and $x_v$.}

   %The third term implies the jump link of $q_e^{(t)}$ and equivariance of $\bar{h}_e^{(t)}\rightarrow \nabla g(\bar{h}_e)$. The first two terms imply jump-link and injection of initial $x_v$.
    
\end{itemize}


\textbf{1. Inspired by xxx, we prove equivariant diffusion form.} 

The equivariance theorem in the previous draft and discussion. 

\textbf{2. Introduce how we implement the equivariant diffusion via neural networks. Overall, we have ED-HNN.}


Suppose we are to approximate $H_v^{(1)}$ where $H^{(0)} = X$, initial $q_e^{(0)}=0$. (put into appendix)
\begin{align*}
        q_e^{(1)} &\leftarrow  \text{prox}_{\frac{1}{\rho},g}(2\bar{h}_e^{(0)}) - \bar{h}_e^{(0)}\\
        h_v^{(1)} &\leftarrow  
         \text{prox}_{\frac{1}{\rho d_v},f}(p_v),\quad \text{where}\; p_v=\frac{1}{d_v}\sum_{e:e\in v}q_{e,v}^{(1)}%\\
        %s_e^{(t+1)} &\leftarrow s_e^{(t)} + r_e^{(t+1)} - \bar{h}_v^{(t+1)}
    \end{align*} 

Or you may choose Gradient-descent (main text):
    \begin{align*}
        h_v^{(t+1)} \leftarrow  h_v^{(t)} - \alpha \left(\nabla f(h_v^{(t)};x_v) + \sum_{e: v\in e} q_{e,v}^{(t)}\right), \quad \text{where}\; q_{e,v}^{(t)} = \nabla g(\bar{h}_e^{(t)}),\; \text{for}\; v\in V.
    \end{align*}
    

% If we consider the update as a hypergraph operator $\psi: h_v^{(t)} \rightarrow h_v^{(t+1)}$, both settings essentially correspond to a mapping function
% %\begin{align*}
% %    h_v^{(t+1)} = \psi_1(h_v^{(t)}, \oplus_{e:v\in e} q_{e,v}^{(t+1)}),\,\text{where}\;q_{e,v}^{(t+1)} = \psi_2(h_v^{(t)}, \oplus_{u\in e/v} h_u^{(t)})  
% %\end{align*}
% \begin{align*}
%     z = \psi(x, \oplus_{e:v\in e}\oplus_{u\in e/v} s_{e,u}),\; \text{where}\; s_{e,u} = h_{u}^{(t)}. %q_{e,v}^{(t+1)}),\,\text{where}\;q_{e,v}^{(t+1)} = \psi_2(h_v^{(t)}, \oplus_{u\in e/v} h_u^{(t)})  
% \end{align*}
% which is invariance with respect to the permutation $\pi_v$ over $\{e|v\in e\}$ and the  permutations $\pi_{v,e}$ over $\{u\in e|u\neq v\}$, i.e., 


\textbf{3. Prove dimension argument: vs ID, vs jump link + ID}

%I use $[\nabla g(\bar{x}_e)]_v$ to denote the gradient w.r.t. $x_v$ of the invariant function $g(\cdot)$ with $|e|$-dim input $\bar{x}_e = (...,x_u,...)_{u\in e}$. 




Our proposal: 
\begin{itemize}
    \item Equivariant operator:
\begin{align*}
    \text{MLP}_3(x_v,x_v^{(0)},\sum_{e:v\in e} \text{MLP}_2(x_v, \sum_{u\in e}\text{MLP}_1(x_u))).
\end{align*}
Theoretically, we just need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2) $\text{MLP}_2: \mathbb{R}^{|e|+1} \rightarrow \mathbb{R}$; (3) $\text{MLP}_3: \mathbb{R}^3 \rightarrow \mathbb{R}$



\item Jump-link + Invariant operator: 
\begin{align*}
    \text{MLP}_3(x_v, \sum_{e:v\in e} \text{MLP}_2(\sum_{u\in e}\text{MLP}_1(x_u))).
\end{align*}
Theoretically, we need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2)
$\text{MLP}_2: \mathbb{R}^{|e|} \rightarrow \mathbb{R}^{(|e|-1)*d_v+1}$; (3) $\text{MLP}_3: \mathbb{R}^{(|e|-1)*d+1} \rightarrow \mathbb{R}$.

% \item Small invariant operator (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% \begin{align*}
%     \text{MLP}_2(\sum_{e:v\in e} \sum_{u\in e}\text{MLP}_1(x_u)).
% \end{align*}
% We know this cannot give universal approximation. But the parameter selection should be at least the same as equivariant operator.


\item Big invariant operator: 
\begin{align*}
    \text{MLP}_3(\sum_{e:v\in e} \text{MLP}_2(\sum_{u\in e}\text{MLP}_1(x_u))).
\end{align*}
We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

\item Attention-based (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
\begin{align*}
    Attention_2(\text{MLP}_2(Attention_1(\{\text{MLP}_1(x_u)|u\in e\}))|e:v\in e).
\end{align*}
We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

\end{itemize}

Empirical comparison: We study the dependence on $k$ from 20-200. We should consider alternative projection and subgradient descent. We should consider the following models with degree and node feature fixed.

%We also add the following three models.

% \begin{itemize}
% \item Small equivariant operator (In sec 3, we do not need to discuss this, which is just for fair comparison):
% \begin{align*}
%     \sum_{e:v\in e} \text{MLP}_2(x_v, \sum_{u\in e}\text{MLP}_1(x_u)).
% \end{align*}

% \item Small invariant operator (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% \begin{align*}
%     \text{MLP}_2(\sum_{e:v\in e} \sum_{u\in e}\text{MLP}_1(x_u)).
% \end{align*}

%\end{itemize}

\begin{itemize}
    \item Equivariant operator:
\begin{align*}
    \text{Linear}_3(x_v,\log d_v,\text{mean}_{e:v\in e} \text{MLP}_2(x_v, \log |e|, \text{mean}_{u\in e}\text{MLP}_1(x_u,\log d_v))).
\end{align*}
%Theoretically, we just need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2) $\text{MLP}_2: \mathbb{R}^{|e|+1} \rightarrow \mathbb{R}$; (3) $\text{MLP}_3: \mathbb{R} \rightarrow \mathbb{R}$



\item Jump-link + Invariant operator: 
\begin{align*}
    \text{Linear}_3(x_v, \log d_v,  \text{mean}_{e:v\in e} \text{MLP}_2(\log |e|,\text{mean}_{u\in e}\text{MLP}_1(x_u,\log d_v))).
\end{align*}
%Theoretically, we need:(1) $\text{MLP}_1: \mathbb{R} \rightarrow \mathbb{R}^{|e|}$; (2)
%$\text{MLP}_2: \mathbb{R}^{|e|} \rightarrow \mathbb{R}^{(|e|-1)*d+1}$; (3) $\text{MLP}_3: \mathbb{R}^{(|e|-1)*d+1} \rightarrow \mathbb{R}$.

% \item Small invariant operator (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
% \begin{align*}
%     \text{MLP}_2(\sum_{e:v\in e} \sum_{u\in e}\text{MLP}_1(x_u)).
% \end{align*}
% We know this cannot give universal approximation. But the parameter selection should be at least the same as equivariant operator.


\item Big invariant operator: 
\begin{align*}
    \text{Linear}_3(\log d_v,\text{mean}_{e:v\in e} \text{MLP}_2(\log |e|, \text{mean}_{u\in e}\text{MLP}_1(x_u,\log d_u))).
\end{align*}
We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

\item Attention-based (In sec 3, we do not need to discuss this, which is just for empirical comparison): 
\begin{align*}
    Attention_2(\log d_v,\text{MLP}_2(Attention_1(\log |e|,\{\text{MLP}_1(x_u)|u\in e\}))|e:v\in e).
\end{align*}
We know this cannot give universal approximation. But the parameter selection should be at least the same as Jump-link + Invariant operator.

\end{itemize}



\begin{itemize}
    \item Equivariant operator: $\text{MLP}_1: 2\times 200, 200\times k$, $\text{MLP}_2: k+2\times 200,  200\times k+2$, $\text{Linear}_3: k+2\times 1$.
    
    \item Fair equivariant operator: $\text{MLP}_1: 1\times 200, 200\times k$, $\text{MLP}_2: k+2\times 200, 200\times 200$. $\text{Linear}_3: 200\times 1$.
    
    \item Jump-link + Invariant operator: $\text{MLP}_1: 1\times 200, 200\times k$,
    $\text{MLP}_2: k+1\times 200, 200\times 200$
    $\text{Linear}_3: 200+2\times 1$.

    %\item Small Invariant operator: $\text{MLP}_1: 1\times 200, 200\times k$,
    %$\text{MLP}_2: k\times 200, 200\times 1$.

    \item Big Invariant operator: $\text{MLP}_1: 1\times 200, 200\times k$,
    $\text{MLP}_2: k+1\times 200, 200\times 200$,
    $\text{Linear}_3: 201\times 1$.   

    \item Attention: $\text{MLP}_1: 1\times 200, 200\times k$,
    $\text{Attention}_1: {k+1}\times {k+1}$,
    $\text{MLP}_2: {k+1}\times 200, 200\times 200$,
    $\text{Attention}_2: 201\times 1$.

\end{itemize}

==> neurips 2022/section_tex_files/old-prelim.tex <==
\section{Hypergraphs, Hyperedge Operators and Hypergraph Diffusion} \label{sec:prelim}
In this section, we

1. Define hypergraphs, node potentials, hyperedge potentials

\begin{itemize}
    \item Attributed hypergraphs: $\gG=(V,E,X)$.  $X\in\mathbb{R}^{|V|\times m}$. $x_v$ denotes the attributes for node $v$. A hyperedge $e\in E$ is a subset of nodes $e=\{v_1^{(e)},...,v_{|e|}^{(e)}\}\subseteq V$ where $|e|$ is the hyperedge size. %(Start from 1-dim case for simplicity).
    
    \item Define node-diffused matrix $H\in\mathbb{R}^{|V|\times m}$ where $h_v$ denotes the row for node $v$. Given $e\in E$, we use notation bar-subscript $\bar{h}_e\in \mathbb{R}^{|e|\times m}$ to denote  concatenation $\oplus_{v\in e} h_v$ whose $i$th block is $h_{v_i^{(e)}}$. We also use the subscript without bar $q_e\in \mathbb{R}^{|e|\times m}$ to denote concatenation of $\oplus_{v\in e} q_{e,v}$ where $q_{e,v}\in \mathbb{R}^{m}$ which is a representation for a hyperedge-node pair.
    
    
    %= (h_{v_1^{(e)}},...,h_{v_|e|^{(e)}})$. %where $z_i = h_{v_i^{(e)}}$ for $i\in[e]$.
    
    \item Node potential: $f_v(\cdot ;x_v)$: $\mathbb{R}^{m} \rightarrow \mathbb{R}.$ %We assume that $f_v = f_{u}$ if the node degree $d_v = d_{u'}$.
    \item hyperedge potential: $g_e(\cdot): \mathbb{R}^{|e|\times m}\times \mathbb{R}$. %We
    %Denote $\bar{z} =(z_1,z_2^{(e)},...,z_|e|^{(e)})$ where $z_{i}^{(e)}$ is the block of the input vector $\bar{z}_e$ associated with node $v_{i}^{(e)}$.
    
    \item In hypergraphs, we often do not have node identities so $f_v=f_u$ if $d_v= d_{u}$. We also assume that $g_e = g_{e'}$ if $|e| = |e'|$ and $g_{e}$ is permutation invariant: $g_e(\bar{h}_e) = g_e(\bar{h}'_e)$ if $\{h_v|v\in e\}=\{h_v'|v\in e\}$. As the information of node degrees and hyperedge sizes are clear, we simply use $f$ and $g$ to uniformly denote node potentials and hyperedge potentials respectively.% by removing the subscripts for simplicity.
    
    
    %where $Z_e\in \mathbb{R}^{|e|\times m}$ and $P$ is a $|e|$-by-$|e|$ permutation matrix. As the information of node degrees and hyperedge sizes are clear, we simply use $f$ and $g$ by removing the subscripts for simplicity.
    %if $\{z_1^{(e)},z_2^{(e)},...,z_{|e|}^{(e)}\}=\{z_1'^{(e)},z_2'^{(e)},...,z_{|e|}'^{(e)}\}$. %In the following, for simplicity, our discussion focus on uniform hypergraphs, though experiments may have non-uniform hypergraphs. So we denote $g_e = g$ for simplicity.
\end{itemize}


2. Define hypergraph diffusion problems. Also discuss higher-order Markov random field MAP problem.

%Define $H\in\mathbb{R}^{|V|\times m}$ where $H_v$ denotes the row for node $v$.
\begin{itemize}
    \item Hypergraph diffusion $\min_{H} \sum_{v\in V} f(h_v; x_v) + \sum_{e\in E} g(\bar{h}_e).$
    \item Applications: Hypergraph cut, higher-order markov MAP, hypergraph PageRank diffusion.
\end{itemize}

\begin{itemize}
    \item For notational simplicity, for $h_v\in\mathbb{R}^m$, we define 
    \begin{align*}
        \nabla f(h_v;x) = \frac{\partial f(z;x)}{\partial z}|_{z=h_v}.  
    \end{align*}
    Given a hyperedge $e$ and $v\in e$, and $\bar{z}_e$ we define
    \begin{align*}
        \nabla_v g(\bar{h}_e) = \frac{\partial g(\bar{z}_e)}{\partial z_v}|_{\bar{z}_e=\bar{h}_e}.  
    \end{align*}
\end{itemize}



==> neurips 2022/section_tex_files/old2-002-prelim.tex <==
\section{Preliminaries: Hypergraphs and Hypergraph Diffusion} \label{sec:prelim}

% We are interested in supervised learning problems on hypergraphs by a diffusion model, in which we are given nodes with features and labels, as well as hyperedges connecting them.

In this section, we formulate the hypergraph diffusion problem, along the way, introduce the notations.
\begin{definition}[Hypergraph] \label{def:hypergraph}
Let $\Set{G} = (\Set{V}, \Set{E}, \Mat{X})$ be an attributed hypergraph where $\Set{V}$ is the node set of size $N$ and $\Set{E}$ is the hyperedge set of size $M$. Each hyperedge $e = \{v_1^{(e)},...,v_{\lvert e \rvert}^{(e)}\}$ is a subset of $\Set{V}$. Unlike graphs, a hyperedge may contain more than two nodes. $\Mat{X}=[...,x_v,...]^T\in\mathbb{R}^{N\times F}$ denotes the node attributes and $\Mat{x}_v$ denotes the attributes of node $v$. Define $d_v=|\{e\in\mathcal{E}:v\in e\}|$ as the degree of node $v$. Let $\Mat{D},\,\Mat{D}_e$ denote the diagonal degree matrix for $v\in\Set{V}$ and sub-matrix for $v\in e$.
%Let $\Mat{K} \in \{0, 1\}^{n \times m}$ denote the incident matrix where $\Mat{K}_{ij} = 1$ if and only if $v_i \in e_j$. 
\end{definition}
%A hyperedge $e$ may contain more than two nodes so hypergraphs are used to model higher-order relational data.
Learning algorithms may combine node attributes and hypergraph structures into (latent) features defined as follows. The features can be further used to make decision for downstream tasks.
\begin{definition}[Latent features] \label{def:node_feat}
Let $\Mat{h}_v \in \real^F$ denote the (latent) features of node $v\in \Set{V}$. The feature matrix $\Mat{H} = \begin{bmatrix}..., \Mat{h}_{v}, ... \end{bmatrix}_{v\in\Set{V}}^\top \in \real^{N \times F}$ include node features as rows. Further, collect the features into a edge feature matrix $\Mat{H}_e = \begin{bmatrix} \Mat{h}_{e, 1} & \cdots & \Mat{h}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert \times F}$, where $\Mat{h}_{e,i}$ corresponds to the feature $\Mat{h}_{v_i^{(e)}}$. Note that for any $v\in e$, there is one corresponding index $i\in e$. Later, we may use subscripts $(e,i)$ and $v$ interchangeably if causing no confusion. For, $i\in [F]$, we use $\Mat{H}_e[i]$ and $\Mat{h}_v[i]$ to denote the corresponding $i$th feature channels.
%collect all the feature vectors of nodes within edge $e$, where $\Mat{h}_{e,i}$ corresponds to the node features of node $v_i^{(e)}$ inside hyperedge $e$. 
%Suppose each node has initial features $\Mat{x}_i \in \real^d$ which are organized by initial feature matrix $\Mat{X} \in \real^{n \times d}$.
\end{definition}

A widely-used heuristic to generate features $\Mat{H}$ is via hypergraph diffusion algorithms. 

\begin{definition}[Hypergraph Diffusion] \label{def:node_feat}
Define node potential functions $f(\cdot;\Mat{x}_v):\mathbb{R}^{F} \rightarrow \mathbb{R}$ for $v\in\Set{V}$ and hyperedge potential functions $g_e(\cdot):\mathbb{R}^{|e|\times F} \rightarrow \mathbb{R}$ for each $e\in\Set{E}$.  The hypergrah diffusion combines the node attributes and the hypergraph structure and is to solve
\begin{align} \label{eqn:diffusion}
    \min_{\Mat{H}} \sum_{v \in \Set{V}} f(\Mat{h}_v; \Mat{x}_v) + \sum_{e \in \Set{E}} g_e(\Mat{H}_e).
\end{align}
In practice, $g_e$ is often shared across hyperedges up-to the size. So, later, we ignore the subscript $e$.
\end{definition}

Previously, the two potential functions are often designed via heuristics. Node potentials often correspond to negative-log kernels of the latent features and the initial attributes. For example, $f(\Mat{h}_v; \Mat{x}_v)$ could be $\|\Mat{h}_v - \Mat{x}_v\|_2^2$ when to compute hypergraph PageRank diffusion~\cite{li2018quadratic,takai2020hypergraph} or $-\Mat{h}_v^T\Mat{x}_v$ to essentially compute hypergraph min-cut~\cite{stobbe2010efficient}. Edge potentials in hypergraph modeling are more significant, as they need to capture relations between more than two objects. Here list a few examples. 

\begin{example}[Edge potentials] \label{exp:potential}
In practice, heuristic $g(\Mat{H}_e)$ can be chosen as follows. Note that most previous works only contain one feature channel $F=1$. Here, we list their general variants.
\begin{itemize}[leftmargin=3mm]
    \item Clique Expansion (CE, hyperedges reduced to cliques) plus pairwise potentials~\cite{zhou2007learning}: $\sum_{u,v\in e} \|\Mat{h}_v-\Mat{h}_{u}\|_2^2 $ or with properly degree normalization $\sum_{u,v\in e}\|\frac{\Mat{h}_v}{\sqrt{d_v}}-\frac{\Mat{h}_u}{\sqrt{d_u}}\|_2^2\,(\triangleq g(\Mat{D}_e^{-1/2}\Mat{H}_e))$.
    \item Divergence to the $p$-norm mean~\cite{tudisco2021nonlinear,tudisco2021nonlinear2}: $\sum_{v\in e} \|\Mat{h}_v-\|\Mat{H}_e\|_p\|_2^2$, where $\|\Mat{H}_e\|_p$ computes the $p$-norm each feature channel of $\Mat{H}_e$ separately.% where the number of features channels is $F=1$.
    \item Total Variation (TV)~\cite{hein2013total,zhang2017re}: $\sum_{i=1}^F\max_{u,v\in e} |\Mat{h}_v[i]-\Mat{h}_u[i]|^p$, $p\in\{1,2\}$.% where the number of features channels is $F=1$.
    \item Lov\'{a}sz Extension for cardinality-based set functions (LEC)~\cite{lovasz1983submodular,li2018quadratic,liu2021strongly}: $\sum_{i=1}^F\langle \Mat{y}_i, \varsigma(\Mat{H}_e[i]) \rangle^p$, $p\in\{1,2\}$ where $\varsigma(\Mat{H}_e[i])$ sort values of $\Mat{H}_e[i]$ in a decreasing order and $\Mat{y}_i\in\mathbb{R}^{|e|}$ is concave, i.e., $2\Mat{y}_i[j]\geq \Mat{y}_{i}[j-1]+\Mat{y}_i[j+1]$, $\forall j\in[e]$. Here, suppose  $\Mat{y}_{i}[-1]=\Mat{y}_{i}[|e|+1]=0$ for convenience.
    %\item Lov\'{a}sz Extension for cardinality-based set functions  (LE)~\cite{lovasz1983submodular,jegelka2013reflection,li2018revisiting,li2018quadratic}: $\sum_{i=1}^F\max_{\Mat{y}_i\in \Set{B}_e}\langle \Mat{y}_i, \Mat{H}_e[i] \rangle^p$, $p\in\{1,2\}$, where  $\Set{B}_e\subset\mathbb{R}^{|e|}$ is the base polytope induced by a submodular function defined on $e$. This generalizes total variation. 
\end{itemize}
\end{example}

To reveal more properties of $g(\cdot)$, we list the following formal definitions.

%Heuristic $g(\cdot)$'s are complicated while they all satisfies permutation invariance defined as follows.  %To reveal more properties of $g(\cdot)$, we list the following formal definitions:

\begin{definition} \label{def:permutation}
Let $\pi: [K] \rightarrow [K]$ be an automorphism, then permutation matrix  is defined as $\Mat{P}_{\pi}$ who has value one at entries $(\pi(i),i), \forall i \in [K]$ while taking zero at any other positions.
A permutation group $\Pi[K]$ is defined as a set which collects all of such $\Mat{P}_\pi$.
\end{definition}

\begin{definition}[Permutation Invariance \& Equivariance] \label{def:permutation_ivariant} 
Function $f(\cdot): \mathbb{R}^{K\times F} \rightarrow \real$ is permutation-invariant if $\,\forall \Mat{P} \in \Pi[K]$, $f(\Mat{P} \Mat{Z}) = f(\Mat{Z})$ for all $\Mat{Z} \in \mathbb{R}^{K\times F}$. Function $f(\cdot): \mathbb{R}^{K\times F} \rightarrow \mathbb{R}^{K\times F'}$ is permutation-equivariant if $\,\forall \Mat{P} \in \Pi[K]$, $f(\Mat{P} \Mat{Z}) = \Mat{P}f(\Mat{Z})$ for all $\Mat{Z} \in \mathbb{R}^{K\times F}$.
\end{definition}

%\begin{definition} \label{def:permutation_equivariant} (Permutation Equivariance)
%Let $f: \real^k \rightarrow \real^k$ be a permutation-equivariant function, then $\forall \Mat{P} \in \Grp{P}_k$, $f(\Mat{P} \Mat{x}) = \Mat{P} f(\Mat{x})$ for all $\Mat{x} \in \real^k$.
%\end{definition}

We may easily verify the permutation invariance of the heuristic edge potentials in  Example~\ref{exp:potential}. The physical meaning behind this observation is that the prediction goal of an application is often independent of node identities so most practical $g$'s  keep invariance w.r.t. the node ordering~\cite{veldt2020hypergraph}.
%affect the diffusion results.   

%We note that potential function $g(\cdot)$ should be permutation-invariant since row permutation of the edge feature matrix results in an equivalent class. \pan{This may be more natural put with g definition together.}
%No matter in which order we arrange data inside $\Mat{H}_e$, $g(\cdot)$ should give the identical potential value. 




% Here are a few examples. 
% \begin{example}[Node potentials]
% The node potential $f(\Mat{h}_v; \Mat{x}_v)$ often corresponds to a negative-log kernel of the latent features and the initial attributes: (a) Hypergraph PageRank diffusion~\cite{li2018quadratic,takai2020hypergraph}, $\|\Mat{h}_v - \Mat{x}_v\|_2^2$; (b) Hypergraph min-cut diffusion~\cite{stobbe2010efficient}, $-\Mat{h}_v^T\Mat{x}_v$.
% \end{example}

% For example, node potential $f(\Mat{h}_v; \Mat{x}_v)$ could be $\|\Mat{h}_v - \Mat{x}_v\|_2^2$ when to compute hypergraph PageRank diffusion~\cite{li2018quadratic,takai2020hypergraph} or $-\Mat{h}_v^T\Mat{x}_v$ to compute hypergraph cut~\cite{stobbe2010efficient}. Examples of edge potentials $g(\Mat{H}_e)$ include a combination of clique expansion and pairwise potentials $\sum_{u,v\in e} \|\Mat{x}_v-\Mat{x}_u\|_2^2$, Lov\'{a}sz extension and \cite{tudisco2021nonlinear}.   

% (Heuristics, cannot apply to heterophilic)

% hypergraph diffusion include hypergraph  

% Node potential: $f_v(\cdot ;x_v)$: $\mathbb{R}^{m} \rightarrow \mathbb{R}.$ %We assume that $f_v = f_{u}$ if the node degree $d_v = d_{u'}$.
%     \item hyperedge potential: $g_e(\cdot): \mathbb{R}^{|e|\times m}\times \mathbb{R}$. %We
%     %Denote $\bar{z} =(z_1,z_2^{(e)},...,z_|e|^{(e)})$ where $z_{i}^{(e)}$ is the block of the input vector $\bar{z}_e$ associated with node $v_{i}^{(e)}$.
    
%     \item In hypergraphs, we often do not have node identities so $f_v=f_u$ if $d_v= d_{u}$. We also assume that $g_e = g_{e'}$ if $|e| = |e'|$ and $g_{e}$ is permutation invariant: $g_e(\bar{h}_e) = g_e(\bar{h}'_e)$ if $\{h_v|v\in e\}=\{h_v'|v\in e\}$. As the information of node degrees and hyperedge sizes are clear, we simply use $f$ and $g$ to uniformly denote node potentials and hyperedge potentials respectively.

% Unlike ordinary graphs, a hyperedge can connect with more than two nodes, i.e., $\lvert e \rvert \ge 2$.
% To attain node adjacent matrix (i.e., an $n$ by $n$ matrix whose non-zero entries indicate which two nodes are connected), one can use $\Mat{K}\Mat{K}^\top$ that transforms hyperedges into cliques.
% \begin{definition}[Node features] \label{def:node_feat}
% Let $\Mat{h}_i \in \real^d$  \pan{revise to $F$} be the node embedding of the node $v_i \in \Set{V}$. We organize all the node features into the rows of a feature matrix $\Mat{H} = \begin{bmatrix} \Mat{h}_{1} & \cdots & \Mat{h}_{n} \end{bmatrix}^\top \in \real^{n \times d}$. Suppose each node has initial features $\Mat{x}_i \in \real^d$ which are organized by initial feature matrix $\Mat{X} \in \real^{n \times d}$.
% \end{definition}

% % Similarly, we let matrix $\Mat{H} = \begin{bmatrix} \Mat{h}_{1} & \cdots & \Mat{h}_{n} \end{bmatrix}^\top \in \real^{n \times d}$ concatenates all the node features after diffusion.
% \begin{definition}[Edge features] \label{def:edge_feat}
% % Given an hyperedge $e \in \Set{E}$, the 
% Let edge feature matrix $\Mat{H}_e = \begin{bmatrix} \Mat{h}_{e, 1} & \cdots & \Mat{h}_{e, \lvert e \rvert} \end{bmatrix}^\top \in \real^{\lvert e \rvert \times d}$ collect all the feature vectors of nodes within edge $e$, where $\Mat{h}_{e,i}$ corresponds to the node features of node $v_i^{(e)}$ inside hyperedge $e$. \pan{Define the relation between $\Mat{h}_{e}$ and $\Mat{h}$. Denote an implicit mapping between $(e,i)$ and $(e,v)$.}
% \end{definition}

% Hypergraph diffusion algorithms solve node embeddings \pan{unify the terminology} $\Mat{H}$ to minimize some potential functions \pan{add some background} defined over hypergraphs.
% We proposed a general hypergraph diffusion model \pan{Review hypergraph diffusion instead of proposing a model; Also motivates the applications of this is crucial.} that accumulates potential of individual node embeddings and the joint potential among nodes connected by each hyperedge in a hypergraph $\Set{G}$:
% \begin{align} \label{eqn:diffusion}
%     \min_{\Mat{H}} \sum_{v \in \Set{V}} f(\Mat{h}_v; \Mat{x}_v) + \sum_{e \in \Set{E}} g(\Mat{H}_e),
% \end{align}
% where $f: \real^{d} \rightarrow \real$ denotes the node potential function, which defines an independent likelihood of each node representation, $g
% : \real^{\lvert e \rvert \times d} \rightarrow \real$ is the hyperedge potential function \pan{different hyperedges may have different sizes}, which specifies a joint constraints on the embeddings of nodes connected by one hyperedge.
% \textcolor{red}{High-Order Page Rank}.
% \textcolor{red}{High-Order Markov Random Field}.

% To optimize Eq.~\eqref{eqn:diffusion}, it is often to use gradient-based methods which we will elaborate in Sec. \ref{sec:model} \pan{Need better motivations, add references and discuss previous approaches; Okay, we should put this into the next section.}. 
% Suppose $f(\cdot)$ and $g(\cdot)$ are differentiable, then we denote the gradient of $f(\cdot)$ taking value at $\Mat{h}_v$ as: $\nabla f(\Mat{h}_v; \Mat{x}) = \frac{\partial f(\Mat{z}; \Mat{x})}{\partial \Mat{z}} \lvert_{\Mat{z} = \Mat{h}_v}$,
% and since $g(\cdot)$ is a function of a set of nodes, its partial derivative with respect to node $v$ taking value at $\Mat{H}_e$ is defined as: $\nabla_v g(\Mat{H}_e) = \nabla_v g\left(\Mat{h}_{e, 1}, \cdots, \Mat{h}_{e,\lvert e \rvert}\right) = \frac{\partial_v g\left(\Mat{z}_{e, 1}, \cdots, \Mat{z}_{e, \lvert e \rvert}\right)}{\partial \Mat{z}_{e, v}} \Big\lvert_{\Mat{z}_{e,i} = \Mat{h}_{e,i}}$ \pan{I think this notation may have some issues.}.
% To reveal more properties of $g(\cdot)$, we list the following formal definitions:

% \begin{definition} \label{def:permutation}
% Let $\pi: [k] \rightarrow [k]$ be an automorphism, then permutation matrix  is defined as $\Mat{P}_{\pi}$ who has value one at entries $(i, \pi(i)), \forall i \in [k]$ while taking zero at any other positions.
% A permutation group $\Grp{P}_k$ \pan{revise to $\Pi[k]$} is defined as a set which collects all of such $\Mat{P}_\pi$.
% \end{definition}

% \begin{definition} \label{def:permutation_ivariant} (Permutation Invariance)
% Let $f: \real^k \rightarrow \real$ be a permutation-invariant function, then $\forall \Mat{P} \in \Grp{P}_k$, $f(\Mat{P} \Mat{x}) = f(\Mat{x})$ for all $\Mat{x} \in \real^k$.
% \end{definition}

% \begin{definition} \label{def:permutation_equivariant} (Permutation Equivariance)
% Let $f: \real^k \rightarrow \real^k$ be a permutation-equivariant function, then $\forall \Mat{P} \in \Grp{P}_k$, $f(\Mat{P} \Mat{x}) = \Mat{P} f(\Mat{x})$ for all $\Mat{x} \in \real^k$.
% \end{definition}

% We note that potential function $g(\cdot)$ should be permutation-invariant since row permutation of the edge feature matrix results in an equivalent class. \pan{This may be more natural put with g definition together.}
% No matter in which order we arrange data inside $\Mat{H}_e$, $g(\cdot)$ should give the identical potential value. 



% \begin{itemize}
%     \item Attributed hypergraphs: $\gG=(V,E,X)$.  $X\in\mathbb{R}^{|V|\times m}$. $x_v$ denotes the attributes for node $v$. A hyperedge $e\in E$ is a subset of nodes $e=\{v_1^{(e)},...,v_{|e|}^{(e)}\}\subseteq V$ where $|e|$ is the hyperedge size. %(Start from 1-dim case for simplicity).
    
%     \item Define node-diffused matrix $H\in\mathbb{R}^{|V|\times m}$ where $h_v$ denotes the row for node $v$. Given $e\in E$, we use notation bar-subscript $\bar{h}_e\in \mathbb{R}^{|e|\times m}$ to denote  concatenation $\oplus_{v\in e} h_v$ whose $i$th block is $h_{v_i^{(e)}}$. We also use the subscript without bar $q_e\in \mathbb{R}^{|e|\times m}$ to denote concatenation of $\oplus_{v\in e} q_{e,v}$ where $q_{e,v}\in \mathbb{R}^{m}$ which is a representation for a hyperedge-node pair.
    
    
%     %= (h_{v_1^{(e)}},...,h_{v_|e|^{(e)}})$. %where $z_i = h_{v_i^{(e)}}$ for $i\in[e]$.
    
%     \item Node potential: $f_v(\cdot ;x_v)$: $\mathbb{R}^{m} \rightarrow \mathbb{R}.$ %We assume that $f_v = f_{u}$ if the node degree $d_v = d_{u'}$.
%     \item hyperedge potential: $g_e(\cdot): \mathbb{R}^{|e|\times m}\times \mathbb{R}$. %We
%     %Denote $\bar{z} =(z_1,z_2^{(e)},...,z_|e|^{(e)})$ where $z_{i}^{(e)}$ is the block of the input vector $\bar{z}_e$ associated with node $v_{i}^{(e)}$.
    
%     \item In hypergraphs, we often do not have node identities so $f_v=f_u$ if $d_v= d_{u}$. We also assume that $g_e = g_{e'}$ if $|e| = |e'|$ and $g_{e}$ is permutation invariant: $g_e(\bar{h}_e) = g_e(\bar{h}'_e)$ if $\{h_v|v\in e\}=\{h_v'|v\in e\}$. As the information of node degrees and hyperedge sizes are clear, we simply use $f$ and $g$ to uniformly denote node potentials and hyperedge potentials respectively.% by removing the subscripts for simplicity.
    
    
%     %where $Z_e\in \mathbb{R}^{|e|\times m}$ and $P$ is a $|e|$-by-$|e|$ permutation matrix. As the information of node degrees and hyperedge sizes are clear, we simply use $f$ and $g$ by removing the subscripts for simplicity.
%     %if $\{z_1^{(e)},z_2^{(e)},...,z_{|e|}^{(e)}\}=\{z_1'^{(e)},z_2'^{(e)},...,z_{|e|}'^{(e)}\}$. %In the following, for simplicity, our discussion focus on uniform hypergraphs, though experiments may have non-uniform hypergraphs. So we denote $g_e = g$ for simplicity.
% \end{itemize}

% \paragraph{Hypergraph Convolutional Networks}
% Graph neural networks (GNN) are broadly adopted for learning problems on graphs.
% Recent works \cite{feng2019hypergraph, bai2021hypergraph, yadati2019hypergcn, dong2020hnhn, huang2021unignn} have generalized various GNNs for ordinary graphs onto hypergraphs.
% Nevertheless, most of existing hypergraph convolution are based on clique expansion propagation with degree normalization and nonlinear transformation.
% Taking HGNN \cite{feng2019hypergraph} for an example, it has the following node-wise update formula for each layer:
% \begin{align} \label{eqn:hgnn}
%     \Mat{h}_v^{(t+1)} = \sigma\left( \frac{1}{\sqrt{d_v}} \sum_{e: v \in e} \frac{1}{\lvert e \rvert} \sum_{u: u \in e} \frac{\Mat{h}_u^{(t)}}{\sqrt{d_u}} \Mat{\Theta}^{(t)} + \Mat{b}^{(t)} \right),
% \end{align}
% where $\Mat{h}_v^{(t)}$ denotes the features of node $v$ at the $t$-th layer, $d_v$ denotes the degree of node $v$, $\sigma$ is a non-linear activation, and $\Mat{\Theta}^{(t)}, \Mat{b}^{(t)}$ are parameters of linear transformation and bias, respectively.
% We argue that each layer's update (Eq. \ref{eqn:hgnn}) can be regarded as an optimization step of a special case of objective Eq. \ref{eqn:diffusion}.
% We show this by letting $g(\Mat{Z}_e) = \sum_{(v, u) \in e} \lVert \Mat{h}_v^{(e)}/\sqrt{d_v} - \Mat{h}_u^{(e)}/\sqrt{d_u} \rVert_2^2$ and $f(\Mat{h}_v; \Mat{x}_v) = 0$.
% Since $g$ is strongly convex, we can reach optimum by gradient descent. And the gradient step will coincide with Eq. \ref{eqn:hgnn} in form.
% \textcolor{red}{need a derivation and correction later.}
% \textcolor{red}{add AllSet?}

% \paragraph{Nonlinear Hypergraph Diffusion (HyperND)}



